Morphism of T*-Representations

Importance of theorem dedicated to isomorphisms consist in statement that they allow to identify different mathematical objects which have something common from the point of view of certain model. This paper considers morphisms of \Ts representation of $\mathfrak{F}$\Hyph algebra and morphisms of \Ts representation of fibered $\mathfrak{F}$\Hyph algebra.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{texSpaceTime}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{texSpaceTime}{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{texSpaceTime}{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{texSpaceTime}{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{texSpaceTime}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{texGenRelativity}{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{texGenRelativity}{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{texAffine,texGeomObject}{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{texAffine}{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{texAffine}{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{texAffine}{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{texAffine}{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{texTidal,texAffine,texGeomObject}{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{texTidal,texNewton}{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{texNewton}{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{texNewton}{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{texLagrange}{Weinberg}
{
Steven Weinberg. The Quantum Theory of Fields. Cambridge university press.
}%

\BiblioItem{texLagrange}{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{texLagrange}{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{texTidal}{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{texPrefaceTidal,texPrefaceRefernceFrame}{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{texTidal}{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{texReferenceFrame,texFiberedAlgebra}{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{texFiberedAlgebra,texTstarMorphism}{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{texGeomObject}{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{texBundle}{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{texAffine,texRepresentation,texBasis,texDrcBasis,texVectorSpace,texLinearMap,texPolyvector}
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem{texPolyvector}{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{texDrcBasis,texBasis}{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{texBundle}{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{texPrefaceRefernceFrame}{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{texPrefaceRefernceFrame}{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{texPrefaceRefernceFrame}{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{texPrefaceRefernceFrame}{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{texPrefaceRefernceFrame}{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame}{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame}{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame,texPrefaceTidal}{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{texBiring,texVectorSpace}{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{texBiring,texVectorSpace}
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{texVectorSpace}{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{texVectorSpace}{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{texVectorSpace}{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{texVectorSpace}{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{texDrcReferenceFrame,texRefernceFrame,texLie,texLieRepresentation}{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2004)
}%

\BiblioItem{texAffine}{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2004)
}%

\BiblioItem{texTidal}{0405.028}
{
Aleks Kleyn, Metric\hyph Affine Manifold,
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2004)
}%

\BiblioItem{texFiberedAlgebra,texBundleRelation,texTstarMorphism}{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2007)
}%

\BiblioItem{texBundleRelation,texPrefaceRelation}{0702.561}
{
Александр Клейн,
Расслоенная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

%\BiblioItem{texBasis,texLinearMap}{math.RA-0501237}
%{
%Александр Клейн,
%Векторное пространство над телом,\\
%eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2005)
%}%

\BiblioItem{texPolymodule}{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Skew-Field, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\ifx\texBiring\Defined
\else
\BiblioItem{texVectorSpace,texFiberedAlgebra}{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2006)
}%
\fi

\ifx\texBundleRelation\Defined
\else
\BiblioItem{texFiberedMorphism}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\ifx\PrintBook\Defined
\BiblioItem{texPrefaceRelation}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\BiblioItem{texHomotopy}{q-alg-9705009}
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{texPrefaceRelation}{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem{texBundleRelation,texPrefaceRelation,texTstarMorphism,texBundle}
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem{texBundle}
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{texFiberedAlgebra}{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{texBundleRelation}{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{texBundle,texCartesian,texFiberedAlgebra,texBundleRelation,texFiberedMorphism}
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{texCalculus}{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{texCalculus}{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{texCalculus}{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem{texFiberedMorphism}{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{texFiberedAlgebra,texFiberedMorphism}{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{texFiberedMorphism}{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{texFiberedMorphism}{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{texPolyvector}{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\CloseBiblio



==> Bundle.Russian.tex <==
%auto-ignore
\def\texBundle{}

\ifx\PrintBook\Defined
				\chapter{Декартово произведение расслоений}
\fi
			\section{Расслоение}

Допустим $M$ - многообразие и
\symb{\bundle{\mathcal{E}}pEM}0{bundle}
	\begin{equation}
	\label{eq: bundle, definition}
\ShowSymbol{bundle}
	\end{equation}
расслоение над $M$ со слоем $E$.\footnote{Так как мне придётся иметь
дело с различными расслоениями, я буду
пользоваться следующим соглашением. Для обозначения расслоения и слоя я буду пользоваться одной
и той же буквой в разных алфавитах.}
Символ $\bundle{}pE{}$ означает, что
$E$ является типичным слоем расслоения.
Множество $\mathcal{E}$ является областью определения
отображения $\bundle{}pE{}$.
Множество $M$ является областью значений
отображения $\bundle{}pE{}$.
Мы будем отождествлять непрерывное отображение $\bundle{}pE{}$
и расслоение \eqref{eq: bundle, definition}.
Отображение $p$ называется
\AddIndex{проекцией расслоения $\mathcal{E}$ вдоль слоя $E$}
{projection of bundle along fiber}.
Обозначим через
\symb{\Gamma(\bundle{}pE{})}1{set of sections of bundle}
множество сечений расслоения $\bundle{}pE{}$.

		\begin{definition}
		\label{definition: locally compact space}
Пространство называется \AddIndex{локально компактным в точке}{locally compact at point space} $p$,
если существует открытое множество $U$, $p\in U$, замыкание которого $\overline U$ компактно.
Пространство называется \AddIndex{локально компактным}{locally compact space},
если оно локально компактно в каждой своей точке.\footnote{Я следую
определению из \citeBib{Hocking Young Topology}, с. 71.}
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: topology finer coarser}
Пусть даны топологии $\mathcal{T}_1$, $\mathcal{T}_2$ в
множестве $X$. Говорят, что $\mathcal{T}_1$ мажорирует $\mathcal{T}_2$ и
что $\mathcal{T}_2$ мажорируется $\mathcal{T}_1$,
если тождественное отображение $X_1\rightarrow X_2$,
где $X_i$ - множество $X$, наделённое топологией $\mathcal{T}_i$,
$i=1,2$, непрерывно. Если $\mathcal{T}_1\ne\mathcal{T}_2$,
то говорят, что $\mathcal{T}_1$ сильнее $\mathcal{T}_2$ и
$\mathcal{T}_2$ слабее $\mathcal{T}_1$.
		\qed
		\end{definition}

Пусть топология $\mathcal{T}_1$ в
множестве $X$ мажорирует топологию $\mathcal{T}_2$. Рассмотрим
диаграмму
\[
\xymatrix{
&&X_1\ar[dd]^{\mathrm{id}}\ar[drr]^{g_1}\\
Y\ar[urr]^{f_1}\ar[drr]_{f_2}&&&&Z\\
&&X_2\ar[urr]_{g_2}
}
\]
Согласно определению \ref{definition: topology finer coarser},
если отображение $f_1$ - непрерывно, то непрерывно отображение $f_2$.
Аналогично,
если отображение $g_2$ - непрерывно, то непрерывно отображение $g_1$.

Пусть $\bundle{\mathcal{E}}pEM$ - расслоение.
Рассмотрим открытое множество $U\subset M$ такое, что существует
локальная тривиализация $\varphi$
	\[
\xymatrix{
U\times E\ar[rr]^{\varphi}\arp[rd]_p
&&\mathcal{E}|_U\arp[ld]^{\bundle{}pE{}}\\
&U
}
	\]
Так как $\varphi$ гомеоморфизм, то топологии в $U\times E$ и $\mathcal{E}|_U$
сравнимы. Так как $U\times E$ - декартово произведение топологических пространств
$U$ и $E$, то мы определим в $\mathcal{E}|_U$ слабейшую из топологий,
при которых непрерывна проекция $\bundle{}pE{}$
(\citeBib{Bourbaki: General Topology 1}, стр. 37).

Отношение $r$ в $\mathcal{E}$ такое, что $(p,q)\in r$ тогда и только тогда,
когда $p$ и $q$ принадлежат одному слою, является отношением эквивалентности.
$\bundle{}pE{}$ - естественное отображение. Рассмотрим диаграмму
	\[
\xymatrix{
\mathcal{E}\arp[d]_{\bundle{}pE{}}\ar[drr]^g\\
M\ar[rr]_f&&N
}
	\]
Из непрерывности отображения $f$ следует непрерывность отображения $g$.
Следовательно, мы можем определить в $M$ фактортопологию,
сильнейшую из топологий, при которых $\bundle{}pE{}$ непрерывно
(\citeBib{Bourbaki: General Topology 1}, стр. 39).

\AddIndex{Декартова степень $A$ множества $B$}{Cartesian power of set}
- это множество \symb{B^A}1{Cartesian power of set}
отображений $f:A\rightarrow B$
(\citeBib{Cohn: Universal Algebra}, стр. 18).
Рассмотрим подмножества $B^A$ вида
\[
W_{K,U}=\{f:A\rightarrow B|f(K)\subset U\}
\]
где $K$ - компактное подмножество пространства $A$,
$U$ - открытое подмножество пространства $B$.
Множества $W_{K,U}$ образуют базис топологии
пространства $B^A$. Эта топология называется
\AddIndex{компактно\hyph открытой топологией}{compact open topology}.
Декартова степень $A$ множества $B$,
снабжённая компактно\hyph открытой топологией называется,
\AddIndex{пространством отображений}{mapping space}
(\citeBib{Maunder: Algebraic Topology}, стр. 213).

Согласно \citeBib{Maunder: Algebraic Topology}, стр. 214
для данных пространств $A$, $B$, $C$, $D$ и
отображений $f:A\rightarrow C$, $g:D\rightarrow B$
мы определим морфизм пространства отображений
\[
g^f:D^C\rightarrow B^A
\]
равенством
\begin{align*}
g^f(h)&=fhg&h:&C\rightarrow D&g^f(h):&A\rightarrow B
\end{align*}
Таким образом, морфизм пространства отображений можно представить
с помощью диаграммы
	\[
\xymatrix{
A\ar[rr]^f\ar[d]_{g^f(h)}&&C\ar[d]^h\\
B&&D\ar[ll]^g
}
	\]

		\begin{remark}
		\label{remark: set of sections of bundle, topology}
Множество $\Gamma(\mathcal{E})$ является подмножеством
множества $\mathcal{E}^M$.
Поэтому мы можем перенести на множество сечений понятия,
определённые для  пространства отображений.
Множества $W_{K,U}$ мы определим следующим образом
\[
W_{K,U}=\{f\in\Gamma(\mathcal{E})|f(K)\subset U\}
\]
где $K$ - компактное подмножество пространства $M$,
$U$ - открытое подмножество пространства $\mathcal{E}$.
		\qed
		\end{remark}

	\begin{remark}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
	\qed
	\end{remark}

	\begin{remark}
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
	\qed
	\end{remark}

		\begin{definition}
		\label{definition: fibered morphism}
Рассмотрим расслоения $$\bundle{\mathcal{A}}pAM$$
и $$\bundle{\mathcal{B}}qBN$$
Пара отображений
\symb{(\begin{array}{cc}
\mathcal{F}:\mathcal{A}\rightarrow\mathcal{B},&
f:M\rightarrow N
\end{array})}
0{fibered morphism from A into B}
	\begin{equation}
\ShowSymbol{fibered morphism from A into B}
	\label{eq: fibered morphism}
	\end{equation}
таких, что диаграма
	\[
\xymatrix{
\mathcal{A}\arp[d]^{\bundle{}pA{}}\ar[rr]^{\mathcal{F}}
&&\mathcal{B}\arp[d]^{\bundle{}qB{}}\\
M\ar[rr]^f&&N
}
	\]
коммутативна, называется
\AddIndex{расслоенным морфизмом из расслоения $\mathcal{A}$ в $\mathcal{B}$}
{fibered morphism from A into B}.
Отображение $f$ называется
\AddIndex{базой отображения}{base of map} $\mathcal{F}$.
Отображение $\mathcal{F}$ называется
\AddIndex{лифтом отображения}{lift of map} $f$.
		\qed
		\end{definition}

	\begin{theorem}
	\label{theorem: fibered morphism defines morphism of spaces of sections}
Если отображение $f$ - биекция, то
отображение $\mathcal{F}$ определяет морфизм $\mathcal{F}^{f^{-1}}$ пространств сечений
$\Gamma(\bundle{}pA{}))$ в $\Gamma(\bundle{}qB{}))$
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{A}\ar[rr]^{\mathcal{F}}&&\mathcal{B}
&u'=\mathcal{F}^{f^{-1}}(u)=\mathcal{F}uf^{-1}\\
M\ars[u]^u="U"\ar[rr]^f&&N\ars[u]_{u'}="UP"
\ar @{=>}^{\mathcal{F}^{f^{-1}}} "U";"UP"
}
	\]%
\shorthandon{"}%
		\end{theorem}
		\begin{proof}
Чтобы доказать непрерывность $u'$, достаточно доказать
непрерывность $f^{-1}$. Но это очевидно, так как $f$
непрерывная биекция.

Мы будем полагать, что на множествах
$\Gamma(\bundle{}pA{}))$ и $\Gamma(\bundle{}qB{}))$
определена топология согласно замечанию
\ref{remark: set of sections of bundle, topology}.
Рассмотрим сечения
$u$, $v\in\Gamma(\bundle{}pA{}))$, 
$u'=\mathcal{F}^{f^{-1}}(u)$, $v'=\mathcal{F}^{f^{-1}}(u')$
такие, что существует
$W_{L,V}\subset\Gamma(\bundle{}qB{}))$,
где $L$ - компактное подмножество пространства $N$,
$V$ - открытое подмножество пространства $\mathcal{B}$,
$u'$, $v'\in W_{L,V}$.
Так как $f$ - непрерывная биекция,
то $K=f^{-1}(L)$ - компактное подмножество пространства $M$.
Так как $\mathcal{F}$ - непрерывно,
то $U=\mathcal{F}^{-1}(V)$ - открытое подмножество пространства $\mathcal{A}$.

Согласно построению
	\begin{equation}
u'f=\mathcal{F}u
	\label{eq: fibered morphism defines morphism of spaces of sections, 1}
	\end{equation}
Из \eqref{eq: fibered morphism defines morphism of spaces of sections, 1} следует
	\begin{equation}
\mathcal{F}u(K)=u'f(K)=u'(L)\subset V
	\label{eq: fibered morphism defines morphism of spaces of sections, 2}
	\end{equation}
Из \eqref{eq: fibered morphism defines morphism of spaces of sections, 2} следует
	\begin{equation}
u(K)\subset \mathcal{F}^{-1}V=U
	\label{eq: fibered morphism defines morphism of spaces of sections, 3}
	\end{equation}
Из \eqref{eq: fibered morphism defines morphism of spaces of sections, 3} следует
$u\in W_{K,U}$. Аналогично доказывается, что $u'\in W_{K,U}$.
Следовательно, для открытого множества $W_{L,V}$ мы нашли открытое множество $W_{K,U}$
такое, что $\mathcal{F}^{f^{-1}}(W_{K,U})\subset W_{L,V}$.
Это доказывает непрерывность отображения $\mathcal{F}^{f^{-1}}$.
		\end{proof}

Если $f=\mathrm{id}$, то $\mathrm{id}^{-1}=\mathrm{id}$.
Поэтому морфизм пространств сечений
мы будем обозначать $\mathcal{F}^{\mathrm{id}}$. Очевидно
\[
\mathcal{F}^{\mathrm{id}}(u)=\mathcal{F}u
\]

		\begin{definition}
		\label{definition: fibered subset}
Пусть $\bundle{\mathcal{A}}aAN$ и $\bundle{\mathcal{B}}bBM$ - расслоения.
Пусть расслоенный морфизм $(\begin{array}{cc}
\mathcal{F}:\mathcal{A}\rightarrow\mathcal{B},&
f:M\rightarrow N
\end{array})$ определён диаграммой
	\[
\xymatrix{
\mathcal{A}\arp[d]^{\bundle{}aA{}}\ar[rr]^{\mathcal{F}}
&&\mathcal{B}\arp[d]^{\bundle{}{b}{B}{}}\\
N\ar[rr]^f&&M
}
	\]
где отображения $\mathcal{F}$ и $f$ инъективны. Тогда мы называем расслоение $\bundle{}aA{}$
\AddIndex{расслоенным подмножеством}{fibered subset} или
\AddIndex{подрасслоением}{subbundle} расслоения $\bundle{}bB{}$.
Мы будем также пользоваться записью
\symb{\bundle{}{a}{A}{}\subseteq\bundle{}{b}{B}{}}1{fibered subset} либо
\symb{\mathcal{A}\subseteq\mathcal{B}}1{subbundle}.

Не нарушая общности, мы можем полагать $A\subseteq B$, $N\subseteq M$.
		\qed
		\end{definition}

Рассмотрим расслоения $$\bundle{\mathcal{A}}pAM$$
и $$\bundle{\mathcal{B}}qBN$$
\AddIndex{Декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}{Cartesian power of bundle}
- это множество \symb{\bundle{}qB{}^{\bundle{}pA{}}}1{Cartesian power of bundle}
расслоенных морфизмов $$(\begin{array}{cc}
\mathcal{F}:\mathcal{A}\rightarrow\mathcal{B},&
f:M\rightarrow N
\end{array})$$
В данный момент я не вижу как определить структуру расслоения
в декартовой степени расслоения.
Хотя для заданных $m\in M$, $n\in N$
я могу рассмотреть декартову степень $B_n{}^{A_m}$.
Опираясь на теорему
\ref{theorem: fibered morphism defines morphism of spaces of sections},
мы можем определить отображение
\[
f:\bundle{}qB{}^{\bundle{}pA{}}\rightarrow\Gamma(\mathcal{B})^{\Gamma(\mathcal{A})}
\]
%Рассмотрим подрасслоения $\bundle{}qB{}^{\bundle{}pA{}}$ вида
%\[
%W_{K,U}=\{f:A\rightarrow B|f(K)\subset U\}
%\]
%где $K$ - компактное подмножество пространства $A$,
%$U$ - открытое подмножество пространства $B$.
Рассмотрим подмножества $W_{K,U}\subset\Gamma(\mathcal{B})^{\Gamma(\mathcal{A})}$,
где $K$ - компактное подмножество сечений расслоения $\mathcal{A}$,
$U$ - открытое подмножество сечений расслоения $\mathcal{B}$.
Множества
$W_{K,U}$
образуют базис топологии
пространства $\Gamma(\mathcal{B})^{\Gamma(\mathcal{A})}$.
Мы выберем самую слабую топологию в $\bundle{}qB{}^{\bundle{}pA{}}$, 
при которой отображение $f$ непрерывно.

Мы рассмотрели структуру открытого множества сечений
расслоения $\mathcal{B}$
в замечании \ref{remark: set of sections of bundle, topology}.
Так как множество сечений расслоения $\mathcal{A}$
является множеством отображений, то мы можем
искать подобие теоремы Арцела для анализа,
(\citeBib{Kolmogorov Fomin}, стр. 110),
что бы ответить на вопрос, когда это множество
является компактным. На данном этапе я этот вопрос оставляю
открытым.

%\mathcal{B}^\mathcal{A}
Согласно \citeBib{Maunder: Algebraic Topology}, стр. 214
для данных пространств $A$, $B$, $C$, $D$ и
отображений $f:A\rightarrow C$, $g:D\rightarrow B$
мы определим морфизм пространства отображений
\[
g^{(\begin{array}{cc}
\mathcal{F}:\mathcal{A}\rightarrow\mathcal{B},&
f:M\rightarrow N
\end{array})}:D^C\rightarrow B^A
\]
равенством
\begin{align*}
g^f(h)&=fhg&h:&C\rightarrow D&g^f(h):&A\rightarrow B
\end{align*}
Таким образом, морфизм пространства отображений можно представить
с помощью диаграммы
	\[
\xymatrix{
A\ar[rr]^f\ar[d]_{g^f(h)}&&C\ar[d]^h\\
B&&D\ar[ll]^g
}
	\]

\ifx\texFuture\Defined
Прежде всего возникает вопрос. Что мы называем расслоением? Когда
мы говорим о расслоении, мы подразумеваем непрерывность базы и
непрерывность слоя. Если слой имеет дискретную топологию, то мы
называем соответствующее множество не расслоением, а слоением.
Расслоения и слоения очень сильно отличаются, и потому мы
используем различные методы для их изучения.
 
Тем не менее, если отвлечься от топологии слоя, эти объекты имеют
нечто общее. Кроме того, нужно иметь в виду следующее.
\begin{itemize}
\item Алгебра может быть определена не только на непрерывном множестве.
Конечные и дискретные группы, например, важны при изучении
многих геометрических объектов и физических явлений.
\item Фактор множество топологического пространства может оказаться
конечным множеством, тем самым разрушая топологию.
В то же время совсем не очевидно, почему мы не должны
рассматривать подобного рода отношение эквивалентности.
\end{itemize}

На данном этапе для меня топология слоя несущественна, но важна
непрерывность базы. Принимая во внимание высказанные выше соображения,
я не буду делать различия между расслоением и накрытием
и буду называть и то, и другое расслоением.
\fi


==> Drc.Morphism.Russian.tex <==
%auto-ignore
\def\texDrcMorphism{}

			\section{\texorpdfstring{$D\RCstar$}{Drc}\hyph линейное отображение векторных пространств}
			\label{section: Linear Map of Vector Spaces}

		\begin{definition}
		\label{definition: src trc linear map of vector spaces}
Пусть $\mathcal{A}$ - $S\RCstar$\Hyph векторное пространство.
Пусть $\mathcal{B}$ - $T\RCstar$\Hyph векторное пространство.
Мы будем называть морфизм
	\[
\xymatrix{
f:S\ar[r]&T&\Vector{A}:\mathcal{A}\ar[r]&\mathcal{B}
}
	\]
\Ts представлений тела в абелевой группе
\AddIndex{$(S\RCstar,T\RCstar)$\Hyph линейным отображением векторных пространств}
{src trc linear map of vector spaces}.
		\qed
		\end{definition}

Согласно теореме
\ref{theorem: decompositions of morphism of representations}
при изучении $(S\RCstar,T\RCstar)$\Hyph линейного отображения
мы можем ограничиться случаем $S=T$.

		\begin{definition}
		\label{definition: drc linear map of vector spaces}
Пусть $\mathcal{A}$ и
$\mathcal{B}$ - \drc векторные пространства.
Мы будем называть отображение
	\begin{equation}
\Vector{A}:\mathcal{A}\rightarrow \mathcal{B}
	\label{eq: drc linear map of vector spaces}
	\end{equation}
\AddIndex{\drc линейным отображением векторных пространств}{drc linear map of vector spaces},
если\footnote{Выражение $a\RCstar \Vector{A}(\Vector{m})$ означает выражение
$a^{\gi a}\ \Vector{A}({}_{\gi a}\Vector{m})$}
	\begin{equation}
	\label{eq: drc linear map of vector spaces, product on scalar}
\Vector{A}(a\RCstar \Vector{m})=a\RCstar \Vector{A}(\Vector{m})
	\end{equation}
для любых $a^{\gi a} \in D$, ${}_{\gi a}\Vector{m} \in \mathcal{A}$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: drc linear map of drc vector space}
Пусть $\Basis{f}=({}_{\gi a}\Vector{f},\gi{a}\in \gi{I})$
- \drc базис в векторном пространстве $\mathcal{A}$
и $\Basis{e}=({}_{\gi b}\Vector{e},\gi{b}\in \gi{J})$
- \drc базис в векторном пространстве $\mathcal{B}$.
Тогда \drc линейное отображение \eqref{eq: drc linear map of vector spaces}
векторных пространств имеет представление
	\begin{equation}
b=a\RCstar A
	\label{eq: drc linear map of vector spaces, presentation}
	\end{equation}
относительно заданных базисов. Здесь
\begin{itemize}
\item $a$ - координатная матрица вектора
$\Vector a$ относительно \drc базиса $\Basis{f}$
\item $b$ - координатная матрица вектора
$$\Vector b=\Vector{A}(\Vector a)$$ относительно \drc базиса $\Basis{e}$
\item $A$ - координатная матрица множества векторов
$(\Vector A({}_{\gi a}\Vector{f}))$ в \drc базисе $\Basis{e}$, которую мы будем называть
\AddIndex{матрицей \drc линейного отображения}{matrix of drc linear map}
относительно базисов $\Basis{f}$ и $\Basis{e}$
\end{itemize}
		\end{theorem}
		\begin{proof}
Вектор $\Vector{a}\in \mathcal{A}$ имеет разложение
	\[
\Vector{a}=a\RCstar \Vector{f}
	\]
относительно \drc базиса $\Basis{f}$.
Вектор $\Vector{b}=f(\Vector{a})\in \mathcal{B}$ имеет разложение
	\begin{equation}
\Vector{b}=b\RCstar \Vector{e}
	\label{eq: drc linear map of vector spaces, presentation, 1}
	\end{equation}
относительно \drc базиса $\Basis{e}$.

Так кaк $\Vector A$ - \drc линейное отображение, то на основании
\eqref{eq: drc linear map of vector spaces, product on scalar} следует,
что
	\begin{equation}
\Vector{b}=\Vector A(\Vector{a})=\Vector A(a\RCstar \Vector{f})
=a\RCstar \Vector A(\Vector{f})
	\label{eq: drc linear map of vector spaces, presentation, 2}
	\end{equation}
$\Vector A({}_{\gi a}\Vector{f})$ также вектор векторного пространства $\mathcal{B}$ и имеет
разложение
	\begin{equation}
\Vector A({}_{\gi a}\Vector{f})
={}_{\gi a}A\RCstar \Vector{e}
={}_{\gi a}A^{\gi b}\ {}_{\gi b}\Vector{e}
	\label{eq: drc linear map of vector spaces, presentation, 3}
	\end{equation}
относительно базиса $\Basis{e}$.
Комбинируя \eqref{eq: drc linear map of vector spaces, presentation, 2}
и \eqref{eq: drc linear map of vector spaces, presentation, 3}, мы получаем
	\begin{equation}
\Vector{b}=a\RCstar A\RCstar\Vector{e}
	\label{eq: drc linear map of vector spaces, presentation, 4}
	\end{equation}
\eqref{eq: drc linear map of vector spaces, presentation}  следует
из сравнения \eqref{eq: drc linear map of vector spaces, presentation, 1}
и \eqref{eq: drc linear map of vector spaces, presentation, 4} и
теоремы \xRef{0701.238}{theorem: expansion relative basis, vector space}.
		\end{proof}

На основании теоремы \ref{theorem: drc linear map of drc vector space}
мы идентифицируем \drc линейное отображение \eqref{eq: drc linear map of vector spaces}
векторных пространств и
матрицу его представления \eqref{eq: drc linear map of vector spaces, presentation}.

		\begin{theorem}
		\label{theorem: product of drc linear maps, vector spaces}
Пусть $$\Basis{f}=({}_{\gi a}\Vector{f},\gi{a}\in \gi{I})$$ \drc базис в векторном пространстве $\mathcal{A}$,
$$\Basis{e}=({}_{\gi b}\Vector{e},\gi{b}\in \gi{J})$$ \drc базис в векторном пространстве $\mathcal{B}$,
и $$\Basis{g}=({}_{\gi c}\Vector{g},\gi{c}\in \gi{L})$$ \drc базис в векторном пространстве $\mathcal{C}$.
Предположим, что мы имеем коммутативную диаграмму \drc линейных отображений
	\[
\xymatrix{
\mathcal{A}\ar[rr]^C\ar[dr]^A & & \mathcal{C}\\
&\mathcal{B}\ar[ur]^B &
}
	\]
где \drc линейное отображение $A$ имеет представление
	\begin{equation}
	\label{eq: product of drc linear maps, left vector spaces, A}
b=a\RCstar A
	\end{equation}
относительно заданных базисов
и \drc линейное отображение $B$ имеет представление
	\begin{equation}
	\label{eq: product of drc linear maps, left vector spaces, B}
c=b\RCstar B
	\end{equation}
относительно заданных базисов.
Тогда \drc линейное отображение $C$ имеет представление
	\begin{equation}
	\label{eq: product of drc linear maps, left vector spaces, C}
c=a\RCstar A\RCstar B
	\end{equation}
относительно заданных базисов.
		\end{theorem}
		\begin{proof}
Доказательство утверждения следует из подстановки
\eqref{eq: product of drc linear maps, left vector spaces, A}
в \eqref{eq: product of drc linear maps, left vector spaces, B}.
		\end{proof}

Записывая \drc линейное отображение в форме \RC произведения, мы можем переписать
\eqref{eq: drc linear map of vector spaces, product on scalar} в виде
	\begin{equation}
(ka)\RCstar A=k(a\RCstar A)
	\label{eq: drc linear map of vector spaces, product on scalar, image}
	\end{equation}
Утверждение теоремы
\ref{theorem: product of drc linear maps, vector spaces}
мы можем записать в виде
	\begin{equation}
(a\RCstar A)\RCstar B=a\RCstar (A\RCstar B)
	\label{eq: product of drc linear maps, vector spaces, image}
	\end{equation}
Равенства
\eqref{eq: drc linear map of vector spaces, product on scalar, image} и
\eqref{eq: product of drc linear maps, vector spaces, image}
представляют собой
\AddIndex{закон ассоциативности для \drc линейных отображений векторных пространств}
{associative law for drc linear maps of vector spaces}.
Это позволяет нам писать подобные выражения не пользуясь скобками.

Равенство \eqref{eq: drc linear map of vector spaces, presentation}
является координатной записью \drc линейного отображения.
На основе теоремы \ref{theorem: drc linear map of drc vector space}
бескоординатная запись также может быть представлена с помощью \RC произведения
	\begin{equation}
\Vector{b}=\Vector{a}\RCstar\Vector A=a\RCstar \Vector{f}\RCstar\Vector A
=a\RCstar A\RCstar \Vector{e}
	\label{eq: drc linear map of vector spaces, presentation, 5}
	\end{equation}
Если подставить равенство \eqref{eq: drc linear map of vector spaces, presentation, 5} в теорему
\ref{theorem: product of drc linear maps, vector spaces},
то мы получим цепочку равенств
	\begin{align*}
\Vector{c}&=\Vector{b}\RCstar\Vector B=b\RCstar \Vector{e}\RCstar\Vector B
=b\RCstar B\RCstar \Vector{g}\\
\Vector{c}&=\Vector{a}\RCstar\Vector A\RCstar\Vector B
=a\RCstar \Vector{f}\RCstar\Vector A\RCstar\Vector B
=a\RCstar A\RCstar B\RCstar \Vector{g}
	\end{align*}

\begin{remark}
На примере \drc линейных отображений легко видеть
насколько теорема 
\ref{theorem: decompositions of morphism of representations}
облегчает наши рассуждения при изучении морфизма \Ts представлений
$\mathfrak{F}$\Hyph алгебры.
Договоримся в рамках этого замечания
теорию \drc линейных отображений называть сокращённой теорией,
а теорию, излагаемую в этом замечании, называть расширенной теорией.

Пусть $\mathcal{A}$ - $S\RCstar$\Hyph векторное пространство.
Пусть $\mathcal{B}$ - $T\RCstar$\Hyph векторное пространство.
Пусть
	\[
\xymatrix{
f:S\ar[r]&T&\Vector{A}:\mathcal{A}\ar[r]&\mathcal{B}
}
	\]
$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств.
Пусть $\Basis{f}=({}_{\gi a}\Vector{f},\gi{a}\in \gi{I})$
- $S\RCstar$\Hyph  базис в векторном пространстве $\mathcal{A}$
и $\Basis{e}=({}_{\gi b}\Vector{e},\gi{b}\in \gi{J})$
- $T\RCstar$\Hyph базис в векторном пространстве $\mathcal{B}$.

Из определений
\ref{definition: src trc linear map of vector spaces} и
\ref{definition: morphism of representations of F algebra}
следует
	\begin{equation}
\Vector{b}=\Vector A(\Vector{a})=\Vector A(a\RCstar \Vector{f})
=f(a)\RCstar \Vector A(\Vector{f})
	\label{eq: src trc linear map of vector spaces, presentation, 1}
	\end{equation}
$\Vector A({}_{\gi a}\Vector{f})$ также вектор векторного пространства $\mathcal{B}$ и имеет
разложение
	\begin{equation}
\Vector A({}_{\gi a}\Vector{f})
={}_{\gi a}A\RCstar \Vector{e}
={}_{\gi a}A^{\gi b}\ {}_{\gi b}\Vector{e}
	\label{eq: src trc linear map of vector spaces, presentation, 2}
	\end{equation}
относительно базиса $\Basis{e}$.
Комбинируя \eqref{eq: src trc linear map of vector spaces, presentation, 1}
и \eqref{eq: src trc linear map of vector spaces, presentation, 2}, мы получаем
	\begin{equation}
\Vector{b}=f(a)\RCstar A\RCstar\Vector{e}
	\label{eq: src trc linear map of vector spaces, presentation, 3}
	\end{equation}

Пусть $\mathcal{C}$ - \drc векторное пространство.
Пусть
	\[
\xymatrix{
g:T\ar[r]&D&\Vector{B}:\mathcal{B}\ar[r]&\mathcal{C}
}
	\]
$(T\RCstar,D\RCstar)$\Hyph линейное отображение векторных пространств.
Пусть $\Basis{h}=({}_{\gi a}\Vector{h},\gi{a}\in \gi{K})$
- \drc  базис в векторном пространстве $\mathcal{C}$.
Тогда, согласно
\eqref{eq: src trc linear map of vector spaces, presentation, 3},
произведение 
$(S\RCstar,T\RCstar)$\Hyph линейного отображения $(f,\Vector{A})$ и
$(T\RCstar,D\RCstar)$\Hyph линейного отображения $(g,\Vector{B})$
имеет вид
	\begin{equation}
\Vector{c}=gf(a)\RCstar g(A)\RCstar B\RCstar\Vector{h}
	\label{eq: src trc linear map of vector spaces, presentation, 4}
	\end{equation}
Сопоставление равенств
\eqref{eq: product of drc linear maps, left vector spaces, C} и
\eqref{eq: src trc linear map of vector spaces, presentation, 4}
показывает насколько рассширеная теория линейных отображений
сложнее сокращённой теории.

При необходимости мы можем пользоваться рассширеной теорией,
но мы не получим новых результатов по сравнению со случаем
сокращённой теорией. В то же время обилие деталей
делает картину менее ясной и требует постоянного внимания.
		\qed
\end{remark}

==> Fibered.Algebra.Russian.tex <==
%auto-ignore
\def\texFiberedAlgebra{}

\ifx\PrintBook\Defined
				\chapter{Расслоенная \texorpdfstring{$\mathfrak{F}$}{F}\Hyph алгебра}
\fi

			\section{Расслоенная \texorpdfstring{$\mathfrak{F}$}{F}\Hyph алгебра}

	 \begin{definition}
n\Hyph арная
\AddIndex{операция на расслоении}{operation on bundle}
$\bundle{}pE{}$
- это расслоенный морфизм
\[
\mathcal{F}:\mathcal{E}^n\rightarrow \mathcal{E}
\]
$n$ - это \AddIndex{арность операции}{arity of operation}.
$0$-арная операция - это сечение расслоения
$\bundle{}pA{}$.
	 \qed
	 \end{definition}

Операция на расслоении может быть представлена диаграммой
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}^n\ar[rr]^\omega\arp@/^2pc/[dd]^p\arp@/_2pc/[dd]_p&&\mathcal{E}\arp[dd]^p\\
\bigodot...\bigodot\ar@{=>}@/^1pc/[rr]^\omega &&\\
M\ar[rr]^{id}&&M
}
	\]
\shorthandon{"}

		\begin{theorem}
		\label{theorem: continuity of operation}
Пусть $U$ - открытое множество базы $M$,
и на $U$ существует тривиализация расслоения $\bundle{}pE{}$.
Пусть $x\in M$.
Пусть $\omega$ - $n$\Hyph арная операция на расслоении $\bundle{}pE{}$ и
\[
\omega(p_1,...,p_n)=p
\]
в слое $E_x$.
Тогда существуют открытые множества $V\subseteq U$,
$W\subseteq E$, $W_1\subseteq E_1$, ..., $W_n\subseteq E_n$
такие, что $x\in V$, $p\in W$, $p_1\in W_1$, ..., $p_n\in W_n$,
и для любых $x'\in V$, $p'\in W\cap\omega V$ существуют
$p'_1\in W_1$, ..., $p'_n\in W_n$ такие, что
\[
\omega(p'_1,...,p'_n)=p'
\]
в слое $E_{x'}$.
%Если множества $V$, $W$ связны,
%то также связны множества $W_1$, ..., $W_n$.
		\end{theorem}
		\begin{proof}
Согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
множества вида $V\times W$, где $V$ принадлежит базису
топологии пространства $U$ и $W$ принадлежит базису топологии пространства $E$,
образуют базис топологии пространства $\mathcal{E}$. 
Аналогично множества вида $V\times W_1\times ...\times W_n$, где $V$ принадлежит базису
топологии пространства $U$ и $W_1$, ..., $W_n$ принадлежат базису топологии пространства $E$,
образуют базис топологии пространства $\mathcal{E}^n$. 

Так как отображение $\omega$ непрерывно, то для открытого множества
$V\times W$ существует открытое множество $S\subseteq \mathcal{E}^n$ такое,
что $\omega S\subseteq V\times W$.
Пусть $x'\in V$.
Выберем произвольную точку
$(x',p')\in\omega S$. Тогда существуют такие $p'_1\in E_{x'}$, ..., $p'_n\in E_{x'}$,
что
\[
\omega(p'_1,...,p'_n)=p'
\]
в слое $E_{x'}$.
Согласно сказанному выше существуют множества $R$, $R'$,
принадлежащие базису топологии пространства $U$,
и множества $T_1$, ..., $T_n$,
$T'_1$, ..., $T'_n$, принадлежащие базису топологии пространства $E$,
такие, что $x\in R$, $x'\in R'$,
$p_1\in T_1$, $p'_1\in T'_1$, ..., $p_n\in T_n$, $p'_n\in T'_n$,
$R\times T_1\times ...\times T_n\subseteq S$,
$R'\times T'_1\times ...\times T'_n\subseteq S$.
Теорема доказана, так как
$W_1=T_1\cup T'_1$, ..., $W_n=T_n\cup T'_n$
- открытые множества.
%
%Если $V$ и $W$ связны, то $V\times W$ связно согласно
%предложению 8
%(\citeBib{Bourbaki: General Topology 1}, стр. 173).
		\end{proof}

Теорема \ref{theorem: continuity of operation} говорит
о непрерывности операции $\omega$, однако эта
теорема ничего не говорит о множествах
$W_1$, ..., $W_n$. В частности, эти множества могут быть
не связными.

Если топология на слое $A$ - дискретна,
то мы можем положить $W=\{p\}$, $W_1=\{p_1\}$, ..., $W_n=\{p_n\}$.
Возникает ощущение, что в окрестности $V$ операция не зависит от
слоя. Мы будем говорить, что операция $\omega$ локально постоянна.
Однако на расслоении в целом условие постоянства может быть нарушено.
Так расслоение над окружностью со слоем группы целых чисел
может оказаться накрытием окружности $R\rightarrow S^1$
действительной прямой, определённым формулой
$p(t)=(\sin t,\cos t)$ для любого $t\in R$.

Рассмотрим альтернативную точку зрения на непрерывность операции $\omega$,
чтобы лучше понять значение непрерывности
Если мы хотим показать,
что бесконечно малые изменения операндов при движении вдоль базы
приводят к бесконечно малому изменению операции, нам надо перейти к сечениям.
Этот переход допустим,
так как операция на расслоении определена послойно.

		\begin{theorem}
		\label{theorem: operation over sections}
n-арная операция на расслоении отображает сечения в сечение.
		\end{theorem}
		\begin{proof}
Допустим $f_1$, ..., $f_n$ - сечения и отображение
	\begin{equation}
f=\omega^{\mathrm{id}}(f_1,...,f_n):M\rightarrow\mathcal{E}
	\label{eq: operation over sections}
	\end{equation}
определено равенством
	\begin{equation}
f(x)=\omega(f_1(x),...,f_n(x))
	\label{eq: operation over sections, x}
	\end{equation}
Пусть $x\in M$ и $u=f(x)$. Пусть $U$ - окрестность точки $u$ в области значений
отображения $f$.

Так как $\omega$ непрерывное отображение,
то согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
для любого значения $i$,
$1\le i\le n$ в области значений сечения $f_i$
определено открытое множество $U_i$ таким образом, что $\prod_{i=1}^nU_i$
открыто в области значений сечения $(f_1,...,f_n)$ расслоения $\mathcal{E}^n$ и
\[
\omega(\prod_{i=1}^nU_i)\subseteq U
\]

Пусть $u'\in U$.
Поскольку $f$ - отображение, существует $x'\in M$ такая, что $f(x')=u'$.
На основании равенства \eqref{eq: operation over sections, x}
существуют $u'_i\in U_i$, $p(u'_i)=x'$ такие, что
$\omega(u'_1,...,u'_n)=u'$.
%Для любого значения $i$,
%$1\le i\le n$ существует открытое множество $U_i$, содержащее точки
%$f_i(x')$ и $u'$.
Так как $f_i$ сечение, то существует открытое в $M$ множество $V_i$
такое, что $f_i(V_i)\subseteq U_i$
и $x\in V_i$, $x'\in V_i$. Следовательно, множество
\[
V=\cap_{i=1}^nV_i
\]
непусто, открыто в $M$ и $x\in V$, $x'\in V$.
Следовательно отображение $f$ непрерывно и является сечением.
		\end{proof}

Операция на расслоении может быть представлена диаграммой
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}^n\ar[rr]^\omega&&\mathcal{E}\\
\times...\times\ar@{=>}@/^1pc/[rr]^{\omega^{\mathrm{id}}} &&\\
M\ars@/^2pc/[uu]^{a_1}\ars@/_2pc/[uu]_{a_n}\ar[rr]^{id}&&M\ars[uu]
}
	\]
\shorthandon{"}

		\begin{theorem}
		\label{theorem: continuous operation over sections}
$\omega^{\mathrm{id}}$ непрерывна на $\Gamma(\mathcal{E})$.
		\end{theorem}
		\begin{proof}
Рассмотрим множество $W_{K,U}$,
где $K$ - компактное подмножество пространства $M$,
$U$ - открытое подмножество пространства $\mathcal{E}$.
Множество $U$ мы можем представить в виде $V\times E$,
где $V$ - открытое множество пространства $M$, $K\subset V$.
$\omega^{-1}(V\times E)=V\times E^n$ является открытым множеством.
Следовательно,
\begin{equation}
(\omega^{\mathrm{id}})^{-1}W_{K,V\times E}=W_{K,V\times E^n}
\label{eq: continuous operation over sections}
\end{equation}
Из \eqref{eq: continuous operation over sections}
следует непрерывность $\omega^{\mathrm{id}}$.
\end{proof}

	 \begin{definition}
Пусть $A$ является $\mathfrak{F}$\Hyph алгеброй
(\citeBib{Burris Sankappanavar}).
Мы можем перенести $\mathfrak{F}$\Hyph алгебраическую структуру со слоя
$A$ на расслоение
$\bundle{\mathcal{A}}pAM$.
Если на $\mathfrak{F}$\Hyph алгебре $A$ определена операция $\omega$
\[
a=\omega(a_1,...,a_n)
\]
то на расслоении определена операция $\omega$
\[
a(x)=\omega(a_1,...,a_n)(x)=\omega(a_1(x),...,a_n(x))
\]
Мы будем говорить, что $\bundle{}pA{}$ - это
\AddIndex{расслоенная $\mathfrak{F}$\Hyph алгебра}{fibered F-algebra}.
	 \qed
	 \end{definition}

В зависимости от структуры мы будем говорить, например, о
\AddIndex{расслоенной группе}{fibered group},
\AddIndex{расслоенном кольце}{fibered ring},
\AddIndex{векторном расслоении}{vector bundle}.

Основные свойства $\mathfrak{F}$\Hyph алгебры
сохраняются и для расслоенной $\mathfrak{F}$\Hyph алгебры. При доказательстве
соответствующих теорем, мы можем ссылаться на это утверждение.
Однако в некоторых случаях доказательство может представлять
самостоятельный интерес, так как позволяет лучше увидеть структуру
расслоенной $\mathfrak{F}$\Hyph алгебры.
Однако свойства $\mathfrak{F}$\Hyph алгебры, возникшей на множестве сечений,
могут отличаться от свойств $\mathfrak{F}$\Hyph алгебры в слое.
Например, умножение в слое может иметь обратный элемент.
В тоже время умножение сечений может не иметь обратного элемента.
Следовательно, расслоенное непрерывное поле порождает
кольцо на множестве сечений.
Это является преимуществом при изучении расслоенной алгебры.
Я хочу также обратить внимание на то, что операция в расслоении не определена для
элементов, принадлежащим разным слоям.

Точка $p\in\mathcal{A}$ имеет представление $(x,p_\alpha)$ в карте $U_\alpha$ и представление
$(x,p_\beta)$ в карте $U_\beta$.
Допустим функции перехода $g_{\epsilon\delta}$ определяют расслоение
$\mathcal{B}$ над базой $N$.
Рассмотрим карты $V_\epsilon\in N$ и $V_\delta\in N$,
$V_\epsilon\cap V_\delta\ne\emptyset$.
Точка $q\in\mathcal{B}$ имеет представление $(y,q_\epsilon)$ в карте $V_\epsilon$ и представление
$(y,q_\delta)$ в карте $V_\delta$.
Следовательно,
\[
p_\alpha=f_{\alpha\beta}(p_\beta)
\]
\[
q_\epsilon=g_{\epsilon\delta}(q_\delta)
\]
Представление соответствия при переходе от карты $U_\alpha$ к карте $U_\beta$
и от карты $V_\epsilon$ к карте $V_\delta$ изменяется согласно закону
\[
(x,y,p_\alpha,q_\epsilon)=(x,y,f_{\alpha\beta}(p_\beta),g_{\epsilon\delta}(q_\delta))
\]
Это согласуется с преобразованием
при переходе от карты $U_\alpha\times V_\epsilon$ к карте $U_\beta\times V_\delta$
в расслоении $\mathcal{A}\times\mathcal{B}$.

		\begin{theorem}
		\label{theorem: operation in two neighborhood}
Допустим функции перехода $f_{\alpha\beta}$ определяют
расслоенную $\mathfrak{F}$\Hyph алгебру
$\bundle{\mathcal{A}}pAM$ над базой $M$.
Тогда функции перехода $f_{\alpha\beta}$
являются гомоморфизмами $\mathfrak{F}$\Hyph алгебры $A$.
		\end{theorem}
		\begin{proof}
Пусть $U_\alpha\in M$ и $U_\beta\in M$,
$U_\alpha\cap U_\beta\ne\emptyset$ - окрестности,
в которых расслоенная $\mathfrak{F}$\Hyph алгебра $\bundle{}pA{}$ тривиальна.
Пусть
	\begin{equation}
a_\beta=f_{\beta\alpha}(a_\alpha)
	\label{eq: operation in two neighborhood}
	\end{equation}
функция перехода из расслоения $\bundle{}pA{}|_{U_\alpha}$ в
расслоение $\bundle{}pA{}|_{U_\beta}$.
Пусть $\omega$ - $n$\hyph арная операция и точки $e_1$, ..., $e_n$
принадлежат слою $A_x$, $x\in U_1\cap U_2$. Положим
	\begin{equation}
e=\omega(e_1,...,e_n)
	\label{eq: operation in two neighborhood, expression}
	\end{equation}

Мы можем представить точку $e\in\bundle{}pA{}|_{U_\alpha}$ в
виде $(x,e_\alpha)$ и точку $e_i\in\bundle{}pA{}|_{U_\alpha}$ в
виде $(x,e_{i\alpha})$.
Мы можем представить точку $e\in\bundle{}pA{}|_{U_\beta}$ в
виде $(x,e_\beta)$ и точку $e_i\in\bundle{}pA{}|_{U_\beta}$ в
виде $(x,e_{i\beta})$. Согласно \eqref{eq: operation in two neighborhood}
	\begin{equation}
e_\beta=f_{\beta\alpha}(e_\alpha)
	\label{eq: operation in two neighborhood, e}
	\end{equation}
	\begin{equation}
e_{i\beta}=f_{\beta\alpha}(e_{i\alpha})
	\label{eq: operation in two neighborhood, ei}
	\end{equation}
Согласно \eqref{eq: operation in two neighborhood, expression},
операция в слое $A_x$ над окрестностью $U_\beta$ имеет вид
	\begin{equation}
e_\beta=\omega(e_{1\beta},...,e_{n\beta})
	\label{eq: operation in two neighborhood, fiber}
	\end{equation}
Подставив \eqref{eq: operation in two neighborhood, e},
\eqref{eq: operation in two neighborhood, ei} в
\eqref{eq: operation in two neighborhood, fiber} мы получим
\[
f_{\beta\alpha}(e_\alpha)=\omega(f_{\beta\alpha}(e_{1\alpha}),...,f_{\beta\alpha}(e_{n\alpha}))
\]
Это доказывает, что $f_{\beta\alpha}$ является гомоморфизмом $\mathfrak{F}$\Hyph алгебры.
		\end{proof}

	\begin{definition}
	\label{definition: homomorphism of fibered F-algebras} 
Пусть $\bundle{\mathcal{A}}{p}{A}M$
и $\bundle{\mathcal{A}'}{p'}{A'}{M'}$
- две расслоенные $\mathfrak{F}$\Hyph алгебры. Мы будем называть расслоенный морфизм
\symb{f}0{homomorphism of fibered F-algebras}
\[
\ShowSymbol{homomorphism of fibered F-algebras}:\mathcal{A}\rightarrow\mathcal{A}'
\]
\AddIndex{гомоморфизмом расслоенных $\mathfrak{F}$\Hyph алгебр}
{homomorphism of fibered F-algebras},
 если соответствующее отображение слоёв
\symb{f_x}0{fiber map}
\[
\ShowSymbol{fiber map}:A_x\rightarrow A_{x'}'
\]
является гомоморфизмом $\mathfrak{F}$\Hyph алгебры $A$.
	 \qed
	 \end{definition}

	\begin{definition}
	\label{definition: isomorphism of fibered F-algebras} 
Пусть $\bundle{\mathcal{A}}{p}{A}M$
и $\bundle{\mathcal{A}'}{p'}{A'}{M'}$
- две расслоенные $\mathfrak{F}$\Hyph алгебры. Мы будем называть гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр
$f$
\AddIndex{изоморфизмом расслоенных $\mathfrak{F}$\Hyph алгебр}
{isomorphism of fibered F-algebras},
 если соответствующее отображение слоёв
\symb{f_x}0{fiber map}
\[
\ShowSymbol{fiber map}:A_x\rightarrow A_{x'}'
\]
является изоморфизмом $\mathfrak{F}$\Hyph алгебры $A$.
	 \qed
	 \end{definition}

	\begin{definition}
		\label{definition: fibered subalgebra}
Пусть $\bundle{\mathcal{A}}pAM$ -
расслоенная $\mathfrak{F}$\Hyph алгебра и $A'$ - $\mathfrak{F}$\Hyph подалгебра
$\mathfrak{F}$\Hyph алгебры $A$.
Расслоенная $\mathfrak{F}$\Hyph алгебра
$\bundle{\mathcal{A}'}p{A'}M$
является \AddIndex{расслоенной $\mathfrak{F}$\Hyph подалгеброй}{fibered F-subalgebra}
расслоенной $\mathfrak{F}$\Hyph алгебры
$\bundle{}pA{}$,
если гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр
$\mathcal{A}'\rightarrow\mathcal{A}$
является вложением слоёв.
	 \qed
	 \end{definition}

Важным обстоятельством в этом определении является гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр.
Если мы просто ограничимся фактом существования $\mathfrak{F}$\Hyph подалгебры в каждом слое,
то мы можем разрушить непрерывность.

Мы определили операцию на базе приведенного декартова произведения расслоений.
Если мы определим операцию на базе декартова произведения расслоений,
то операция будет определена для любых элементов расслоения. Однако,
если $p(a_i)=p(b_i)$, $i=1$, ..., $n$, то $p(\omega(a_1,...,a_n))=p(\omega(b_1,...,b_n))$.
Следовательно, операция определена между слоями и посредством проекции
переносится на базу. Эта конструкция не отличается от факторизации $\mathfrak{F}$\Hyph алгебры
и не создаёт новый элемент в теории расслоений. В то же время эта конструкция
довольно проблематична с точки зрения перехода между различными картами
расслоения и возможности определения операции над сечениями. 

			\section{Представление расслоенной \texorpdfstring{$\mathfrak{F}$}{F}\Hyph алгебры}
			\label{section: Representation of Fibered F-Algebra}

	\begin{definition}
	\label{definition: nonsingular transformation, bundle} 
Мы будем называть морфизм расслоений
\[
\mathcal{T}:\mathcal{E}\rightarrow\mathcal{E}
\]
\AddIndex{преобразованием расслоения}
{transformation of bundle},
если соответствующее отображение слоёв
\[
t_x:E_x\rightarrow E_x
\]
является преобразованием слоя.
	 \qed
	 \end{definition}

		\begin{theorem}
		\label{theorem: continuity of transformation}
Пусть $U$ - открытое множество базы $M$,
на котором существует тривиализация расслоения $\bundle{}pE{}$.
Пусть $t$ - преобразование расслоения $\bundle{}pE{}$.
Пусть $x\in M$ и $p'=t_x(p)$ в слое $E_x$.
Тогда для открытого множества $V\subseteq M$,
$x\in V$ и для открытого множества $W'\subseteq E$,
$p'\in W'$
существует открытое множество $W\subseteq E$, $p\in W$,
такое, что если $x_1\in V$, $p_1\in W$,
то $p'_1=t_{x_1}(p_1)\in W'$.
		\end{theorem}
		\begin{proof}
Согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
множества вида $V\times W$, где $V$ принадлежит базису
топологии пространства $U$ и $W$ принадлежит базису топологии пространства $E$,
образуют базис топологии пространства $\mathcal{E}$. 

Так как отображение $t$ непрерывно, то для открытого множества
$V\times W'$ существует открытое множество $V\times W$ такое,
что $t( V\times W)\subseteq V\times W'$. Это и есть содержание теоремы.
		\end{proof}

		\begin{theorem}
		%\label{theorem: continuity of operation}
Преобразование расслоения $\bundle{}pE{}$
отображает сечение в сечение.
		\end{theorem}
		\begin{proof}
Образ сечения $s$ при преобразовании $t$
определён из коммутативности диаграммы
	\[
\xymatrix{
\mathcal{E}\ar[rr]^t&&\mathcal{E}\\
&M\ars[ul]^s\ars[ur]_{s'}&
}
	\]
Непрерывность отображения $s'$
следует из теоремы
\ref{theorem: continuity of transformation}.
		\end{proof}

	 \begin{definition}
	\label{definition: Tstar transformation of bundle} 
Преобразование расслоения называется
\AddIndex{левосторонним преобразованием}{left-side transformation of bundle}
или
\AddIndex{\Ts преобразованием расслоения}{Tstar transformation of bundle},
если оно действует слева
\[
u'=t u
\]
Мы будем обозначать
\symb{{}^\star \mathcal{E}}1
{set of Tstar nonsingular transformations of bundle} или
\symb{{}^\star \bundle{}pE{}}1
{set of Tstar nonsingular transformations of bundle, projection}
множество невырожденных \Ts преобразований расслоения
$\bundle{}pE{}$.
	 \qed
	 \end{definition}

	 \begin{definition}
Преобразование называется
\AddIndex{правосторонним преобразованием}
{right-side transformation of bundle}
или
\AddIndex{\sT преобразованием расслоения}{starT transformation of bundle},
если оно действует справа
\[
u'= ut
\]
Мы будем обозначать
\symb{\mathcal{E}^\star}1{set of starT nonsingular transformations of bundle} или
\symb{\bundle{}pE{}^\star}1{set of starT nonsingular transformations of bundle, projection}
множество \sT невырожденных преобразований расслоения
$\bundle{}pA{}$.
	 \qed
	 \end{definition}

Мы будем обозначать
\symb{e}1{identical transformation of bundle}
тождественное преобразование расслоения.

		\begin{remark}
		\label{remark: topology on set of transformations of bundle}
Так как \Ts преобразование расслоения определено послойно, то множество ${}^\star \bundle{}pE{}$
является расслоением, изоморфным расслоению $\bundle{}p{{}^\star E}{}$.
Так как $^\star E=E^E$,
то мы можем определить в слое компактно-открытую топологию.
Это даёт возможность ответить на вопрос: насколько близки преобразования,
возникающие в соседних слоях.
Мы будем полагать, что преобразования $t(x)$, $t(x_1)$
близки, если существует открытое множество $W_{K,U}\subset E^E$,
$t(x)\in W_{K,U}$, $t(x_1)\in W_{K,U}$.
%Согласно теореме \ref{theorem: continuity of transformation}
%как только точка 
%$x_1\in M$ оказывается в окрестности точки $x\in M$,
%а точка $p_1\in E_{x_1}$ оказывается в окрестности точки $p\in E_x$
%образ отображения $t_{x_1}(p_1)$ оказывается в окрестности образа отображения $t_x(p)$.
%Однако из теории метрических пространств известно,
%что выбор окрестности $W'$ существенно зависит от выбора точки $p$.
		\qed
		\end{remark}

		\begin{definition}
		\label{definition: Tstar representation of fibered F-algebra} 
Пусть на множестве ${}^\star \bundle{}pA{}$
определена структура расслоенной $\mathfrak{F}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $\bundle{}pB{}$ является расслоенной $\mathfrak{F}$\Hyph алгеброй.
Мы будем называть гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр
	\begin{equation}
f:\bundle{}pB{}\rightarrow {}^\star \bundle{}pA{}
	\label{eq: Tstar representation of fibered F-algebra}
	\end{equation}
\AddIndex{левосторонним представлением}
{left-side representation of fibered F-algebra} или
\AddIndex{\Ts представлением расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{}pB{}$}
{Tstar representation of fibered F-algebra}.
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: starT representation of fibered F-algebra} 
Пусть на множестве $\bundle{}pA{}^\star$
определена структура расслоенной $\mathfrak{F}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $\bundle{}pB{}$ является расслоенной $\mathfrak{F}$\Hyph алгеброй.
Мы будем называть гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр
	\[
f:\bundle{}pB{}\rightarrow \bundle{}pA{}^\star
	\]
\AddIndex{правосторонним представлением}
{right-side representation of fibered F-algebra} или
\AddIndex{\sT представлением расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{}pB{}$}
{starT representation of fibered F-algebra}.
		\qed
		\end{definition}

Мы распространим на теорию расслоенных представлений соглашение,
описанное в замечании
\xRef{0701.238}{remark: left and right matrix notation}.
Мы можем записать принцип двойственности в следующей форме

		\begin{theorem}[принцип двойственности]
		\label{theorem: duality principle, fibered F-algebra representation}
Любое утверждение, справедливое для
\Ts представления расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{}pA{}$,
будет справедливо для \sT представления расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{}pA{}$.
		\end{theorem}

Существует два способа определить \Ts представление $\mathfrak{F}$\Hyph алгебры $B$ в расслоении
$\bundle{}pA{}$. Мы можем определить определить \Ts представление в слое,
либо определить \Ts представление на множестве $\Gamma(\bundle{}pA{})$.
В первом случае представление определяет одно и то же преобразование во
всех слоях. Во втором случае картина менее ограничена, однако она не даёт полной
картины разнообразия представлений в расслоении. Когда мы рассматриваем представление
расслоенной $\mathfrak{F}$\Hyph алгебры, мы сразу оговариваем, что преобразования в разных слоях
независимы. Требование непрерывной зависимости преобразования
от слоя накладывает дополнительные ограничения на \Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры.
В то же время это ограничение позволяет изучать представления расслоенных $\mathfrak{F}$\Hyph алгебр,
когда в слое определена $\mathfrak{F}$\Hyph алгебра, параметры которой
(например, структурные константы группы Ли) непрерывно зависят от слоя.

		\begin{remark}
		\label{remark: reduce details on the diagram, fibered F-algebra}
На языке диаграмм определение
\ref{definition: Tstar representation of fibered F-algebra}
означает следующее.
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}&\mathcal{E}'\arp[dr]_{p'}\ar[rr]^\varphi="C2"
& & \mathcal{E}'\arp[dl]^{p'}\\
M\ars[u]^\alpha="C1"\ar[rr]^F& & M'\\
\ar @{=>}@/_1pc/ "C1";"C2"
}
	\]
\shorthandon{"}%
Отображение $F$ - инъекция. Так как мы ожидаем, что представление расслоенной
$\mathfrak{F}$\Hyph алгебры действует в каждом слое, то мы видим, что отображение $F$ - биекция.
Не нарушая общности, мы можем положить, что $M=M'$ и отображение $F$ - тождественное
отображение. Мы будем говорить, что задано представление расслоенной $\mathfrak{F}$\Hyph алгебры
$\bundle{}pB{}$ в расслоении $\bundle{}pA{}$ над множеством $M$.
Поскольку база расслоения известна, то, чтобы не перегружать диаграмму деталями, мы будем
описывать представление с помощью диаграммы
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}&\mathcal{E}'\ar[rr]^\varphi="C2"
& & \mathcal{E}'\\
M\ars[u]^\alpha="C1"\\
\ar @{=>}@/_1pc/ "C1";"C2"
}
	\]
\shorthandon{"}%
		\qed
		\end{remark}

	\begin{theorem}
	\label{theorem: continuous dependene of transformation, fiber}
Пусть задано \Ts представление $\mathcal F$ расслоенной $\mathfrak{F}$\Hyph алгебры
$\mathcal A$ в расслоении $\bundle{}qE{}$. Тогда для открытого
множества $V\subset M$, $x\in V$ и для открытого множества
$W_{K,U}\subset E^E$, $\mathcal F(x,p)\in W_{K,U}$
существует открытое множество $W\subset A$, $p\in W$ такое,
что $x_1\in V$, $p_1\in W$ как только
$\mathcal F(x_1,p_1)\in W_{K,U}$.
		\end{theorem}
		\begin{proof}
Утверждение теоремы является следствием непрерывности отображения $\mathcal F$
и определения топологии расслоения $\mathcal A$.
		\end{proof}

	\begin{theorem}
	\label{theorem: continuous dependene of transformation, section}
Пусть задано \Ts представление $\mathcal F$ расслоенной $\mathfrak{F}$\Hyph алгебры
$\mathcal A$ в расслоении $\bundle{}qE{}$. Пусть $a$ - сечение расслоения $\mathcal A$.
Тогда для открытого
множества $V\subset M$, $x\in V$ и для открытого множества
$W_{K,U}\subset E^E$, $\mathcal F^\mathrm{id}(a)(x)\in W_{K,U}$
существует открытое множество $W\subset A$, $a(x)\in W$ такое,
что $x_1\in V$, $a(x_1)\in W$ как только
$\mathcal F^\mathrm{id}(a)(x_1)\in W_{K,U}$.
		\end{theorem}
		\begin{proof}
Следствие теоремы \ref{theorem: continuous dependene of transformation, fiber}.
		\end{proof}

	 \begin{definition}
	 \label{definition: effective representation of fibered F-algebra}
Мы будем называть \Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{}pB{}$
\AddIndex{эффективным}{effective representation of fibered F-algebra},
если отображение \eqref{eq: Tstar representation of fibered F-algebra} -
изоморфизм расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{}pB{}$ в ${}^\star \bundle{}pA{}$.
	 \qed
	 \end{definition}

		\begin{remark}
		\label{remark: notation for effective representation of fibered F-algebra}
Если \Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры
$\mathcal A$ эффективно, мы можем отождествлять
сечение расслоенной $\mathfrak{F}$\Hyph алгебры
$\mathcal A$ с его образом и записывать \Ts преобразование,
порождённое сечением $a\in\Gamma(\mathcal A)$,
в форме
\[v'=av\]
Если \sT представление расслоенной $\mathfrak{F}$\Hyph алгебры
$\mathcal A$ эффективно, мы можем отождествлять
сечение расслоенной $\mathfrak{F}$\Hyph алгебры
$\mathcal A$ с его образом и записывать \sT преобразование,
порождённое сечением $a\in\Gamma(\mathcal A)$,
в форме
\[v'=va\]
		\qed
		\end{remark}

	 \begin{definition}
	 \label{definition: transitive representation of fibered F-algebra}
Мы будем называть \Ts представление $\mathcal{F}$ расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{}pA{}$
\AddIndex{транзитивным}{transitive representation of fibered F-algebra},
если \Ts представление $F_x$ $\mathfrak{F}$\Hyph алгебры $A_x$
транзитивно для любого $x$.
Мы будем называть \Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of fibered F-algebra},
если оно транзитивно и эффективно.
	 \qed
	 \end{definition}

	 \begin{theorem}
	 \label{theorem: transitive representation of fibered F-algebra}
Допустим множество $E$ локально компактно.
\Ts представление $\mathcal{F}$ расслоенной $\mathfrak{F}$\Hyph алгебры
\[\bundle{\mathcal{A}}rAM\] в расслоении \[\bundle{\mathcal{E}}pEM\]
транзитивно,
если для любых сечений $a, b \in\Gamma(\mathcal{E})$ существует такое сечение
$g\in\Gamma(\mathcal{A})$, что
\[b=\mathcal{F}^\mathrm{id}(g)a\]
	 \end{theorem}
		\begin{proof}
Рассмотрим сечения $a, b \in\Gamma(\mathcal{E})$. В слое $E(x)$ эти сечения
определяет элементы $a(x)$, $b(x) \in E(x)$. Согласно определению
\ref{definition: transitive representation of fibered F-algebra}
%однозначно
определён $g(x)\in A(x)$ такой, что
\[b(x)=\mathcal{F}^\mathrm{id}(g(x))a(x)\]
%Наша задача - доказать, что отображения $g$ непрерывно как это
%описано в теореме \ref{theorem: continuity of transformation}.

Пусть $U_M$ - открытое множество базы $M$,
на котором существует тривиализация расслоения $\bundle{}pE{}$,
$x\in U_M$.
Пусть $W'\subseteq E$ - открытое множество,
$b(x)\in W'$.
Тогда согласно теореме \ref{theorem: continuity of transformation}
существует открытое множество $W\subseteq E$, $a(x)\in W$,
такое, что если $x_1\in U_M$, $a(x_1)\in W$,
то $b(x_1)=\mathcal{F}^\mathrm{id}(g)(x_1)(a(x_1))\in W'$.

Если замыкание $\overline W$ компактно, то положим $K=\overline W$.
Допустим замыкание $\overline W$ не компактно.
Тогда существует открытое множество $W(x)$, $a(x)\in W(x)$ такое, что
$\overline W(x)$ компактно.
Аналогично существует открытое множество $W(x_1)$, $a(x_1)\in W(x_1)$ такое, что
$\overline W(x_1)$ компактно.
Множество $V=W\cap(W(x)\cup W(x_1))$ открыто, $a(x)\in V$, $a(x_1)\in V$,
замыкание $\overline V$ компактно. Положим $K=\overline V$.

Пусть $U(x)$ - окрестность множества $g(x)K$.
Пусть $U(x_1)$ - окрестность множества $g(x_1)K$.
Положим $U=W'\cup U(x)\cup U(x_1)$.
Тогда $W_{K,U}\subset E^E$ - открытое множество,
$\mathcal{F}^\mathrm{id}(g)(x)\in W_{K,U}$,
$\mathcal{F}^\mathrm{id}(g)(x_1)\in W_{K,U}$.

Согласно теореме \ref{theorem: continuous dependene of transformation, section}
существует открытое множество $S\subset A$,
$g(x)\in S$, $g(x_1)\in S$.
		\end{proof}

		\begin{theorem}	%однотранзитивное
Допустим множество $E$ локально компактно.
\Ts представление $\mathcal{F}$ расслоенной $\mathfrak{F}$\Hyph алгебры
\[\bundle{\mathcal{A}}rAM\] в расслоении \[\bundle{\mathcal{E}}pEM\]
однотранзитивно тогда и только тогда, когда
для любых сечений $a, b \in\Gamma(\mathcal{E})$ существует одно и только одно сечение
$g\in\Gamma(\mathcal{A})$ такое, что
\[b=\mathcal{F}^\mathrm{id}(g)a\]
		\end{theorem}
		\begin{proof}
Следствие определений \ref{definition: effective representation of fibered F-algebra},
\ref{definition: transitive representation of fibered F-algebra}
и теоремы \ref{theorem: transitive representation of fibered F-algebra}.
		\end{proof}


==> Fibered.Morphism.Russian.tex <==
%auto-ignore
\def\texFiberedMorphism{}
\ifx\PrintBook\Defined
				\chapter{Расслоенный морфизм}
\fi

			\section{Расслоенный морфизм}

		\begin{theorem}
		\label{theorem: quotient bundle}
Пусть на расслоении $\bundle{\mathcal{E}}pEM$
определена расслоенная эквивалентность $\bundle{\mathcal{S}}sSM$.
Тогда существует расслоение
\[\bundle{\mathcal{E}/\mathcal{S}}t{E/S}M\]
называемое \AddIndex{фактор расслоением}{quotient bundle}
расслоения $\mathcal{E}$ по
эквивалентности $\mathcal{S}$.
Морфизм расслоений
\[
\mathrm{nat}\mathcal{S}:\mathcal{E}\rightarrow
\mathcal{E}/\mathcal{S}
\]
называется \AddIndex{расслоенным естественным морфизмом}{fibered natural morphism}
или \AddIndex{расслоенным морфизмом отождествления}{fibered identification morphism}.
		\end{theorem}
		\begin{proof}
Рассмотрим коммутативную диаграмму
\begin{equation}
\label{eq: quotient bundle}
\xymatrix{
\mathcal{E}\ar[rr]^{\mathrm{nat}\mathcal{S}}\arp[rd]_{\bundle{}pE{}}
&&\mathcal{E}/\mathcal{S}\arp[dl]^{\bundle{}t{E/S}{}}\\
&M&
}
\end{equation}
Мы определим в $\mathcal{E}/\mathcal{S}$ фактортопологию
(\citeBib{Bourbaki: General Topology 1}, стр. 39),
требуя непрерывность отображения $\mathrm{nat}\mathcal{S}$.
Согласно предложению \citeBib{Bourbaki: General Topology 1}-I.3.6
отображение $\bundle{}t{E/S}{}$ непрерывно.

Так как эквивалентность $S$ определена только между точками
одного слоя $E$, то классы эквивалентности принадлежат
одному и тому слою $E/S$ (сравни с замечанием к предложению
\citeBib{Bourbaki: General Topology 1}-I.3.6).
		\end{proof}

Пусть $f:\mathcal{A}\rightarrow\mathcal{B}$ -
расслоенный морфизм, база которого является
тождественным отображением.
Согласно определению
\xRef{0707.2246}{definition: inverse reduced fibered correspondence}
существует обратное приведенное расслоенное соответствие $f^{-1}$.
Согласно теоремам
\xRef{0707.2246}{theorem: composition of reduced fibered correspondences}
и \xRef{0707.2246}{theorem: 2 ary fibered relation}
$f^{-1}\circ f$ является $2$\Hyph арным расслоенным отношением.

		\begin{theorem}
		\label{theorem: decomposition of fibered morphism}
Расслоенное отношение $\mathcal{S}=f^{-1}\circ f$ является
расслоенной эквивалентностью на расслоении $\mathcal{A}$.
Существует разложение расслоенного морфизма $f$ в произведение
расслоенных морфизмов
	\[
f=itj
	\]
\[
\xymatrix{
\mathcal{A}/\mathcal{S}\ar[rr]^t&&f(\mathcal{A})\ar[d]^i\\
\mathcal{A}\ar[u]^j\ar[rr]^f&&\mathcal{B}
}
\]
$j=\mathrm{nat}\mathcal{S}$ - естественный гомоморфизм
	\[
\textcolor{red}{j(a)}=j(a)
	\]
$t$ - изоморфизм
	\[
\textcolor{red}{r(a)}=t(\textcolor{red}{j(a)})
	\]
$i$ - вложение
	\[
r(a)=i(\textcolor{red}{r(a)})
	\]
		\end{theorem}
		\begin{proof}
Утверждение теоремы проверяется в слое. Необходимо
также проверить, что эквивалентность непрерывно зависит от слоя.

%Пусть $x\in M$, $p\in A$, $q\in A$,
%$(x,p)\in A_x$, $(x,q)\in A_x$. Положим $R_x=f_x^{-1}\circ f_x$.
%Положим, $(p,q)\in R_x$.
%Пусть $U\subset M$ - открытое множество, $x\in U$.
%Положим $r=f_x(p)\in B$.
%Пусть $U_B\subset B$ - открытое множество, $r\in U_B$.
%Поскольку $f$ - непрерывное отображение, то существуют
%открытые множества $U_p\subset A$, $p\in U_p$, $f(U_p)\subset U_B$,
%$U_q\subset A$, $p\in U_q$, $f(U_q)\subset U_B$.
		\end{proof}

\section{Свободное \texorpdfstring{$T\star$}{T*}-представление
расслоенной группы}

Отображение $\mathrm{nat}\mathcal{S}$ не порождает расслоения,
так как разные классы эквивалентности, вообще говоря, не гомеоморфны.
Однако доказательство теоремы \ref{theorem: quotient bundle}
подсказывает конструкцию, очень напоминающую построение,
предложенное в \citeBib{Postnikov: Differential Geometry}, стр. 16 - 17.

	 \begin{definition}
	 \label{definition: fibered little group}
Рассмотрим \Ts представление $f$ расслоенной группы $\bundle{}pG{}$
в расслоении $\mathcal{M}$.
\AddIndex{Расслоенная малая группа}{fibered little group} или
\AddIndex{расслоенная группа стабилизации}{fibered stability group}
сечения $h\in \Gamma(\mathcal{M})$ -
это множество
\symb{\mathcal{G}_h}0{fibered little group}
\symb{\mathcal{G}_h}0{fibered stability group}
\[
\ShowSymbol{fibered little group}=\{g\in \Gamma(\mathcal{G}):f(g)h=h\}
\]
	 \qed
	 \end{definition}

		\begin{theorem}
		\label{theorem: fibered little group}
Рассмотрим \Ts представление $f$ расслоенной группы $\bundle{}pG{}$
в расслоении $\bundle{\mathcal{E}}rEM$.
Допустим $\mathcal{G}_h$ - расслоенная малая группа
сечения $h$. Для любого $x\in M$ слой $\mathcal{G}_{h,x}$
расслоенной малой группы
сечения $h$ является подгруппой малой группы
$G_{h(x)}$ элемента $h(x)\in E_x$.
		\end{theorem}
		\begin{proof}
Выберем сечение $g\in\Gamma(\mathcal{G}_h)$ так,
что преобразование $f(g)$ оставляет неподвижным
сечение $h\in\Gamma(\mathcal{E})$. Следовательно, преобразование
$f(h(x))$ оставляет неподвижным $h(x)\in E_x$.
		\end{proof}

	 \begin{definition}
	 \label{definition: free representation of fibered group}
Мы будем называть \Ts представление $f$ расслоенной группы $\bundle{}pG{}$
\AddIndex{свободным}{free representation of fibered group},
если для любого $x\in M$ \Ts представление $f_x$
группы $G_x$ в слое $E_x$ свободно.
	 \qed
	 \end{definition}

		\begin{theorem}	%
		\label{theorem: free representation of group}
Если определено свободное \Ts представление $f$ расслоенной группы
$\bundle{}pG{}$ в расслоении $\bundle{\mathcal{E}}rEM$,
то определено взаимно однозначное соответствие
между орбитой представления в слое и группой $G$.
Если группа $G$ - топологическая группа, то орбита представления в слое
гомеоморфна группе $G$.
		\end{theorem}
		\begin{proof}
		\end{proof}

Рассмотрим ковариантное свободное \Ts представление $f$
расслоенной группы $\bundle{}pG{}$ на расслоении $\bundle{}pE{}$.
Это \Ts представление определяет на $\bundle{}aE{}$ расслоенное отношение
эквивалентности $\mathcal{S}$, $(p,q)\in S$ если $p$ и $q$ принадлежат
общей орбите. 
Так как представление в каждом слое свободно,
все классы эквивалентности гомеоморфны группе $G$.
Следовательно, отображение $\mathrm{nat}\mathcal{S}$
является проекцией расслоения
$\bundle{\mathcal{E}}{\mathrm{nat}\mathcal{S}}G{\mathcal{E}/\mathcal{S}}$.
Мы также будем пользоваться символом $\mathcal{S}=\mathcal{G}\star$.
Мы можем представить диаграмму \eqref{eq: quotient bundle}
в виде конструкции
\[
\xymatrix{
\mathcal{E}\arp[drr]^{\bundle{}{\mathrm{nat}\mathcal{S}}G{}}
\arp[dd]^{\bundle{}pE{}}&&\\
&&\mathcal{E}/\mathcal{S}\arp[dll]^{\bundle{}t{E/S}{}}\\
M&&
}
\]
Мы будем называть расслоение $\bundle{}{\mathrm{nat}\mathcal{S}}G{}$
\AddIndex{расслоением уровня $2$}{bundle of level 2}.

\begin{example}
Рассмотрим представление группы вращений $SO(2)$ в $R^2$.
Все точки, кроме точки
$(0,0)$, имеют тривиальную малую группу.
Таким образом, на множестве $R^2\setminus \{(0,0)\}$
определено свободное представление группы $SO(2)$.

Мы не можем воспользоваться этой операцией в случае расслоения
$\bundle{}p{R^2}{}$ и представления расслоенной группы $\bundle{}t{SO(2)}{}$.
Пусть $\mathcal{S}$ - отношение расслоенной эквивалентности.
Расслоение $\bundle{}p{R^2\setminus \{(0,0)\}}{}/\bundle{}t{SO(2)}{}\star$
не является полным. В результате предельный переход может привести в
несуществующий слой. Поэтому мы предпочитаем рассматривать
расслоение $\bundle{}p{R^2}{}/\bundle{}t{SO(2)}{}\star$,
имея в виду, что слой над точкой $(x,0,0)$ - вырожден.
	 \qed
\end{example}

Мы упростим обозначения и представим полученную конструкцию в виде
\symb{p[E_2,E_1]}0{bundle of level 2}
\[
\xymatrix{
\ShowSymbol{bundle of level 2}:\mathcal{E}_2\arp[r]&
\mathcal{E}_1\arp[r]&
M
}
\]
где мы предполагаем расслоения
\begin{align*}
\bundle{\mathcal{E}_2}{p_2}{E_2}{\mathcal{E}_1}&&
\bundle{\mathcal{E}_1}{p_1}{E_1}M&
\end{align*}
Аналогичным образом мы можем рассматривать
\AddIndex{расслоение уровня $n$}{bundle of level n}
\symb{p[E_n,...,E_1]}0{bundle of level n}
\begin{equation}
\label{eq: bundle of level n}
\xymatrix{
\ShowSymbol{bundle of level n}:\mathcal{E}_n\arp[r]&\ar@{}[r]_{...}&\arp[r]&
\mathcal{E}_1\arp[r]&
M
}
\end{equation}
Последовательность расслоений \eqref{eq: bundle of level n}
мы будем называть \AddIndex{башней расслоений}{tower of bundles}.
Это определение я дал по аналогии с башней Постникова
(\citeBib{Hatcher: Algebraic Topology}).
Башня Постникова - это башня расслоений. Слой расслоения уровня $n$ - это
гомотопическая группа порядка $n$.
Подобные конструкции известны, однако я привёл определение башни
расслоений, поскольку оно естественным образом возникает из
вышеизложенного текста.

Я хочу рассмотреть ещё один пример башни расслоений, который
привлёк моё внимание (\citeBib{geometry of differential equations},
\citeBib{cohomological analysis}, часть 2).
В качестве базы выберем множество $J^0(n,m)$ $0$\Hyph джетов
отображений из $R^n$ в $R^m$. В качестве расслоения уровня $p$
выберем множество $J^p(n,m)$ $p$\Hyph джетов
отображений из $R^n$ в $R^m$.

\section{Морфизм \texorpdfstring{$T\star$}{T*}-представлений расслоенной
\texorpdfstring{$\mathfrak{F}$\Hyph }{F-}алгебры}

		\begin{definition}
		\label{definition: morphism of representations of fibered F algebra}
Рассмотрим \Ts представление
\[
\mathcal{F}:\mathcal{A}\rightarrow {}^\star\mathcal{P}
\]
расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{\mathcal{A}}aAM$ в расслоении $\bundle{\mathcal{P}}pPM$
и \Ts представление
\[
\mathcal{G}:\mathcal{B}\rightarrow {}^\star\mathcal{Q}
\]
расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{\mathcal{B}}bBM$ в расслоении $\bundle{\mathcal{Q}}qQM$.
Пара отображений
	\begin{equation}
(\begin{array}{cc}
\mathcal{C}:\mathcal{A}\rightarrow\mathcal{B},&
\mathcal{R}:\mathcal{P}\rightarrow\mathcal{Q}
\end{array})
	\label{eq: morphism of representations of fibered F algebra, definition, 1}
	\end{equation}
таких, что $\mathcal{C}$ - гомоморфизм расслоенной $\mathfrak{F}$\Hyph алгебры и
	\begin{equation}
\textcolor{blue}{\mathcal{R}(\mathcal{F}(a)m)}=\mathcal{G}(\textcolor{red}{\mathcal{C}(a)})\textcolor{blue}{\mathcal{R}(m)}
	\label{eq: morphism of representations of fibered F algebra, definition, 2}
	\end{equation}
называется
\AddIndex{морфизмом расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}
{morphism of fibered representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}
{morphism of representations of fibered F algebra}.
		\qed
		\end{definition}

Морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры можно представить в виде диаграммы
\shorthandoff{"}
\[
\xymatrix{
\mathcal P\ar[dd]_{\mathcal{F}(g)}="D1"\ar[rr]^{\mathcal R}
&&\mathcal Q\ar[dd]^{\mathcal{G}(\textcolor{red}{\mathcal C(g)})}="D2"\\
\\
\mathcal P\ar[rr]^{\mathcal R}&&\mathcal Q\\
\mathcal{A}\ar[rr]^{\mathcal C}&&\mathcal B\\
&M\ars[ul]^g="C1"\ars[ur]_{\mathcal C(g)}="C2"\\
\ar @{=>}@/^4pc/^{\mathcal{F}} "C1";"D1"
\ar @{=>}@/_4pc/_{\mathcal{G}} "C2";"D2"
}
	\]
\shorthandon{"}%
Отсюда следует, что в слое морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры
является морфизмом \Ts представлений $\mathfrak{F}$\Hyph алгебры.

		\begin{theorem}
	\label{theorem: morphism of representations of fibered F algebra}
Если \Ts представление
\[
\mathcal{F}:\mathcal{A}\rightarrow {}^\star\mathcal{P}
\]
расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{\mathcal{A}}aAM$ в расслоении $\bundle{\mathcal{P}}pPM$
однотранзитивно и \Ts представление
\[
\mathcal{G}:\mathcal{B}\rightarrow {}^\star\mathcal{Q}
\]
расслоенной $\mathfrak{F}$\Hyph алгебры $\bundle{\mathcal{B}}bBM$ в расслоении $\bundle{\mathcal{Q}}qQM$
однотранзитивно,
то существует морфизм
\[
(\begin{array}{cc}
\mathcal{C}:\mathcal{A}\rightarrow\mathcal{B},&
\mathcal{R}:\mathcal{P}\rightarrow\mathcal{Q}
\end{array})
\]
расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$.
		\end{theorem}
		\begin{proof}
Следствие теоремы \ref{theorem: morphism of representations of F algebra}
и определения \ref{definition: morphism of representations of fibered F algebra}.
		\end{proof}

		\begin{theorem}
		\label{theorem: product of morphisms of representations of fibered F algebra}
Пусть
\[
\mathcal F:\mathcal A\rightarrow {}^\star \mathcal M
\]
\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры $\mathcal A$,
\[
\mathcal G:\mathcal B\rightarrow {}^\star \mathcal N
\]
\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры $\mathcal B$,
\[
\mathcal H:\mathcal C\rightarrow {}^\star \mathcal L
\]
\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры $\mathcal C$.
Пусть определены морфизмы \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры
\[
(\begin{array}{cc}
\mathcal U:\mathcal A\rightarrow\mathcal B,&
\mathcal P:\mathcal M\rightarrow\mathcal N
\end{array})
\]
\[
(\begin{array}{cc}
\mathcal V:\mathcal B\rightarrow\mathcal C,&
\mathcal Q:\mathcal N\rightarrow\mathcal L
\end{array})
\]
Тогда определён морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры
\[
(\begin{array}{cc}
\mathcal W:\mathcal A\rightarrow\mathcal C,&
\mathcal R:\mathcal M\rightarrow\mathcal L
\end{array})
\]
где $\mathcal W=\mathcal U\mathcal V$, $\mathcal R=\mathcal P\mathcal Q$.
Мы будем называть морфизм $(\mathcal W,\mathcal R)$ расслоенных \Ts представлений из $\mathcal F$ в $\mathcal H$
\AddIndex{произведением морфизмов $(\mathcal U,\mathcal P)$ и $(\mathcal V,\mathcal Q)$
\Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}
{product of morphisms of representations of fibered F algebra}.
		\end{theorem}
		\begin{proof}
Отображение $\mathcal W$ является гомоморфизмом расслоенной $\mathfrak{F}$\Hyph
алгебры $\mathcal A$ в
расслоенную $\mathfrak{F}$\Hyph алгебру $\mathcal C$.
Нам надо показать, что пара отображений $(\mathcal W,\mathcal R)$ удовлетворяет
\eqref{eq: morphism of representations of F algebra, definition, 2}:
\begin{align*}
\textcolor{blue}{\mathcal R(\mathcal F(a)m)}&=\textcolor{blue}{\mathcal Q\mathcal P(\mathcal F(a)m)}\\
&=\textcolor{blue}{\mathcal Q(\mathcal G(\textcolor{red}{\mathcal U(a)})\textcolor{blue}{\mathcal P(m)})}\\
&=\mathcal H(\textcolor{red}{\mathcal V\mathcal U(a)})\textcolor{blue}{\mathcal Q\mathcal P(m)})\\
&=\mathcal H(\textcolor{red}{\mathcal W(a)})\textcolor{blue}{R(m)}
\end{align*}
		\end{proof}

		\begin{theorem}
		\label{theorem: decompositions of morphism of fibered representations}
Пусть
\[
\mathcal F:\mathcal A\rightarrow {}^\star \mathcal D
\]
\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры $\mathcal A$,
\[
\mathcal G:\mathcal B\rightarrow {}^\star \mathcal E
\]
\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры $\mathcal B$.
Пусть
\[
(\begin{array}{cc}
\mathcal R_1:\mathcal A\rightarrow\mathcal B,&
\mathcal R_2:\mathcal D\rightarrow\mathcal E
\end{array})
\]
морфизм расслоенных представлений из $\mathcal F$ в $\mathcal G$.
Положим
\begin{align*}
\mathcal S_1&=\mathcal R_1\mathcal R_1^{-1}&\mathcal S_2&=\mathcal R_2\mathcal R_2^{-1}
\end{align*}
Тогда для отображений $\mathcal R_1$, $\mathcal R_2$ существуют разложения,
которые можно описать диаграммой
\shorthandoff{"}
\[
\xymatrix{
&&&\mathcal D/\mathcal S_2\ar[rrr]^{\mathcal T_2}&&
&\mathcal R_2\mathcal D\ar[ddddd]^{\mathcal I_2}\\
\mathcal A/\mathcal S_1\ar[rr]^(.3){\mathcal T_1}&&\mathcal R_1\mathcal A\ar[d]^{\mathcal I_1}&&&&\\
\mathcal A\ar[rr]_(.6){\mathcal R_1}\ar[u]^{\mathcal J_1}\ar@{}[urr]_(.7){(1)}&&\mathcal B&&
\mathcal D/\mathcal S_2\ar[r]^{\mathcal T_2}\ar[luu]_{\mathcal{F}_1(\textcolor{red}{\mathcal J_1a})}="E2"&
\mathcal R_2\mathcal D\ar[d]^{\mathcal I_2}\ar[ruu]^{\mathcal{G}_1(\textcolor{red}{\mathcal R_1a})}="E3"\\
&
&&&
\mathcal D\ar[r]_{\mathcal R_2}\ar[u]^{\mathcal J_2}\ar@{}[ur]|{(2)}\ar[ddl]^{\mathcal{F}(a)}="E1"&
\mathcal E\ar[ddr]_{\mathcal{G}(\textcolor{red}{\mathcal R_1a})}="E4"\\
&&&&&&&\\
&M\ars@/^2pc/[uuul]^a="B1"\ars[uuuul]^{\mathcal J_1a}="B2"\ars[uuur]_{\mathcal R_1a}="B4"\ars[uuuur]^{\mathcal R_1a}="B3"
&&\mathcal D\ar[uuuuu]^{\mathcal J_2}\ar[rrr]_{\mathcal R_2}&&&\mathcal E\\
\ar @{=>}@/_1pc/^{\mathcal{F}} "B1";"E1"
\ar @{=>}@/^5pc/^{\mathcal{F}_1} "B2";"E2"
\ar @{=>}^{\mathcal{G}_1} "B3";"E3"
\ar @{=>}@/^1pc/^{\mathcal{G}} "B4";"E4"
}
\]
\shorthandon{"}%
\begin{itemize}
\item $s=\mathrm{ker}\ \mathcal R_1$ является конгруэнцией на $\mathcal A$.
Существует разложение гомоморфизма $\mathcal R_1$
	\begin{equation}
\mathcal R_1=\mathcal I_1\mathcal T_1\mathcal J_1
	\label{eq: morphism of representations of fibered algebra, homomorphism, 1}
	\end{equation}
$\mathcal J_1=\mathrm{nat}\ s$ - естественный гомоморфизм
	\begin{equation}
\textcolor{red}{\mathcal J_1(a)}=\mathcal J_1(a)
	\label{eq: morphism of representations of fibered algebra, homomorphism, 2}
	\end{equation}
$\mathcal T_1$ - изоморфизм
	\begin{equation}
\textcolor{red}{\mathcal R_1(a)}=\mathcal T_1(\textcolor{red}{\mathcal J_1(a)})
	\label{eq: morphism of representations of fibered algebra, homomorphism, 3}
	\end{equation}
$\mathcal I_1$ - вложение
	\begin{equation}
\mathcal R_1(a)=\mathcal I_1(\textcolor{red}{\mathcal R_1(a)})
	\label{eq: morphism of representations of fibered algebra, homomorphism, 4}
	\end{equation}
\item $\mathcal S_2=\mathrm{ker}\ \mathcal R_2$ является эквивалентностью на $\mathcal D$.
Существует разложение отображения $\mathcal R_2$
	\begin{equation}
\mathcal R_2=\mathcal I_2\mathcal T_2\mathcal J_2
	\label{eq: morphism of representations of fibered algebra, map, 1}
	\end{equation}
$\mathcal J_2=\mathrm{nat}\ \mathcal S_2$ - сюръекция
	\begin{equation}
\textcolor{blue}{\mathcal J_2(m)}=\mathcal J_2(m)
	\label{eq: morphism of representations of fibered algebra, map, 2}
	\end{equation}
$\mathcal T_2$ - биекция
	\begin{equation}
\textcolor{blue}{\mathcal R_2(m)}=\mathcal T_2(\textcolor{blue}{\mathcal J_2(m)})
	\label{eq: morphism of representations of fibered algebra, map, 3}
	\end{equation}
$\mathcal I_2$ - вложение
	\begin{equation}
\mathcal R_2(m)=\mathcal I_2(\textcolor{blue}{\mathcal R_2(m)})
	\label{eq: morphism of representations of fibered algebra, map, 4}
	\end{equation}
\item $\mathcal{F}_1$ - \Ts представление $\mathfrak{F}$\Hyph алгебры $\mathcal A/\mathcal S_1$ в $\mathcal D/\mathcal S_2$
\item $\mathcal G_1$ - \Ts представление $\mathfrak{F}$\Hyph алгебры $\mathcal R_1\mathcal A$ в $\mathcal R_2\mathcal D$
\item Существует разложение морфизма представлений
\[
(\mathcal R_1,\mathcal R_2)=(\mathcal I_1,\mathcal I_2)(\mathcal T_1,\mathcal T_2)(\mathcal J_1,\mathcal J_2)
\]
\end{itemize} 
		\end{theorem}
		\begin{proof}
Справедливость диаграмм $(1)$, $(2)$ следует из теоремы
\ref{theorem: decomposition of fibered morphism}.
Остальные утверждения теоремы проверяются в слое и следуют из теоремы
\ref{theorem: decompositions of morphism of representations}.
		\end{proof}


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index{texLinearMap}%1%1
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index{texPolymodule}%2%66
   {$(2)$\hyph векторное пространство}%
   {(2)-vector space}%
\Index{texBundleRelation}%2%122
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index{texBiring}%A%2
   {$(^{\gi a}_{\gi b})$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index{texBiring}%A%34
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index{texCalculus}%A%67
   {$A$\Hyph значная функция}%
   {A valued function}%
\SetIndexSpace%
\Index{texBiring}%C%3
   {\subs строка матрицы}%
   {c row}%
\Index{texVectorSpace}%C%5
   {\CR матричная группа}%
   {cr-matrix group}%
\Index{texBiring}%C%6
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index{texBiring}%C%7
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index{texBiring}%C%8
   {\CR степень}%
   {cr power}%
\Index{texVectorSpace}%C%9
   {\crd векторное пространство}%
   {crd vector space}%
\Index{texBiring}%C%10
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index{texVectorSpace}%D%11
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index{texVectorSpace}%D%12
   {\dcr вектор}%
   {dcr vector}%
\Index{texVectorSpace}%D%13
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index{texVectorSpace}%D%14
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index{texVectorField}%D%373
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index{texVectorSpace}%D%15
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index{texVectorSpace}%D%55
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index{texVectorSpace}%D%17
   {\drc базис в векторном пространстве}%
   {drc basis, vector space}%
\Index{texVectorSpace}%D%375
   {\drc базис в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index{texVectorField}%D%376
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index{texVectorSpace}%D%18
   {\drc вектор}%
   {drc vector}%
\Index{texVectorSpace}%D%19
   {\drc векторное пространство}%
   {drc vector space}%
\Index{texVectorSpace}%D%20
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index{texCalculus}%D%46
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index{texVectorSpace}%D%83
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index{texVectorSpace}%D%23
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index{texVectorField}%D%374
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index{texVectorSpace}%D%114
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index{texDrcMorphism}%D%25
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index{texVectorField}%D%383
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index{texVectorField}%D%365
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index{texVectorField}%D%366
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index{texVectorSpace}%D%27
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index{texVectorField}%D%372
   {$\mathcal D\star$\hyph линейная комбинация векторные полей}%
   {linear composition of vector fields}%
\Index{texVectorSpace}%D%26
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index{texVectorField}%D%370
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index{texCalculus}%D%96
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\SetIndexSpace%
\Index{texELie}%E%28
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index{texDiffEq}%E%29
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index{texRefernceFrame}%G%205
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index{texTypeBasis}%G%30
   {\Gbasis}%
   {G-basis}%
\Index{texTypeBasis}%G%31
   {\Gcoords ы}%
   {G-coordinates}%
\Index{texTypeBasis}%G%32
   {\Gspace о}%
   {GSpace}%
\Index{texBasis}%G%267
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index{texBasis}%G%270
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index{texBasis}%G%271
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index{texPolyvector}%M%361
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\Index{texPolyvector}%M%24
   {$m$\Hyph вектор}%
   {m-vector}%
\SetIndexSpace%
\Index{texPolymodule}%N%231
   {$(n)$\hyph векторное пространство}%
   {(n)-vector space}%
\Index{texBundleRelation}%N%218
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index{texBiring}%R%35
   {\sups строка матрицы}%
   {r row}%
\Index{texVectorSpace}%R%36
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index{texVectorSpace}%R%37
   {\RC главный минор}%
   {RC-major minor}%
\Index{texBiring}%R%38
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index{texVectorSpace}%R%39
   {\RC матричная группа}%
   {rc-matrix group}%
\Index{texVectorSpace}%R%40
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index{texBiring}%R%41
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index{texBiring}%R%42
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index{texVectorSpace}%R%43
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index{texBiring}%R%44
   {\RC степень}%
   {rc power}%
\Index{texVectorSpace}%R%45
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index{texVectorSpace}%R%213
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index{texBiring}%R%47
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index{texDrcMorphism}%S%314
   {$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств}%
   {src trc linear map of vector spaces}%
\Index{texVectorField}%S%381
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index{texLinearMap}%S%48
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index{texVectorSpace}%S%217
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index{texVectorSpace}%S%216
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index{texTstarRepresentation}%S%49
   {\sT сдвиг}%
   {starT shift}%
\Index{texFiberedGroup}%S%50
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\Index{texTstarMorphism}%S%160
   {\sT представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {starT representation of algebra}%
\Index{texFiberedAlgebra}%S%162
   {\sT представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {starT representation of fibered F-algebra}%
\Index{texFiberedGroup}%S%163
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index{texTstarMorphism}%S%308
   {\sT преобразование}%
   {starT transformation}%
\Index{texFiberedAlgebra}%S%167
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\SubIndex{}%71%
   {невырожденное}%
   {nonsingular transformation of bundle}%
\SetIndexSpace%
\Index{texVectorSpace}%T%51
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index{texVectorSpace}%T%52
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index{texFiberedGroup}%T%316
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\Index{texTstarMorphism}%T%386
   {\Ts преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index{texTstarRepresentation}%T%53
   {\Ts сдвиг}%
   {Tstar shift}%
\Index{texTstarMorphism}%T%301
   {\Ts представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {Tstar representation of algebra}%
\Index{texFiberedAlgebra}%T%321
   {\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {Tstar representation of fibered F-algebra}%
\Index{texTstarMorphism}%T%309
   {\Ts преобразование}%
   {Tstar transformation}%
\Index{texFiberedAlgebra}%T%327
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\SetIndexSpace%
\Index{texAffine}%А%56
   {автопараллельная кривая}%
   {auto parallel line}%
\Index{texDrcBasis}%А%57
   {активное \sT представление}%
   {active representation, vector space}%
\Index{texBasis}%А%262
   {активное представление}%
   {active representation}%
\Index{texBasis}%А%263
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index{texLie}%А%58
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\SubIndex{texLie}%9%
   {определённая слева}%
   {left defined algebra Lie}%
\SubIndex{texLie}%10%
   {определённая справа}%
   {right defined algebra Lie}%
\Index{texBiring}%А%59
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index{texFiberedGroup}%А%60
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index{texBundleRelation}%А%156
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index{texFiberedAlgebra}%А%61
   {арность операции}%
   {arity of operation}%
\Index{texBasis}%А%277
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index{texBasis}%А%275
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index{texBundle}%Б%172
   {база отображения}%
   {base of map}%
\Index{texBundleRelation}%Б%233
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index{texTypeBasis}%Б%16
   {базис}%
   {}%
\SubIndex{texTypeBasis}%1%
   {аффинный}%
   {Affine Basis}%
\SubIndex{texTypeBasis}%2%
   {ортонормальный}%
   {Orthonornal Basis}%
\SubIndex{texTypeBasis}%3%
   {центро-аффинный}%
   {Central Affine Basis}%
\Index{texBasis}%Б%266
   {базис векторного пространства}%
   {Basis}%
\Index{texLieRepresentation}%Б%62
   {базовый вектор}%
   {}%
\SubIndex{texLieRepresentation}%11%
   {\sT представления}%
   {basis vector of starT representation}%
\SubIndex{texLieRepresentation}%12%
   {\Ts представления}%
   {basis vector of Tstar representation}%
\Index{texLie}%Б%63
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index{texFiberedMorphism}%Б%351
   {башня расслоений}%
   {tower of bundles}%
\Index{texLieRepresentation}%Б%64
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index{texBiring}%Б%65
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index{texPolymodule}%В%230
   {($D_1\RCstar$, ..., $D_n\RCstar$)\hyph векторное пространство}%
   {(d1rc,dnrc)-vector space}%
\Index{texPolymodule}%В%229
   {($S\star$, $\star T$)\hyph векторное пространство}%
   {(Sstar,starT)-vector space}%
\Index{texDiffProperty}%В%69
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index{texRepresentation}%В%261
   {вектор\hyph столбец}%
   {column vector}%
\Index{texFiberedAlgebra}%В%70
   {векторное расслоение}%
   {vector bundle}%
\Index{texNewton}%В%54
   {векторный потенциал}%
   {vector potential}%
\Index{texRepresentation}%В%260
   {вектор\hyph строка}%
   {row vector}%
\Index{texDiffEq}%В%71
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index{texNewton}%В%72
   {второй закон Ньютона}%
   {Second Newton law}%
\SetIndexSpace%
\Index{texDrcBasis}%Г%73
   {геометрический объект}%
   {}%
\SubIndex{texDrcBasis}%13%
   {в координатном представлении,	определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\SubIndex{texDrcBasis}%14%
   {определённый в векторном пространстве}%
   {geometrical object, vector space}%
\SubIndex{texDrcBasis}%15%
   {типа $A$}%
   {geometrical object of type A, vector space}%
\Index{texBasis}%Г%290
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index{texBasis}%Г%288
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index{texBasis}%Г%293
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index{texRefernceFrame}%Г%74
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index{texRefernceFrame}%Г%195
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index{texFiberedAlgebra}%Г%75
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Index{texFiberedGroup}%Г%76
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index{texTypeBasis}%Г%77
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%274
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%264
   {группа симметрии}%
   {symmetry group}%
\Index{texDrcBasis}%Г%78
   {группа симметрии}%
   {SymmetryGroup}%
\Index{texTstarRepresentation}%Г%344
   {группа стабилизации}%
   {stability group}%
\Index{texGroupRing}%Г%79
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index{}%Д%283
   {движение на многообразии базисов}%
   {movement transformation}%
\Index{texBundle}%Д%331
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index{texBundle}%Д%357
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%176
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%180
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index{texCartesian}%Д%181
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index{texBundleRelation}%Д%113
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index{texBundleRelation}%Д%227
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index{texCalculus}%Д%105
   {дифференциал отображения нормированного \drc векторного пространства в нормированное тело}%
   {differential, drc vector space to skew field}%
\Index{texCalculus}%Д%99
   {дифференцируемая функция \drc векторного пространства в тело $D$ }%
   {differentiable functions, drc vector space to skew field}%
\SetIndexSpace%
\Index{texDrcMorphism}%З%312
   {закон ассоциативности для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\Index{texVectorField}%З%385
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index{texVectorSpace}%З%310
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index{texVectorField}%З%367
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index{texTstarRepresentation}%З%80
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for Tstar covariant representation}%
\Index{texLinearMap}%З%311
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index{texBundleRelation}%З%155
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index{texVectorSpace}%З%81
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index{texVectorField}%З%368
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index{texVectorSpace}%З%82
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index{texVectorField}%З%369
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\SetIndexSpace%
\Index{texFiberedAlgebra}%И%84
   {изоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {isomorphism of fibered F-algebras}%
\Index{texLinearLie}%И%85
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index{texHomotopy}%К%4
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index{texBundleRelation}%К%111
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index{texBundleRelation}%К%112
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index{texBasis}%К%278
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texBasis}%К%284
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texFiberedGroup}%К%318
   {ковариантное \Ts представление расслоенной группы}%
   {Tstar covariant representation of fibered group}%
\Index{texBundleRelation}%К%228
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index{texBundle}%К%332
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index{texFiberedGroup}%К%317
   {контравариантное \Ts представление расслоенной группы}%
   {Tstar contravariant representation of fibered group}%
\Index{texVectorSpace}%К%21
   {координатная матрица}%
   {}%
\SubIndex{texVectorSpace}%6%
   {вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\SubIndex{texVectorSpace}%7%
   {множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\SubIndex{texVectorSpace}%8%
   {множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index{texVectorField}%К%377
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index{texRefernceFrame}%К%86
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index{texVectorSpace}%К%87
   {координатное \drc векторное пространство}%
   {coordinate drc vector space}%
\Index{texVectorField}%К%380
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index{texBasis}%К%285
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index{texDrcBasis}%К%88
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%287
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texVectorSpace}%К%89
   {координатный \drc изоморфизм}%
   {coordinate drc isomorphism}%
\Index{texBasis}%К%286
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%22
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index{texVectorField}%К%378
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index{texDrcBasis}%К%90
   {координаты геометрического объекта}%
   {}%
\SubIndex{texDrcBasis}%22%
   {в векторном пространстве}%
   {coordinates of geometrical object, vector space}%
\SubIndex{texDrcBasis}%23%
   {в координатном векторном пространстве}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texBasis}%К%291
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index{texBasis}%К%289
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texVectorSpace}%К%91
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%92
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index{texDrcBasis}%К%93
   {координаты представления}%
   {coordinates of representation}%
\Index{texBasis}%К%265
   {координаты представления}%
   {coordinates of representation}%
\Index{texPolyvector}%К%360
   {косое произведение векторов}%
   {skew product of vectors}%
\Index{texAffine}%К%94
   {кривизна Картана}%
   {Cartan curvature}%
\SetIndexSpace%
\Index{texVectorSpace}%Л%98
   {левое векторное пространство}%
   {left vector space}%
\Index{texLie}%Л%101
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index{texRepresentation}%Л%247
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation}%
\Index{texRepresentation}%Л%249
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation}%
\Index{texTstarMorphism}%Л%302
   {левостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {left-side representation of algebra}%
\Index{texRepresentation}%Л%244
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index{texFiberedAlgebra}%Л%322
   {левостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {left-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%Л%164
   {левостороннее преобразование}%
   {left-side transformation}%
\Index{texFiberedAlgebra}%Л%328
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index{texLie}%Л%103
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index{texVectorSpace}%Л%214
   {левый модуль}%
   {left module}%
\Index{texTstarRepresentation}%Л%108
   {левый сдвиг}%
   {left shift}%
\Index{texRepresentation}%Л%251
   {левый сдвиг на группе}%
   {left shift, group}%
\Index{texFiberedGroup}%Л%109
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index{texRepresentation}%Л%240
   {линейное представление группы}%
   {linear representation of group}%
\Index{texBundle}%Л%116
   {лифт отображения}%
   {lift of map}%
\Index{texBundleRelation}%Л%232
   {лифт соответствия}%
   {lift of correspondence}%
\Index{texRefernceFrame}%Л%117
   {локальная система отсчёта}%
   {local reference frame}%
\Index{texBundle}%Л%363
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index{texBundle}%Л%362
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index{texTstarRepresentation}%М%343
   {малая группа}%
   {little group}%
\Index{texDrcMorphism}%М%118
   {матрица \drc линейного отображения}%
   {matrix of drc linear map}%
\Index{texVectorField}%М%384
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index{texGeomObject}%М%119
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index{texDrcBasis}%М%120
   {многообразие базисов}%
   {}%
\SubIndex{texDrcBasis}%24%
   {\drc векторного пространства}%
   {basis manifold of vector space}%
\SubIndex{texTypeBasis}%25%
   {аффинного пространства}%
   {Basis Manifold, Affine Space}%
\SubIndex{texTypeBasis}%26%
   {евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\SubIndex{texTypeBasis}%27%
   {центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texBasis}%М%276
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texBasis}%М%268
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%282
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texBasis}%М%280
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texDrcReferenceFrame}%М%123
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index{texFiberedMorphism}%М%355
   {морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of fibered F algebra}%
\Index{texTstarMorphism}%М%298
   {морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of F algebra}%
\Index{texTstarMorphism}%М%300
   {морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры в $\mathfrak{H}$\Hyph алгебре}%
   {morphism of representations of F algebra in H algebra}%
\Index{texTstarMorphism}%М%307
   {морфизм \Ts представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index{texFiberedMorphism}%М%356
   {морфизм расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index{texVectorSpace}%Н%124
   {невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index{texRepresentation}%Н%241
   {невырожденное \Ts преобразование}%
   {nonsingular transformation}%
\Index{texRefernceFrame}%Н%125
   {неголономная координата}%
   {anholonomic coordinate}%
\Index{texRefernceFrame}%Н%126
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index{texRefernceFrame}%Н%127
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index{texRefernceFrame}%Н%110
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index{texGeomObject}%Н%128
   {неметричность}%
   {nonmetricity}%
\Index{texBundleRelation}%Н%339
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index{texCalculus}%Н%97
   {норма на \drc векторном пространстве}%
   {norm on drc vector space}%
\Index{texCalculus}%Н%100
   {норма на теле}%
   {absolute value on skew field}%
\Index{texCalculus}%Н%102
   {нормированное тело}%
   {valued skew field}%
\Index{texCalculus}%Н%104
   {нормированным \drc векторное пространство}%
   {normed drc vector space}%
\SetIndexSpace%
\Index{texBundleRelation}%О%121
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index{texBundleRelation}%О%115
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index{texBiring}%О%129
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index{texRefernceFrame}%О%130
   {объект неголономности}%
   {anholonomity object}%
\Index{texTstarRepresentation}%О%131
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texRepresentation}%О%259
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texFiberedGroup}%О%132
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index{texTstarMorphism}%О%303
   {однотранзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index{texRepresentation}%О%258
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index{texFiberedAlgebra}%О%323
   {однотранзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {single transitive representation of fibered F-algebra}%
\Index{texFiberedAlgebra}%О%133
   {операция на расслоении}%
   {operation on bundle}%
\Index{texBiring}%О%134
   {определитель матрицы}%
   {determinant}%
\Index{texTstarRepresentation}%О%135
   {орбита \Ts представления группы}%
   {orbit of representation of group}%
\Index{texRepresentation}%О%253
   {орбита представления группы}%
   {orbit of representation of group}%
\Index{texFiberedGroup}%О%136
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index{texBasis}%О%281
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texTidal}%О%137
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index{texDrcReferenceFrame}%О%138
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\SetIndexSpace%
\Index{texGeomObject}%П%139
   {параллелограмм}%
   {parallelogram}%
\Index{texTstarRepresentation}%П%140
   {парные представления группы}%
   {twin representations of group}%
\Index{texFiberedGroup}%П%319
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index{texLinearMap}%П%320
   {парные представления тела}%
   {twin representations of skew field}%
\Index{texDrcBasis}%П%141
   {пассивное \Ts представление}%
   {passive representation}%
\Index{texBasis}%П%273
   {пассивное представление}%
   {passive representation}%
\Index{texBasis}%П%272
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index{texNewton}%П%142
   {первый закон Ньютона}%
   {First Newton law}%
\Index{texAffine}%П%143
   {перенос Картана}%
   {Cartan transport}%
\Index{texAffine}%П%144
   {перенос Френе}%
   {Frenet transport}%
\Index{texBundle}%П%220
   {подрасслоение}%
   {subbundle}%
\Index{texVectorField}%П%371
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index{texPolyvector}%П%358
   {поливектор}%
   {polyvector}%
\Index{texNewton}%П%146
   {потенциальная энергия}%
   {potential energy}%
\Index{texVectorSpace}%П%149
   {правое векторное пространство}%
   {right vector space}%
\Index{texLie}%П%151
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index{texRepresentation}%П%248
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation}%
\Index{texRepresentation}%П%250
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation}%
\Index{texTstarMorphism}%П%304
   {правостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {right-side representation of algebra}%
\Index{texRepresentation}%П%245
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index{texFiberedAlgebra}%П%324
   {правостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {right-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%П%242
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texRepresentation}%П%243
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texLie}%П%153
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index{texVectorSpace}%П%215
   {правый модуль}%
   {right module}%
\Index{texTstarRepresentation}%П%158
   {правый сдвиг}%
   {right shift}%
\Index{texRepresentation}%П%252
   {правый сдвиг на группе}%
   {right shift, group}%
\Index{texBundleRelation}%П%342
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index{texBundleRelation}%П%335
   {предел фильтра}%
   {limit of filter}%
\Index{texBundleRelation}%П%334
   {предельное множество фильтра}%
   {limit set of filter}%
\Index{texBasis}%П%292
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcBasis}%П%159
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texTstarRepresentation}%П%161
   {представление группы}%
   {}%
\SubIndex{texDrcBasis}%38%
   {\drc линейное \sT}%
   {linear representation of group}%
\SubIndex{texDrcBasis}%39%
   {\rcd}%
   {rcd linear representation of group}%
\SubIndex{texTstarRepresentation}%40%
   {\sT}%
   {starT representation of group}%
\SubIndex{texTstarRepresentation}%41%
   {\Ts}%
   {Tstar representation of group}%
\SubIndex{texTstarRepresentation}%42%
   {ковариантное \Ts}%
   {Tstar covariant representation of group}%
\SubIndex{texTstarRepresentation}%43%
   {контравариантное \Ts}%
   {Tstar contravariant representation of group}%
\SubIndex{texTstarRepresentation}%44%
   {эффективное}%
   {effective representation of group}%
\Index{texRepresentation}%П%246
   {представление группы}%
   {representation of group}%
\Index{texRefernceFrame}%П%165
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index{texTstarMorphism}%П%313
   {преобразование множества}%
   {transformation of set}%
\Index{texDrcBasis}%П%166
   {преобразование на многообразии базисов}%
   {}%
\SubIndex{texDrcBasis}%62%
   {активное}%
   {active transformation, vector space}%
\SubIndex{texTypeBasis}%63%
   {аффинное}%
   {affine transformation}%
\SubIndex{texTypeBasis}%64%
   {движение}%
   {movement transformation}%
\SubIndex{texTypeBasis}%65%
   {квазиаффинное}%
   {quasi affine transformation}%
\SubIndex{texTypeBasis}%66%
   {квазидвижение}%
   {quasi movement}%
\SubIndex{texDrcBasis}%67%
   {пассивное}%
   {passive transformation, vector space}%
\Index{texFiberedAlgebra}%П%329
   {преобразование расслоения}%
   {transformation of bundle}%
\Index{texCartesian}%П%221
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index{texCartesian}%П%222
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index{texBundleRelation,texBundleRelation}%П%225
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index{texBundleRelation}%П%226
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index{texBiring}%П%168
   {приводимое бикольцо}%
   {reducible biring}%
\Index{texBiring}%П%169
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index{texBiring}%П%170
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index{texDrcBasis}%П%171
   {принцип инвариантности}%
   {invariance principle}%
\Index{texBasis}%П%296
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index{texBundleRelation}%П%235
   {продолжение соответствия}%
   {extension of correspondence}%
\Index{texBundle}%П%354
   {проекция расслоения $\mathcal{E}$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index{texDrcBasis}%П%173
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index{texBasis}%П%295
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index{texTstarMorphism}%П%299
   {произведение морфизмов \Ts представлений $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of F algebra}%
\Index{texVectorField}%П%382
   {произведение морфизмов \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of fibered F algebra}%
\Index{texBundleRelation}%П%154
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index{texBundleRelation}%П%188
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\SubIndex{texVectorSpace}%74%
   {\drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\SubIndex{texVectorSpace}%75%
   {\rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index{texAffine}%П%174
   {производная Картана}%
   {Cartan derivative}%
\Index{texDiffProperty}%П%175
   {производная Ли}%
   {Lie derivative}%
\SubIndex{texDiffProperty}%72%
   {метрики}%
   {Lie derivative of metric}%
\SubIndex{texDiffProperty}%73%
   {связности}%
   {Lie derivative of connection}%
\Index{texPolyvector}%П%359
   {простой поливектор}%
   {simple polyvector}%
\Index{texTstarRepresentation}%П%352
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index{texCartesian}%П%333
   {пространство отображений}%
   {mapping space}%
\Index{texBundleRelation}%П%236
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index{texLieRepresentation}%П%177
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index{texTstarRepresentation}%П%178
   {прямое произведение \Ts представлений группы}%
   {direct product of representations of group}%
\Index{texRepresentation}%П%254
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index{texFiberedGroup}%П%179
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index{texRefernceFrame}%П%182
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index{texVectorSpace}%Р%183
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index{texFiberedMorphism}%Р%350
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index{texFiberedMorphism}%Р%349
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index{texFiberedAlgebra}%Р%184
   {расслоенная $\mathfrak{F}$\Hyph алгебра}%
   {fibered F-algebra}%
\Index{texFiberedAlgebra}%Р%186
   {расслоенная $\mathfrak{F}$\Hyph подалгебра}%
   {fibered F-subalgebra}%
\Index{texFiberedAlgebra}%Р%185
   {расслоенная группа}%
   {fibered group}%
\Index{texFiberedMorphism}%Р%347
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index{texFiberedMorphism}%Р%346
   {расслоенная малая группа}%
   {fibered little group}%
\Index{texBundleRelation}%Р%145
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index{texBundleRelation}%Р%237
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index{texBundleRelation}%Р%238
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index{texFiberedAlgebra}%Р%187
   {расслоенное кольцо}%
   {fibered ring}%
\Index{texBundle}%Р%219
   {расслоенное подмножество}%
   {fibered subset}%
\Index{texBundleRelation}%Р%224
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index{texBundleRelation}%Р%330
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index{texBundleRelation}%Р%223
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index{texFiberedMorphism}%Р%337
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index{texVectorField}%Р%379
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index{texBundle}%Р%353
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Index{texFiberedMorphism}%Р%338
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index{texBundleRelation}%Р%157
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\SetIndexSpace%
\Index{texTstarRepresentation}%С%345
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index{texFiberedMorphism}%С%348
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index{texAffine}%С%189
   {связность Картана}%
   {Cartan connection}%
\Index{texAffine}%С%190
   {символ Картана}%
   {Cartan symbol}%
\Index{texBiring}%С%191
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index{texBundleRelation}%С%148
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index{texGenRelativity}%С%192
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index{texVectorSpace}%С%193
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index{texRefernceFrame}%С%194
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index{texNewton}%С%196
   {скалярный потенциал}%
   {scalar potential}%
\Index{texTidal}%С%197
   {скорость отклонения}%
   {speed of deviation}%
\Index{texBundleRelation}%С%297
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index{texBundleRelation}%С%340
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index{texBiring}%С%198
   {стандартное представление матрицы}%
   {Standard representation}%
\Index{texDrcBasis}%С%199
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBasis}%С%269
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBundleRelation}%С%234
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index{texLinearMap}%С%200
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index{texDrcBasis}%С%201
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index{texBasis}%С%294
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index{texGeomObject}%Т%95
   {тензор кручения}%
   {torsion tensor}%
\Index{texNewton}%Т%202
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index{texLie}%Т%203
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index{texVectorSpace}%Т%204
   {тип векторного пространства}%
   {vector space type}%
\Index{texCalculus}%Т%152
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index{texCalculus}%Т%33
   {топологическое тело}%
   {topological skew field}%
\Index{texBundleRelation}%Т%147
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index{texTstarMorphism}%Т%305
   {транзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index{texRepresentation}%Т%257
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index{texFiberedAlgebra}%Т%325
   {транзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {transitive representation of fibered F-algebra}%
\SetIndexSpace%
\Index{texDiffProperty}%У%206
   {уравнение Килинга}%
   {Killing equation}%
\Index{texDiffProperty}%У%207
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index{texBiring}%У%208
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index{texFiberedMorphism}%Ф%336
   {фактор расслоение}%
   {quotient bundle}%
\Index{texBundleRelation}%Ф%341
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index{texGeomObject}%Ф%239
   {форма кручение}%
   {torsion form}%
\Index{texCalculus}%Ф%150
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index{texCalculus}%Ф%68
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index{texBasis}%Ц%279
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index{texCalculus}%Ч%106
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, skew field}%
\Index{texCalculus}%Ч%107
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, drc vector space}%
\SetIndexSpace%
\Index{texVectorField}%Э%364
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered skew field}%
\Index{texAffine}%Э%209
   {экстремальная кривая}%
   {extreme line}%
\Index{texTstarMorphism}%Э%306
   {эффективное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index{texRepresentation}%Э%256
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texFiberedAlgebra}%Э%326
   {эффективное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {effective representation of fibered F-algebra}%
\Index{texFiberedGroup}%Э%315
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index{texVectorSpace}%Э%210
   {эффективное представление тела}%
   {effective representation of skew field}%
\SetIndexSpace%
\Index{texTstarRepresentation}%Я%211
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of representation of group}%
\Index{texRepresentation}%Я%255
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index{texFiberedGroup}%Я%212
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%

\CloseIndex


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb{texBiring}%
   {минор}%
   {A from b a}%
\Symb{texBiring}%
   {минор}%
   {A from columns T}%
\Symb{texBiring}%
   {минор}%
   {A from rows S}%
\Symb{texBiring}%
   {минор}%
   {A without column a}%
\Symb{texBiring}%
   {минор}%
   {A without columns T}%
\Symb{texBiring}%
   {минор}%
   {A without row b}%
\Symb{texBiring}%
   {минор}%
   {A without rows S}%
\Symb{texPolymodule}%
   {активное преобразование}%
   {active transformation}%
\Symb{texTypeBasis}%
   {аффинное пространство}%
   {affine space}%
\Symb{texBasis}%
   {аффинное пространство}%
   {An}%
\Symb{texBiring}%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb{texBiring}%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb{texBiring}%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb{texBiring}%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb{texVectorSpace}%
   {\dcr вектор}%
   {dcr vector}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb{texVectorSpace}%
   {\drc вектор}%
   {drc vector}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb{texPolymodule}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texBiring}%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb{texBiring}%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb{texBiring}%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb{texBiring}%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb{texBiring}%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb{texTstarRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texPolyvector}%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb{texFiberedGroup}%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb{texTstarRepresentation}%
   {левый сдвиг}%
   {Tstar shift}%
\Symb{texFiberedGroup}%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb{texRefernceFrame}%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb{texRefernceFrame}%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%
\Symb{texBasis}%
   {многообразие базисов аффинного пространства}%
   {BAn}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства $\mathcal{V}$}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb{texBasis}%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb{texBundle}%
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Symb{texBundle}%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb{texTypeBasis}%
   {многообразие базисов аффинного пространства}%
   {FAn}%
\Symb{texTypeBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb{texTypeBasis}%
   {многообразие базисов евклидова пространства}%
   {FEn}%

\SetIndexSpace%
\Symb{texBasis}%
   {центро-аффинное пространство}%
   {CAn}%
\Symb{texTypeBasis}%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb{texLie}%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb{texLie}%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb{texVectorField}%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb{texVectorSpace}%
   {координатное \drc векторное пространство}%
   {coordinate drc vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to drc vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to skew field}%
\Symb{texVectorSpace}%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace D}%
\Symb{texAffine}%
   {производная}%
   {overline D}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, skew field}%
\Symb{texVectorSpace}%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb{texTidal}%
   {скорость отклонения}%
   {speed of deviation}%
\Symb{texVectorSpace}%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%
\Symb{texTypeBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texTypeBasis}%
   {базис}%
   {basis}%
\Symb{texBasis}%
   {базис векторного пространства}%
   {Basis e}%
\Symb{texBasis}%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb{texVectorSpace}%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb{texPolymodule}%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb{texCartesian}%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb{texBasis}%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb{texVectorField}%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb{texRefernceFrame}%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb{texBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texTypeBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texTypeBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texFiberedAlgebra}%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb{texBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb{texBasis}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texRefernceFrame}%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb{texRefernceFrame}%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb{texBasis}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb{texVectorSpace}%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb{texDiffEq}%
   {центро-аффинный}%
   {Central Affine Basis}%
\Symb{texBundle}%
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Symb{texBundleRelation}%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb{texFiberedAlgebra}%
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb{texCartesian}%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb{texTstarRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texTypeBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texRefernceFrame}%
   {система отсчёта}%
   {reference frame}%
\Symb{texRefernceFrame}%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb{texPolymodule}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texPolymodule}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb{texFiberedMorphism}%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb{texFiberedMorphism}%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb{texLie}%
   {алгебра Ли группы Ли}%
   {g}%
\Symb{texLie}%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb{texTypeBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texLie}%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb{texBasis}%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb{texTstarRepresentation}%
   {малая группа элемента $x$}%
   {little group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective starT covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective starT covariant representation of group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective Tstar covariant representation of group}%
\Symb{texVectorSpace}%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb{texTstarRepresentation}%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%
\Symb{texBiring}%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb{texLinearMap}%
   {\rcd векторное пространство \drc линейных отображений}%
   {rcd vector space of drc linear maps}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb{texLinearLie}%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%
\Symb{texRepresentation}%
   {левый сдвиг}%
   {left shift}%
\Symb{texDiffProperty}%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb{texDiffProperty}%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb{texBundleRelation}%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb{texBasis}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texRepresentation}%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texTstarMorphism}%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb{texTstarMorphism}%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb{texTstarRepresentation}%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%
\Symb{texBasis}%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb{texBasis}%
   {геометрический объект}%
   {geometrical object, vector space}%
\Symb{texFiberedGroup}%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb{texRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%
\Symb{texBundle}%
   {расслоение}%
   {bundle}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb{texCartesian}%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%
\Symb{texBasis}%
   {активное преобразование}%
   {active transformation}%
\Symb{texAffine}%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb{texVectorSpace}%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb{texAffine}%
   {кривизна}%
   {GLn curvature_overline}%
\Symb{texVectorSpace}%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb{texRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texRepresentation}%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb{texVectorSpace}%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%
\Symb{texLie}%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%
\Symb{texBasis}%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb{texBasis}%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb{texVectorSpace}%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb{texLinearMap}%
   {($S$, $T$)\hyph бимодуль}%
   {R S bimodule}%
\Symb{texVectorSpace}%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb{texVectorSpace}%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb{texBasis}%
   {векторное пространство}%
   {V}%

\SetIndexSpace%
\Symb{texPolymodule}%
   {геометрический объект в координатном представлении,		определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\Symb{texPolymodule}%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%

\SetIndexSpace%
\Symb{texTidal}%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb{texRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texTstarMorphism}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texBasis}%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb{texBiring}%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb{texAffine}%
   {символ Картана}%
   {Cartan symbol}%
\Symb{texAffine}%
   {связность}%
   {conection overline}%
\Symb{texRefernceFrame}%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb{texAffine}%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb{texBundle}%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%
\Symb{texLie}%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb{texLie}%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, skew field}%
\Symb{texRefernceFrame}%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%

\SetIndexSpace%
\Symb{texLie}%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%
\Symb{texBundle}%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb{texBundle}%
   {подрасслоение}%
   {subbundle}%

\CloseIndex


==> Tstar.Morphism.Russian.tex <==
%auto-ignore
\def\texTstarMorphism{}
\ifx\PrintBook\undefined
\title{Морфизм \texorpdfstring{\Ts}{T*-}представлений}
\pdfbookmark[1]{Морфизм T*-представлений}{TitleRussian}
\begin{abstract}
Значимость теорем об изоморфизмах состоит в том,
что они позволяют отождествлять различные математические
объекты, имеющие нечто общее с точки зрения некоторой модели.
Эта статья изучает морфизмы \Ts представлений $\mathfrak{F}$\Hyph алгебры
и морфизмы \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры.
\end{abstract}

\maketitle

Эта статья возникла на пересечении двух исследований, которые я
веду параллельно. Первая половина статьи посвящена
морфизмам \Ts представлений $\mathfrak{F}$\Hyph алгебры.
Вторая половина статьи рассматривает
морфизмы \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры.
Рассматриваемые конструкции возникли в результате изучения
\drc линейных отображений, которые являются
морфизмами \Ts представлений тела в абелевой группе.
Поэтому я использую \drc линейные отображения
в качестве иллюстрации излагаемой теории.
\fi

			\section{Представление \texorpdfstring{$\mathfrak{F}$\Hyph }{F-}алгебры}
			\label{section: Representation of F-Algebra}

	\begin{definition}
Мы будем называть отображение
\[
t:M\rightarrow M
\]
\AddIndex{преобразованием множества}{transformation of set} $M$.
	 \qed
	 \end{definition}

	 \begin{definition}
Преобразование называется
\AddIndex{левосторонним преобразованием}{left-side transformation}
или
\AddIndex{\Ts преобразованием}{Tstar transformation},
если оно действует слева
\[
u'=t u
\]
Мы будем обозначать
\symb{{}^\star M}1{set of Tstar transformations}
множество \Ts преобразований множества $M$.

Если на множестве $M$ определена структура $\mathfrak{H}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}),
то множество ${}^\star M$ состоит из \Ts преобразований, являющихся гомоморфизмами
$\mathfrak{H}$\Hyph алгебры.
	 \qed
	 \end{definition}

	 \begin{definition}
Преобразование называется
\AddIndex{правосторонним преобразованием}{right-side transformation}
или
\AddIndex{\sT преобразованием}{starT transformation},
если оно действует справа
\[
u'= ut
\]
Мы будем обозначать
\symb{M^\star}1{set of starT transformations}
множество \sT преобразований множества $M$.

Если на множестве $M$ определена структура $\mathfrak{H}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}),
то множество $M^\star$ состоит из \sT преобразований, являющихся гомоморфизмами
$\mathfrak{H}$\Hyph алгебры.
	 \qed
	 \end{definition}

Мы будем обозначать
\symb{\delta}1{identical transformation}
тождественное преобразование.

		\begin{definition}
		\label{definition: Tstar representation of algebra} 
Пусть на множестве ${}^\star M$ определена структура $\mathfrak{F}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $A$ является $\mathfrak{F}$\Hyph алгеброй.
Мы будем называть гомоморфизм
	\begin{equation}
f:A\rightarrow {}^\star M
	\label{eq: Tstar representation of algebra}
	\end{equation}
\AddIndex{левосторонним}
{left-side representation of algebra} или
\AddIndex{\Ts представлением $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}
{Tstar representation of algebra}
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: starT representation of algebra} 
Пусть на множестве $M^\star$ определена структура $\mathfrak{F}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $A$ является $\mathfrak{F}$\Hyph алгеброй.
Мы будем называть гомоморфизм
	\[
f:A\rightarrow M^\star
	\]
\AddIndex{правосторонним}
{right-side representation of algebra} или
\AddIndex{\sT представлением $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}
{starT representation of algebra}
		\qed
		\end{definition}

Мы распространим на теорию представлений соглашение,
описанное в замечании
\xRef{0701.238}{remark: left and right matrix notation}.
Мы можем записать принцип двойственности в следующей форме

		\begin{theorem}[принцип двойственности]
		\label{theorem: duality principle, algebra representation}
Любое утверждение, справедливое для
\Ts представления $\mathfrak{F}$\Hyph алгебры $A$,
будет справедливо для \sT представления $\mathfrak{F}$\Hyph алгебры $A$.
		\end{theorem}

Диаграмма
\[
\xymatrix{
M\ar[rr]^{f(a)}&&M\\
&A\ar@{=>}[u]^f&
}
\]
означает, что мы рассматриваем представление $\mathfrak{F}$\Hyph алгебры $A$.
Отображение $f(a)$ является образом $a\in A$.

	 \begin{definition}
	 \label{definition: effective representation of algebra}
Мы будем называть \Ts представление $\mathfrak{F}$\Hyph алгебры $A$
\AddIndex{эффективным}{effective representation of algebra},
если отображение \eqref{eq: Tstar representation of algebra} -
изоморфизм $\mathfrak{F}$\Hyph алгебры $A$ в ${}^\star M$.
	 \qed
	 \end{definition}

		\begin{remark}
		\label{remark: notation for effective representation of algebra}
Если \Ts представление $\mathfrak{F}$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\mathfrak{F}$\Hyph алгебры с его образом и записывать \Ts преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=av\]
Если \sT представление $\mathfrak{F}$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\mathfrak{F}$\Hyph алгебры с его образом и записывать \sT преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=va\]
		\qed
		\end{remark}

	 \begin{definition}
	 \label{definition: transitive representation of algebra}
Мы будем называть \Ts представление $\mathfrak{F}$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)b\]
Мы будем называть \Ts представление $\mathfrak{F}$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и эффективно.
	 \qed
	 \end{definition}

		\begin{theorem}	%однотранзитивное
\Ts представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in A$ такое, что $a=f(g)b$
		\end{theorem}
		\begin{proof}
Следствие определений \ref{definition: effective representation of algebra}
и \ref{definition: transitive representation of algebra}.
		\end{proof}

Если на множестве $M$ определена дополнительная структура,
мы предъявляем к представлению $\mathfrak{F}$\Hyph алгебры
дополнительные требования.

Пусть на множестве $M$ определена структура алгебры типа $\mathfrak{H}$.
Тогда мы полагаем, что \Ts преобразование
	\[
u'=f(a)u
	\]
является автоморфизмом алгебры типа $\mathfrak{H}$
либо отражает симметрии алгебры типа $\mathfrak{H}$.

Если на множестве $M$ определено понятие непрерывности,
то мы полагаем, что \Ts преобразование
	\[
u'=f(a)u
	\]
непрерывно по $u$
и, следовательно,
\[\left|\frac { \partial u'} {\partial u}\right|\neq 0\]

\section{Морфизм \texorpdfstring{$T\star$}{T*}-представлений
\texorpdfstring{$\mathfrak{F}$\Hyph }{F-}алгебры}

		\begin{theorem}
Пусть $A$ и $B$ - $\mathfrak{F}$\Hyph алгебры.
\Ts представление $\mathfrak{F}$\Hyph алгебры $B$
	\[
f:B\rightarrow {}^\star M
	\]
и гомоморфизм $\mathfrak{F}$\Hyph алгебры
	\begin{equation}
h:A\rightarrow B
	\label{eq: homomorphism of algebra F}
	\end{equation}
определяют \Ts представление $\mathfrak{F}$\Hyph алгебры $A$
	\[
\xymatrix{
A\ar[dr]^h\ar[rr]^f&&{}^\star M\\
&B\ar[ur]^g&
}
	\]
		\end{theorem}
		\begin{proof}
Отображение $h$ является гомоморфизмом $\mathfrak{F}$\Hyph алгебры $A$ в
$\mathfrak{F}$\Hyph алгебру ${}^\star M$,
так как отображение $f$ является гомоморфизмом $\mathfrak{F}$\Hyph алгебры $B$ в
$\mathfrak{F}$\Hyph алгебру ${}^\star M$.
		\end{proof}

Если мы изучаем представление $\mathfrak{F}$\Hyph алгебры
в множествах $M$ и $N$, то нас интересуют отображения
из $M$ в $N$, сохраняющие структуру представления.

		\begin{definition}
		\label{definition: morphism of representations of F algebra}
Рассмотрим \Ts представление
\[
f:A\rightarrow {}^\star M
\]
$\mathfrak{F}$\Hyph алгебры $A$ в $M$
и \Ts представление
\[
g:B\rightarrow {}^\star N
\]
$\mathfrak{F}$\Hyph алгебры $B$ в $N$.
Пара отображений $(r,R)$
	\begin{equation}
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
	\label{eq: morphism of representations of F algebra, definition, 1}
	\end{equation}
таких, что $r$ - гомоморфизм $\mathfrak{F}$\Hyph алгебры и
	\begin{equation}
\textcolor{blue}{R(f(a)m)}=g(\textcolor{red}{r(a)})\textcolor{blue}{R(m)}
	\label{eq: morphism of representations of F algebra, definition, 2}
	\end{equation}
называется
\AddIndex{морфизмом \Ts представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры}
{morphism of representations of F algebra}.
		\qed
		\end{definition}

		\begin{remark}
Рассмотрим морфизм \Ts представлений
\eqref{eq: morphism of representations of F algebra, definition, 1}.
Мы можем обозначать элементы множества $B$, пользуясь буквой по образцу $b\in B$.
Но если мы хотим показать, что $b$ является образом элемента $a\in A$,
мы будем пользоваться обозначением $\textcolor{red}{r(a)}$.
Таким образом, равенство
\[
\textcolor{red}{r(a)}=r(a)
\]
означает, что $\textcolor{red}{f(a)}$ (в левой части равенства)
является образом $a\in A$ (в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $N$ в виде $\textcolor{blue}{R(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\mathfrak{F}$\Hyph алгебр
и отображениями между множествами, где определены
соответствующие \Ts представления.

Мы можем интерпретировать
\eqref{eq: morphism of representations of F algebra, definition, 2}
двумя способами
\begin{itemize}
\item Пусть \Ts преобразование $f(a)$ отображает $m\in M$ в $f(a)m$.
Тогда \Ts преобразование $g(\textcolor{red}{r(a)})$ отображает
$\textcolor{blue}{R(m)}\in N$ в $\textcolor{blue}{R(f(a)m)}$.
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\[
\xymatrix{
&M\ar[dd]_(.3){f(a)}\ar[rr]^R&&N\ar[dd]^(.3){g(\textcolor{red}{r(a)})}\\
&\ar @{}[rr]|{(1)}&&\\
&M\ar[rr]^R&&N\\
A\ar[rr]^r\ar@{=>}[uur]^(.3)f&&B\ar@{=>}[uur]^(.3)g
}
\]
Из \eqref{eq: morphism of representations of F algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
		\qed
		\end{remark}

		\begin{theorem}
Рассмотрим \Ts представление
\[
f:A\rightarrow {}^\star M
\]
$\mathfrak{F}$\Hyph алгебры $A$ 
и \Ts представление
\[
g:B\rightarrow {}^\star N
\]
$\mathfrak{F}$\Hyph алгебры $B$.
Морфизм
\[
\xymatrix{
h:A\ar[r]&B&H:M\ar[r]&N
}
\]
\Ts представлений из $f$ в $g$
удовлетворяет соотношению
	\begin{equation}
H(\omega(f(a_1),...,f(a_n))m)=\omega(g(h(a_1)),...,g(h(a_n)))H(m)
	\label{eq: morphism of representations of F algebra, 1}
	\end{equation}
для произвольной $n$-арной операции $\omega$ $\mathfrak{F}$\Hyph алгебры.
		\end{theorem}
		\begin{proof}
Так как $f$ - гомоморфизм, мы имеем
	\begin{equation}
H(\omega(f(a_1),...,f(a_n))m)=H(f(\omega(a_1,...,a_n))m)
	\label{eq: morphism of representations of F algebra, 2}
	\end{equation}
Из \eqref{eq: morphism of representations of F algebra, definition, 2} и
\eqref{eq: morphism of representations of F algebra, 2} следует
	\begin{equation}
H(\omega(f(a_1),...,f(a_n))m)=g(h(\omega(a_1,...,a_n)))H(m)
	\label{eq: morphism of representations of F algebra, 3}
	\end{equation}
Так как $h$ - гомоморфизм, из
\eqref{eq: morphism of representations of F algebra, 3} следует
	\begin{equation}
H(\omega(f(a_1),...,f(a_n))m)=g(\omega(h(a_1),...,h(a_n)))H(m)
	\label{eq: morphism of representations of F algebra, 4}
	\end{equation}
Так как $g$ - гомоморфизм, из
\eqref{eq: morphism of representations of F algebra, 4} следует
\eqref{eq: morphism of representations of F algebra, 1}.
		\end{proof}

		\begin{theorem}
	\label{theorem: morphism of representations of F algebra}
Если \Ts представление
\[
f:A\rightarrow {}^\star M
\]
$\mathfrak{F}$\Hyph алгебры $A$ однотранзитивно и \Ts представление
\[
g:B\rightarrow {}^\star N
\]
$\mathfrak{F}$\Hyph алгебры $B$ однотранзитивно,
то существует морфизм
\[
\xymatrix{
p:A\ar[r]&B&P:M\ar[r]&N
}
\]
\Ts представлений из $f$ в $g$.
		\end{theorem}
		\begin{proof}
Выберем гомоморфизм $h$.
Выберем элемент $m\in M$
и элемент $n\in N$. 
Чтобы построить отображение $H$, рассмотрим следующую диаграмму
\[
\xymatrix{
&M\ar[dd]^(.3)a\ar[rr]^H&&N\ar[dd]_(.3){p(a)}\\
&\ar @{}[rr]|{(1)}&&\\
&M\ar[rr]^H&&N\\
A\ar[rr]^p\ar@{=>}[uur]^(.3)f&&B\ar@{=>}[uur]^(.3)g
}
\]
Из коммутативности диаграммы $(1)$ следует
\[
H(am)=p(a)H(m)
\]
Для произвольного $m'\in M$ однозначно определён $a\in A$ такой,
что $m'=am$. Следовательно, мы построили отображении $H$,
которое удовлетворяет равенству
\eqref{eq: morphism of representations of F algebra, definition, 2}.
		\end{proof}

		\begin{theorem}
Если \Ts представление
\[
f:A\rightarrow {}^\star M
\]
$\mathfrak{F}$\Hyph алгебры $A$ однотранзитивно,
то для любого автоморфизма $\mathfrak{F}$\Hyph алгебры $A$ существует морфизм
\[
\xymatrix{
p:A\ar[r]&A&P:M\ar[r]&M
}
\]
\Ts представлений из $f$ в $f$.
		\end{theorem}
		\begin{proof}
Рассмотрим следующую диаграмму
\[
\xymatrix{
&M\ar[dd]^(.3)a\ar[rr]^H&&N\ar[dd]_(.3){p(a)}\\
&\ar @{}[rr]|{(1)}&&\\
&M\ar[rr]^H&&N\\
A\ar[rr]^p\ar@{=>}[uur]^(.3)f&&A\ar@{=>}[uur]^(.3)g
}
\]
Утверждение теоремы является следствием теоремы
\ref{theorem: morphism of representations of F algebra}.
		\end{proof}

		\begin{theorem}
		\label{theorem: product of morphisms of representations of F algebra}
Пусть
\[
f:A\rightarrow {}^\star M
\]
\Ts представление $\mathfrak{F}$\Hyph алгебры $A$,
\[
g:B\rightarrow {}^\star N
\]
\Ts представление $\mathfrak{F}$\Hyph алгебры $B$,
\[
h:C\rightarrow {}^\star L
\]
\Ts представление $\mathfrak{F}$\Hyph алгебры $C$.
Пусть определены морфизмы \Ts представлений $\mathfrak{F}$\Hyph алгебры
\[
\xymatrix{
p:A\ar[r]&B&P:M\ar[r]&N
}
\]
\[
\xymatrix{
q:B\ar[r]&C&Q:N\ar[r]&L
}
\]
Тогда определён морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры
\[
\xymatrix{
r:A\ar[r]&C&R:M\ar[r]&L
}
\]
где $r=qp$, $R=QP$.
Мы будем называть морфизм $(r,R)$ \Ts представлений из $f$ в $h$
\AddIndex{произведением морфизмов $(p,P)$ и $(q,Q)$
\Ts представлений $\mathfrak{F}$\Hyph алгебры}
{product of morphisms of representations of F algebra}.
		\end{theorem}
		\begin{proof}
Отображение $r$ является гомоморфизмом $\mathfrak{F}$\Hyph алгебры $A$ в
$\mathfrak{F}$\Hyph алгебру $C$.
Нам надо показать, что пара отображений $(r,R)$ удовлетворяет
\eqref{eq: morphism of representations of F algebra, definition, 2}:
\begin{align*}
\textcolor{blue}{R(f(a)m)}&=\textcolor{blue}{QP(f(a)m)}\\
&=\textcolor{blue}{Q(g(\textcolor{red}{p(a)})\textcolor{blue}{P(m)})}\\
&=h(\textcolor{red}{qp(a)})\textcolor{blue}{QP(m)})\\
&=h(\textcolor{red}{r(a)})\textcolor{blue}{R(m)}
\end{align*}
		\end{proof}

Представления и морфизмы представлений $\mathfrak{F}$\Hyph алгебры
порождают категорию представлений $\mathfrak{F}$\Hyph алгебры.

\begin{definition}
Пусть на множестве $M$ определена эквивалентность $S$.
\Ts преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия $m_1\equiv m_2(\mathrm{mod} S)$ следует
$fm_1\equiv fm_2(\mathrm{mod} S)$.
\end{definition}

\begin{theorem}
\label{theorem: transformation correlated with equivalence}
Пусть на множестве $M$ определена эквивалентность $S$.
Пусть на множестве ${}^\star M$ определена $\mathfrak{F}$\Hyph алгебра.
Если \Ts преобразования согласованны с эквивалентностью $S$,
то мы можем определить структуру $\mathfrak{F}$\Hyph алгебры
на множестве ${}^\star(M/S)$.
\end{theorem}
\begin{proof}
Пусть $h=\mathrm{nat}\ S$. Если $m_1\equiv m_2(\mathrm{mod} S)$,
то $h(m_1)=h(m_2)$. Поскольку
$f\in{}^\star M$ согласованно с эквивалентностью $S$,
то $h(f(m_1))=h(f(m_2))$. Это позволяет определить
\Ts преобразование $F$ согласно правилу
\[
F([m])=h(f(m))
\]

Пусть $\omega$ - n\Hyph арная операция $\mathfrak{F}$\Hyph алгебры.
Пусть $f_1$, ..., $f_n\in{}^\star M$ и
\begin{align*}
F_1([m])&=h(f_1(m))&&...&F_n([m])&=h(f_n(m))
\end{align*}
Мы определим операцию на множестве ${}^\star(M/S)$ по правилу
\[
\omega(F_1,...,F_n)[m]=h(\omega(f_1,...,f_n)m)
\]
Это определение корректно, так как
$\omega(f_1,...,f_n)\in{}^\star M$ и согласованно с эквивалентностью $S$.
\end{proof}

		\begin{theorem}
		\label{theorem: decompositions of morphism of representations}
Пусть
\[
f:A\rightarrow {}^\star M
\]
\Ts представление $\mathfrak{F}$\Hyph алгебры $A$,
\[
g:B\rightarrow {}^\star N
\]
\Ts представление $\mathfrak{F}$\Hyph алгебры $B$.
Пусть
\[
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
\]
морфизм представлений из $f$ в $g$.
Положим
\begin{align*}
s&=rr^{-1}&S&=RR^{-1}
\end{align*}
Тогда для отображений $r$, $R$ существуют разложения,
которые можно описать диаграммой
\[
\xymatrix{
&&M/S\ar[rrrrr]^T\ar@{}[drrrrr]|{(5)}&&\ar@{}[dddddll]|{(4)}&
\ar@{}[dddddrr]|{(6)}&&RM\ar[ddddd]^I\\
&&&&&&&\\
A/s\ar[r]^t\ar@/^2pc/@{=>}[urrr]^F&
rA\ar[d]^i\ar@{=>}[urrrrr]^(.4)G&&&
M/S\ar[r]^T\ar[lluu]_{F(\textcolor{red}{j(a)})}&
RM\ar[d]^I\ar[rruu]_{G(\textcolor{red}{r(a)})}\\
A\ar[r]_r\ar[u]^j\ar@{}[ur]|{(1)}\ar@/_2pc/@{=>}[drrr]^f&
B\ar@{=>}[drrrrr]^(.4)g&&&
M\ar[r]_R\ar[u]^J\ar@{}[ur]|{(2)}\ar[ddll]^{f(a)}&
N\ar[ddrr]^{g(\textcolor{red}{r(a)})}\\
&&&&&&&\\
&&M\ar[uuuuu]^J\ar[rrrrr]_R\ar@{}[urrrrr]|{(3)}&&&&&N
}
\]
\begin{itemize}
\item $s=\mathrm{ker}\ r$ является конгруэнцией на $A$.
Существует разложение гомоморфизма $r$
	\begin{equation}
r=itj
	\label{eq: morphism of representations of algebra, homomorphism, 1}
	\end{equation}
$j=\mathrm{nat}\ s$ - естественный гомоморфизм
	\begin{equation}
\textcolor{red}{j(a)}=j(a)
	\label{eq: morphism of representations of algebra, homomorphism, 2}
	\end{equation}
$t$ - изоморфизм
	\begin{equation}
\textcolor{red}{r(a)}=t(\textcolor{red}{j(a)})
	\label{eq: morphism of representations of algebra, homomorphism, 3}
	\end{equation}
$i$ - вложение
	\begin{equation}
r(a)=i(\textcolor{red}{r(a)})
	\label{eq: morphism of representations of algebra, homomorphism, 4}
	\end{equation}
\item $S=\mathrm{ker}\ R$ является эквивалентностью на $M$.
Существует разложение отображения $R$
	\begin{equation}
R=ITJ
	\label{eq: morphism of representations of algebra, map, 1}
	\end{equation}
$J=\mathrm{nat}\ S$ - сюръекция
	\begin{equation}
\textcolor{blue}{J(m)}=J(m)
	\label{eq: morphism of representations of algebra, map, 2}
	\end{equation}
$T$ - биекция
	\begin{equation}
\textcolor{blue}{R(m)}=T(\textcolor{blue}{J(m)})
	\label{eq: morphism of representations of algebra, map, 3}
	\end{equation}
$I$ - вложение
	\begin{equation}
R(m)=I(\textcolor{blue}{R(m)})
	\label{eq: morphism of representations of algebra, map, 4}
	\end{equation}
\item $F$ - \Ts представление $\mathfrak{F}$\Hyph алгебры $A/s$ в $M/S$
\item $G$ - \Ts представление $\mathfrak{F}$\Hyph алгебры $rA$ в $RM$
\item Существует разложение морфизма представлений
\[
(r,R)=(i,I)(t,T)(j,J)
\]
\end{itemize} 
		\end{theorem}
		\begin{proof}
Существование диаграммы $(1)$ следует из теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, с. 74).
Существование диаграммы $(2)$ следует из теоремы I.3.1
(\citeBib{Cohn: Universal Algebra}, с. 28).

Мы начнём с диаграммы $(4)$.

Пусть $m_1\equiv m_2(\mathrm{mod}\ S)$.
%Тогда $J(m_1)=J(m_2)$,
Следовательно,
\begin{equation}
\textcolor{blue}{R(m_1)}=\textcolor{blue}{R(m_2)}
\label{eq: morphism of representations of algebra, (4), 1}
\end{equation}
%$JT(m_1)=JT(m_2)$,
%так как $JT$ - отображение на $MR$.
Если $a_1\equiv a_2(\mathrm{mod}s)$, то
\begin{equation}
\textcolor{red}{r(a_1)}=\textcolor{red}{r(a_2)}
\label{eq: morphism of representations of algebra, (4), 2}
\end{equation}
Следовательно,
$j(a_1)=j(a_2)$.
Так как $(r,R)$ - морфизм представлений, то
\begin{equation}
\textcolor{blue}{R(f(a_1)m_1)}=g(\textcolor{red}{r(a_1)})\textcolor{blue}{R(m_1)}
\label{eq: morphism of representations of algebra, (4), 3}
\end{equation}
\begin{equation}
\textcolor{blue}{R(f(a_2)m_2)}=g(\textcolor{red}{r(a_2)})\textcolor{blue}{R(m_2)}
\label{eq: morphism of representations of algebra, (4), 4}
\end{equation}
Из \eqref{eq: morphism of representations of algebra, (4), 1},
\eqref{eq: morphism of representations of algebra, (4), 2},
\eqref{eq: morphism of representations of algebra, (4), 3},
\eqref{eq: morphism of representations of algebra, (4), 4}
следует
\begin{equation}
\textcolor{blue}{R(f(a_1)m_1)}=\textcolor{blue}{R(f(a_2)m_2)}
\label{eq: morphism of representations of algebra, (4), 5}
\end{equation}
Из \eqref{eq: morphism of representations of algebra, (4), 5}
следует
\begin{equation}
f(a_1)m_1\equiv f(a_2)m_2(\mathrm{mod} S)
\label{eq: morphism of representations of algebra, (4), 6}
\end{equation}
и, следовательно,
\begin{equation}
\textcolor{blue}{J(f(a_1)m_1)}=\textcolor{blue}{J(f(a_2)m_2)}
\label{eq: morphism of representations of algebra, (4), 7}
\end{equation}
Из \eqref{eq: morphism of representations of algebra, (4), 7}
следует, что отображение
\begin{equation}
F(\textcolor{red}{j(a)})(\textcolor{blue}{J(m)})
=\textcolor{blue}{J(f(a)m))}
\label{eq: morphism of representations of algebra, (4), 8}
\end{equation}
определено корректно и является \Ts преобразованием множества $M/S$.

Из равенства
\eqref{eq: morphism of representations of algebra, (4), 6}
(в случае $a_1=a_2$) следует, что для любого $a$ \Ts преобразование
согласованно с эквивалентностью $S$.
Из теоремы
\ref{theorem: transformation correlated with equivalence} следует,
что на множестве ${}^\star(M/S)$ определена структура $\mathfrak{F}$\Hyph алгебры.
Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
\Ts преобразований
\begin{align*}
F(\textcolor{red}{j(a_i)})\textcolor{blue}{J(m)}&=
\textcolor{blue}{J(f(a_i)m))}
&i&=1,...,n
\end{align*}
пространства $M/S$. Мы положим
\[
\omega(F(\textcolor{red}{j(a_1)}),...,F(\textcolor{red}{j(a_n)}))
\textcolor{blue}{J(m)}=
J(\omega(f(a_1),...,f(a_n)))m)
\]
Следовательно, отображение $F$ является представлением
$\mathfrak{F}$\Hyph алгебры $A/s$.

Из \eqref{eq: morphism of representations of algebra, (4), 8}
следует, что $(j,J)$ является морфизмом представлений $f$ и $F$.

Рассмотрим диаграмму $(5)$.

Так как $T$ - биекция, то мы можем отождествить элементы множества
$M/S$ и множества $MR$, причём это отождествление имеет вид
\begin{equation}
T(\textcolor{blue}{J(m)})=\textcolor{blue}{R(m)}
\label{eq: morphism of representations of algebra, (5), 1}
\end{equation}
Мы можем записать \Ts преобразование $F(\textcolor{red}{j(a)})$
множества $M/S$ в виде
\begin{equation}
F(\textcolor{red}{j(a)}):\textcolor{blue}{J(m)}\rightarrow
F(\textcolor{red}{j(a)})\textcolor{blue}{J(m)}
\label{eq: morphism of representations of algebra, (5), 2}
\end{equation}
%Из \eqref{eq: morphism of representations of algebra, (4), 8}
%следует, что мы можем записать
%\eqref{eq: morphism of representations of algebra, (5), 2} в виде
%\begin{equation}
%F(\textcolor{red}{j(a)}):\textcolor{blue}{J(m)}\rightarrow
%\textcolor{blue}{J(f(a)m))}
%\label{eq: morphism of representations of algebra, (5), 3}
%\end{equation}
Так как $T$ - биекция, то мы можем определить \Ts преобразование
\begin{equation}
T(\textcolor{blue}{J(m)})\rightarrow
T(F(\textcolor{red}{j(a)})\textcolor{blue}{J(m)})
\label{eq: morphism of representations of algebra, (5), 3}
\end{equation}
множества $RM$. \Ts преобразование
\eqref{eq: morphism of representations of algebra, (5), 3}
зависит от $\textcolor{red}{j(a)}\in A/s$.
Так как $t$ - биекция, то мы можем отождествить элементы множества
$A/s$ и множества $rA$, причём это отождествление имеет вид
\[
t(\textcolor{red}{j(a)})=\textcolor{red}{r(a)}
\]
Следовательно, мы определили отображение
\[
G:rA\rightarrow{}^\star RM
\]
согласно равенству
\begin{equation}
G(t(\textcolor{red}{j(a)}))T(\textcolor{blue}{J(m)})=
T(F(\textcolor{red}{j(a)})\textcolor{blue}{J(m)})
\label{eq: morphism of representations of algebra, (5), 4}
\end{equation}

Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
\Ts преобразований
\begin{align*}
G(\textcolor{red}{r(a_i)})\textcolor{blue}{R(m)}&=
T(F(\textcolor{red}{j(a_i)})\textcolor{blue}{J(m)})
&i&=1,...,n
\end{align*}
пространства $RM$. Мы положим
\[
\omega(G(\textcolor{red}{r(a_1)}),...,G(\textcolor{red}{r(a_n)}))
\textcolor{blue}{R(m)}=
T(\omega(F(\textcolor{red}{j(a_1)},...,F(\textcolor{red}{j(a_n)}))
\textcolor{blue}{J(m)})
\]
Согласно \eqref{eq: morphism of representations of algebra, (5), 4}
операция $\omega$ корректно определена на множестве ${}^\star RM$.
Следовательно, отображение $G$ является представлением
$\mathfrak{F}$\Hyph алгебры.

Из \eqref{eq: morphism of representations of algebra, (5), 4}
следует, что $(t,T)$ является морфизмом представлений $F$ и $G$.

Диаграмма $(6)$ является самым простым случаем в нашем доказательстве.
Поскольку отображение $I$ является вложением и диаграмма $(2)$
коммутативна, мы можем отождествить $n\in N$ и $\textcolor{blue}{R(m)}$,
если $n\in\textrm{Im}R$. Аналогично, мы можем отождествить
соответствующие \Ts преобразования.
\begin{equation}
g'(i(\textcolor{red}{r(a)}))I(\textcolor{blue}{R(m)})=
I(G(\textcolor{red}{r(a)})\textcolor{blue}{R(m)})
\label{eq: morphism of representations of algebra, (6), 1}
\end{equation}
\[
\omega(g'(\textcolor{red}{r(a_1)}),...,g'(\textcolor{red}{r(a_n)}))
\textcolor{blue}{R(m)}=
I(\omega(G(\textcolor{red}{r(a_1)},...,G(\textcolor{red}{r(a_n)}))
\textcolor{blue}{R(m)})
\]
Следовательно,
$(i,I)$ является морфизмом представлений $G$ и $g$.

Для доказательства теоремы осталось показать, что определённое
в процессе доказательства \Ts представление $g'$ совпадает
с представлением $g$, а операции над преобразованиями совпадают
с соответствующими операциями на ${}^\star N$.
\begin{align*}
g'(i(\textcolor{red}{r(a)}))I(\textcolor{blue}{R(m)})
&=I(G(\textcolor{red}{r(a)})\textcolor{blue}{R(m)})
&&\textrm{согласно}\ \eqref{eq: morphism of representations of algebra, (6), 1}\\
&=I(G(t(\textcolor{red}{j(a)}))T(\textcolor{blue}{J(m)}))
&&\textrm{согласно}\ \eqref{eq: morphism of representations of algebra, homomorphism, 3},
\eqref{eq: morphism of representations of algebra, map, 3}\\
&=IT(F(\textcolor{red}{j(a)})\textcolor{blue}{J(m)})
&&\textrm{согласно}\ \eqref{eq: morphism of representations of algebra, (5), 4}\\
&=ITJ(f(a)m)
&&\textrm{согласно}\ \eqref{eq: morphism of representations of algebra, (4), 8}\\
&=R(f(a)m)
&&\textrm{согласно}\ \eqref{eq: morphism of representations of algebra, map, 1}\\
&=g(r(a))R(m)
&&\textrm{согласно}\ \eqref{eq: morphism of representations of F algebra, definition, 2}
\end{align*}
\begin{align*}
\omega(G(\textcolor{red}{r(a_1)}),...,G(\textcolor{red}{r(a_n)}))
\textcolor{blue}{R(m)}
&=T(\omega(F(\textcolor{red}{j(a_1)},...,F(\textcolor{red}{j(a_n)}))
\textcolor{blue}{J(m)})\\
&=T(F(\omega(\textcolor{red}{j(a_1)},...,\textcolor{red}{j(a_n)}))
\textcolor{blue}{J(m)})\\
&=T(F(j(\omega(a_1,...,a_n)))
\textcolor{blue}{J(m)})\\
&=T(J(f(\omega(a_1,...,a_n))m))\\
\end{align*}
		\end{proof}

Из теоремы \ref{theorem: decompositions of morphism of representations}
следует, что мы можем свести задачу изучения морфизма \Ts представлений
$\mathfrak{F}$\Hyph алгебры
к случаю, описываемому диаграммой
\begin{equation}
\xymatrix{
&M\ar[dd]_(.3){f(a)}\ar[rr]^J&&M/S\ar[dd]^(.3){F(\textcolor{red}{j(a)})}\\
&&&\\
&M\ar[rr]^J&&M/S\\
A\ar[rr]^j\ar@{=>}[uur]^(.3)f&&A/s\ar@{=>}[uur]^(.3)F
}
\label{eq: morphism of representations of algebra, reduce, 1}
\end{equation}

		\begin{theorem}
		\label{theorem: morphism of representations of algebra, reduce}
Диаграмма \eqref{eq: morphism of representations of algebra, reduce, 1}
может быть дополнена \Ts представлением $F_1$
$\mathfrak{F}$\Hyph алгебры $A$ в множестве $M/S$ так,
что диаграмма
\begin{equation}
\xymatrix{
&M\ar[dd]_(.3){f(a)}\ar[rr]^J&&M/S\ar[dd]^(.3){F(\textcolor{red}{j(a)})}\\
&&&\\
&M\ar[rr]^(.65)J&&M/S\\
A\ar[rr]^j\ar@{=>}[uur]^(.3)f\ar@{=>}[uurrr]^(.7){F_1}&&A/s\ar@{=>}[uur]^(.3)F
}
\label{eq: morphism of representations of algebra, reduce, 2}
\end{equation}
коммутативна. При этом множество \Ts преобразований \Ts представления $F$ и
множество \Ts преобразований \Ts представления $F_1$ совпадают.
		\end{theorem}
		\begin{proof}
Для доказательства теоремы достаточно положить
\[F_1(a)=F(\textcolor{red}{j(a)})\]
Так как отображение $j$ - сюрьекция, то $\mathrm{Im}F_1=\mathrm{Im}F$.
Так как $j$ и $F$ - гомоморфизмы $\mathfrak{F}$\Hyph алгебры, то $F_1$
- также гомоморфизм $\mathfrak{F}$\Hyph алгебры.
		\end{proof}

Теорема \ref{theorem: morphism of representations of algebra, reduce}
завершает цикл теорем, посвящённых структуре морфизма \Ts представлений
$\mathfrak{F}$\Hyph алгебры.
Из этих теорем следует, что мы можем упростить задачу изучения морфизма \Ts представлений
$\mathfrak{F}$\Hyph алгебры и ограничиться морфизмом \Ts представлений вида
\[
\xymatrix{
id:A\ar[r]&A&R:M\ar[r]&N
}
\]
В этом случае мы можем отождествить морфизм $(id,R)$ \Ts представлений
$\mathfrak{F}$\Hyph алгебры и отображение $R$.

		\begin{definition}
Пусть
\[
f:A\rightarrow {}^\star M
\]
\Ts представление $\mathfrak{F}$\Hyph алгебры $A$
в $\mathfrak{H}$\Hyph алгебре $M$ и 
\[
g:B\rightarrow {}^\star N
\]
\Ts представление $\mathfrak{F}$\Hyph алгебры $B$
в $\mathfrak{H}$\Hyph алгебре $N$.
Морфизм $(h,H)$ \Ts представлений алгебры типа $\mathfrak{F}$
называется
\AddIndex{морфизмом \Ts представлений $\mathfrak{F}$\Hyph алгебры
в $\mathfrak{H}$\Hyph алгебре}
{morphism of representations of F algebra in H algebra}.
		\qed
		\end{definition}



==> Vector.Bundle.Russian.tex <==
%auto-ignore
\def\texVectorField{}
\ifx\PrintBook\Defined
				\chapter{Векторное расслоение над телом}
				\label{chapter: Vector Bundle Over Skew-Field}
\fi

			\section{Векторное расслоение над телом}
			\label{section: Vector Bundle Over Skew-Field}

Чтобы определить \Ts представление
	\[
\mathcal F:\mathcal R\rightarrow {}^\star \mathcal{V}
	\]
расслоенного кольца $\mathcal R$ на расслоении $\mathcal{V}$
мы должны определить структуру расслоенного кольца на расслоении
${}^\star \mathcal{V}$.

		\begin{theorem}
		\label{theorem: Ts representation of the ring}
\Ts представление $\mathcal F$
расслоенного кольца $\mathcal R$ на расслоении $\mathcal{V}$ определенно тогда и только
тогда, когда определены \Ts представления расслоенных мультипликативной и аддитивной групп
расслоенного кольца $\mathcal R$
и эти расслоенные \Ts представления удовлетворяют соотношению
\[
\mathcal F(a(b+c))=\mathcal F(a)\mathcal F(b)+\mathcal F(a)\mathcal F(c)
\]
		\end{theorem}
		\begin{proof}
Теорема следует из определения
\ref{definition: Tstar representation of fibered F-algebra}.
		\end{proof}

		\begin{theorem}
		\label{theorem: effective Ts representation of the fibered skew field}
\Ts представление расслоенного тела $\mathcal D$
\AddIndex{эффективно}{effective representation of fibered skew field},
если эффективно \Ts представление расслоенной мультипликативной группы тела $D$.
		\end{theorem}
		\begin{proof}
Согласно определениям \ref{definition: effective representation of fibered F-algebra}
и \ref{definition: isomorphism of fibered F-algebras} утверждение теоремы
проверяется в слое. В слое утверждение теоремы является следствием теоремы
\xRef{0701.238}{theorem: effective Ts representation of the skew field}.
		\end{proof}

Согласно замечанию
\ref{remark: notation for effective representation of fibered F-algebra},
если представление расслоенного тела эффективно, мы отождествляем сечение
расслоенного тела и соответствующее
ему \Ts преобразование.

		\begin{definition}
		\label{definition: Tstar vector field}
$\mathcal{V}$ - \AddIndex{$\mathcal D\star$\Hyph векторное расслоение}{Dstar vector bundle}
нaд расслоенным телом $\mathcal D$,
если $\mathcal{V}$ - расслоенная абелева группa и
определено эффективное \Ts представление расслоенного тела $\mathcal D$.
Сечение $\mathcal D\star$\Hyph векторного расслоения
называется \AddIndex{$\mathcal D\star$\Hyph векторным полем}{Dstar vector field}.
		\qed
		\end{definition} 

		\begin{theorem}
$\mathcal D\star$\Hyph векторные поля $\mathcal{V}$ удовлетворяют
соотношениям
\begin{itemize}
\item 
\AddIndex{закону ассоциативности}{associative law, Dstar vector fields}
	\begin{equation}
	\label{eq: associative law, Dstar vector fields}
(ab)\Vector{m}=a(b\Vector{m})
	\end{equation}
\item 
\AddIndex{закону дистрибутивности}{distributive law, Dstar vector fields}
	\begin{align}
	\label{eq: distributive law, Dstar vector fields, 1}
a(\Vector{m}+\Vector{n})&=a\Vector{m}+a\Vector{n}\\
	\label{eq: distributive law, Dstar vector fields, 2}
(a+b)\Vector{m}&=a\Vector{m}+b\Vector{m}
	\end{align}
\item 
\AddIndex{закону унитарности}{unitarity law, Dstar vector fields}
	\begin{equation}
	\label{eq: unitarity law, Dstar vector fields}
1\Vector{m}=\Vector{m}
	\end{equation}
\end{itemize}
для любых $a, b \in \Gamma(\mathcal D)$, $\Vector{m}, \Vector{n} \in \Gamma(\mathcal{V})$.
Мы будем называть \Ts представление
\AddIndex{$\mathcal D\star$\Hyph произведением векторного поля на скаляр}
{Dstar product of vector field over scalar, vector space}.
		\end{theorem}
		\begin{proof}
Утверждение теоремы
проверяется в слое и является следствием теоремы
\xRef{0701.238}{theorem: definition of vector space}.
		\end{proof}

		\begin{definition}
Пусть $\mathcal{V}$ - $\mathcal D\star$\hyph векторное расслоение
нaд расслоенным телом $\mathcal D$.
Подрасслоение $\mathcal{N}\subset\mathcal{V}$ -
\AddIndex{подрасслоение $\mathcal D\star$\hyph векторного расслоения}
{subbundle of Dstar vector bundle} $\mathcal{V}$,
если $\Vector{a}+\Vector{b}\in\Gamma(\mathcal{N})$
и $k\Vector{a}\in\Gamma(\mathcal{N})$ для любых
$\Vector{a}$, $\Vector{b} \in\Gamma(\mathcal{N})$ и для любого $k\in\Gamma(\mathcal D)$.
		\qed
		\end{definition}

		\begin{definition}
Допустим $\Vector u$, $\Vector v\in\Gamma(\mathcal{V})$ - $\mathcal D\star$\hyph векторные поля. Мы будем
говорить, что векторное поле $\Vector w$ является
\AddIndex{$\mathcal D\star$\hyph линейной комбинацией векторные полей}
{linear composition of vector fields} $\Vector u$ и $\Vector v$,
если мы можем записать $\Vector w=a\Vector u+b\Vector v$, где $a$ и $b$ - скаляры.
		\qed
		\end{definition}

		\begin{remark}
		\label{remark: left and right vector bundle notation}
Мы распространим на векторное расслоение и его тип соглашение,
описанное в замечании
\xRef{0701.238}{remark: left and right vector space notation}.
Предполагается, что слоем \Drc векторного расслоения является
\drc векторное пространство.
		\qed
		\end{remark}

			\section{\texorpdfstring{$\mathcal D\RCstar$}{Drc}-базис векторного расслоения}
			\label{section: Basis of Vector Bundle}

		\begin{definition}
Векторные поля ${}_{\gi a}\Vector{a}$, $\gi{a}\in\gi{I}$ \Drc векторного расслоения
$\mathcal{V}$ \AddIndex{\Drc линейно независимы}
{linearly independent vector fields},
если $c=0$ следует из уравнения
\[c\RCstar\Vector{a}=0\]
В противном случае, векторные поля ${}_{\gi a}\Vector{a}$
\AddIndex{\Drc линейно зависимы}{linearly dependent vector fields}.
		\qed
		\end{definition}

		\begin{definition}
Множество векторных полей
\symb{\Basis{e}=({}_{\gi a}\Vector{e},\gi{a}\in \gi{I})}1
{drc basis, vector bundle}
- \AddIndex{\Drc базис векторного расслоения}{drc basis, vector bundle},
если векторы ${}_{\gi a}\Vector{e}$ \Drc линейно независимы и добавление
любого вектора к этой системе
делает эту систему \Drc линейно зависимой.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: expansion relative basis, vector bundle}
Если $\Basis{e}$ - \Drc базис векторного расслоения $\mathcal{V}$,
то любое векторное поле $\Vector{v}\in \mathcal{V}$
имеет одно и только одно разложение
	\begin{equation}
\Vector{v}=v\RCstar\Vector{e}
	\label{eq: expansion relative basis, vector bundle}
	\end{equation}
относительно этого \Drc базиса.
		\end{theorem}
		\begin{proof}
Утверждение теоремы проверяется в слое и является следствием
теоремы \xRef{0701.238}{theorem: expansion relative basis, vector space}.
		\end{proof}

		\begin{definition}
Мы будем называть матрицу
$v$ разложения \eqref{eq: expansion relative basis, vector bundle}
\AddIndex{координатной матрицей векторного поля $\Vector{v}$ в \Drc базисе $\Basis{e}$}
{coordinate matrix of vector field in drc basis}
и её элементы
\AddIndex{координатами векторного поля $\Vector{v}$ в \Drc базисе $\Basis{e}$}
{coordinates of vector field in drc basis}.
		\qed
		\end{definition}

Согласно построению все операции над векторными полями выполняются в
слое и поэтому в большинстве случаев мы можем применять методы
теории \drc векторных пространств.
Однако существует отличие.
Координатная матрица, так же как и координаты векторного поля,
является функцией координат точки на базе.\footnote{Однако
вопрос о непрерывности этой функции я пока оставлю открытым.}
Это может привести к различным ситуациям. Например,
\drc линейная зависимость векторных полей в слое
зависит от того, вырождена или нет координатная матрица соответствующих векторов.
Это одна из причин, почему мы имеем проблему определения
размерности, если мы рассматриваем \Drc векторное расслоение над
кольцом сечений $\Gamma(\mathcal D)$.
Рассматривая \Drc векторное расслоение как расслоенное представление,
мы получаем большую гибкость в определении \Drc базиса.

		\begin{theorem}
		\label{theorem: coordinate vector bundle}
Множество координат $a$ векторного поля $\Vector{a}$ в \Drc базисе $\Basis{e}$
порождают \Drc векторное расслоение \symb{\mathcal D^{\gi n}}1{coordinate drc vector bundle},
изоморфное \Drc векторному расслоению $\mathcal{V}$.
Это \Drc векторное расслоение называется
\AddIndex{координатным \Drc векторным расслоением}
{coordinate drc vector bundle},
а изоморфизм
\AddIndex{расслоенным координатным \Drc изоморфизмом}{fibered coordinate drc isomorphism}.
		\end{theorem}
		\begin{proof}
Допустим векторы $\Vector{a}$ и $\Vector{b}\in\mathcal{V}$ имеют разложение
\[
\Vector{a}=a\RCstar \Vector{e}
\]
\[
\Vector{b}=b\RCstar \Vector{e}
\]
в базисе $\Basis{e}$. Тогда
\[
\Vector{a}+\Vector{b}=
a\RCstar \Vector{e}+b\RCstar \Vector{e}
=(a+b)\RCstar\Vector{e}
\]
\[
m\Vector{a}=m(a\RCstar \Vector{e})=(ma)\RCstar\Vector{e}
\]
для любого $m\in D$.
Таким образом, операции в векторном расслоении определены по координатно
\[
(a+b)^{\gi a}=a^{\gi a}+b^{\gi a}
\]
\[
(ma)^{\gi a}=ma^{\gi a}
\]
Это доказывает теорему.
		\end{proof}

Так как мы линейная комбинация определена в слое,
принцип двойственности, сформулированный в теоремах
\xRef{0701.238}{theorem: duality principle, vector space},
\xRef{0701.238}{theorem: duality principle, vector space, quasideterminants},
сохраняется для векторных расслоений.

			\section{\texorpdfstring{$\mathcal D\RCstar$}{Drc}\hyph линейное отображение векторных расслоений}
			\label{section: Linear Map of Vector Bundles}

		\begin{definition}
		\label{definition: src trc linear map of vector bundles}
Пусть $\mathcal{A}$ - $\mathcal S\RCstar$\Hyph векторное расслоение.
Пусть $\mathcal{B}$ - $\mathcal T\RCstar$\Hyph векторное расслоение.
Мы будем называть морфизм
	\[
\xymatrix{
\mathcal F:\mathcal S\ar[r]&\mathcal T&\Vector{\mathcal H}:\mathcal{A}\ar[r]&\mathcal{B}
}
	\]
\Ts представлений расслоенного тела в расслоенной абелевой группе
\AddIndex{$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейным отображением векторных расслоений}
{src trc linear map of vector bundles}.
		\qed
		\end{definition}

Согласно теореме
\ref{theorem: decompositions of morphism of fibered representations}
при изучении $(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейного отображения
мы можем ограничиться случаем $\mathcal S=\mathcal T$.

		\begin{definition}
		\label{definition: drc linear map of vector bundles}
Пусть $\mathcal{A}$ и
$\mathcal{B}$ - \Drc векторные расслоения.
Мы будем называть отображение
	\begin{equation}
\Vector{\mathcal H}:\mathcal{A}\rightarrow \mathcal{B}
	\label{eq: drc linear map of vector bundles}
	\end{equation}
\AddIndex{\Drc линейным отображением векторных расслоений}{drc linear map of vector bundles},
если
	\begin{equation}
	\label{eq: drc linear map of vector bundles, product on scalar}
\Vector{\mathcal H}(a\RCstar \Vector{m})=a\RCstar \Vector{\mathcal H}(\Vector{m})
	\end{equation}
для любых $a^{\gi a} \in \Gamma(D)$, ${}_{\gi a}\Vector{m} \in \Gamma(\mathcal{A})$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: drc linear map of drc vector bundle}
Пусть $\Basis{f}=({}_{\gi a}\Vector{f},\gi{a}\in \gi{I})$
- \Drc базис в векторном расслоении $\mathcal{A}$
и $\Basis{e}=({}_{\gi b}\Vector{e},\gi{b}\in \gi{J})$
- \Drc базис в векторном расслоении $\mathcal{B}$.
Тогда \Drc линейное отображение \eqref{eq: drc linear map of vector bundles}
векторных расслоений имеет представление
	\begin{equation}
b=a\RCstar \mathcal H
	\label{eq: drc linear map of vector bundles, presentation}
	\end{equation}
относительно заданных базисов. Здесь
\begin{itemize}
\item $a$ - координатная матрица векторного поля
$\Vector a$ относительно \Drc базиса $\Basis{f}$
\item $b$ - координатная матрица векторного поля
$$\Vector b=\Vector{\mathcal H}(\Vector a)$$ относительно \Drc базиса $\Basis{e}$
\item $\mathcal H$ - координатная матрица множества векторных полей
$(\Vector {\mathcal H}({}_{\gi a}\Vector{f}))$ в \Drc базисе $\Basis{e}$, которую мы будем называть
\AddIndex{матрицей расслоенного \Drc линейного отображения}{matrix of fibered drc linear map}
относительно базисов $\Basis{f}$ и $\Basis{e}$
\end{itemize}
		\end{theorem}
		\begin{proof}
Векторное поле $\Vector{a}\in \Gamma(\mathcal{A})$ имеет разложение
	\[
\Vector{a}=a\RCstar \Vector{f}
	\]
относительно \Drc базиса $\Basis{f}$.
Векторное поле $\Vector{b}=f(\Vector{a})\in \Gamma(\mathcal{B})$ имеет разложение
	\begin{equation}
\Vector{b}=b\RCstar \Vector{e}
	\label{eq: drc linear map of vector bundles, presentation, 1}
	\end{equation}
относительно \Drc базиса $\Basis{e}$.

Так кaк $\Vector {\mathcal H}$ - \Drc линейное отображение, то на основании
\eqref{eq: drc linear map of vector bundles, product on scalar} следует,
что
	\begin{equation}
\Vector{b}=\Vector {\mathcal H}(\Vector{a})=\Vector{\mathcal H}(a\RCstar \Vector{f})
=a\RCstar \Vector {\mathcal H}(\Vector{f})
	\label{eq: drc linear map of vector bundles, presentation, 2}
	\end{equation}
$\Vector {\mathcal H}({}_{\gi a}\Vector{f})$ также векторное поле векторного расслоения $\mathcal{B}$ и имеет
разложение
	\begin{equation}
\Vector {\mathcal H}({}_{\gi a}\Vector{f})
={}_{\gi a}\mathcal H\RCstar \Vector{e}
={}_{\gi a}\mathcal H^{\gi b}\ {}_{\gi b}\Vector{e}
	\label{eq: drc linear map of vector bundles, presentation, 3}
	\end{equation}
относительно базиса $\Basis{e}$.
Комбинируя \eqref{eq: drc linear map of vector bundles, presentation, 2}
и \eqref{eq: drc linear map of vector bundles, presentation, 3}, мы получаем
	\begin{equation}
\Vector{b}=a\RCstar \mathcal H\RCstar\Vector{e}
	\label{eq: drc linear map of vector bundles, presentation, 4}
	\end{equation}
\eqref{eq: drc linear map of vector bundles, presentation}  следует
из сравнения \eqref{eq: drc linear map of vector bundles, presentation, 1}
и \eqref{eq: drc linear map of vector bundles, presentation, 4} и
теоремы \ref{theorem: expansion relative basis, vector bundle}.
		\end{proof}

На основании теоремы \ref{theorem: drc linear map of drc vector bundle}
мы идентифицируем расслоенное \Drc линейное отображение \eqref{eq: drc linear map of vector bundles}
векторных пространств и
матрицу его представления \eqref{eq: drc linear map of vector bundles, presentation}.

		\begin{theorem}
		\label{theorem: product of drc linear maps, vector bundles}
Пусть $$\Basis{f}=({}_{\gi a}\Vector{f},\gi{a}\in \gi{I})$$ \Drc базис в векторном расслоении $\mathcal{A}$,
$$\Basis{e}=({}_{\gi b}\Vector{e},\gi{b}\in \gi{J})$$ \Drc базис в векторном расслоении $\mathcal{B}$,
и $$\Basis{g}=({}_{\gi c}\Vector{g},\gi{c}\in \gi{L})$$ \Drc базис в векторном расслоении $\mathcal{C}$.
Предположим, что мы имеем коммутативную диаграмму \Drc линейных отображений
	\[
\xymatrix{
\mathcal{A}\ar[rr]^{\mathcal H}\ar[dr]^{\mathcal F} & & \mathcal{C}\\
&\mathcal{B}\ar[ur]^{\mathcal G} &
}
	\]
где \drc линейное отображение $\mathcal F$ имеет представление
	\begin{equation}
	\label{eq: product of drc linear maps, tstar vector bundles, A}
b=a\RCstar \mathcal F
	\end{equation}
относительно заданных базисов
и \drc линейное отображение $\mathcal G$ имеет представление
	\begin{equation}
	\label{eq: product of drc linear maps, tstar vector bundles, B}
c=b\RCstar \mathcal G
	\end{equation}
относительно заданных базисов.
Тогда \drc линейное отображение $\mathcal H$ имеет представление
	\begin{equation}
	\label{eq: product of drc linear maps, tstar vector bundles, C}
c=a\RCstar \mathcal F\RCstar \mathcal G
	\end{equation}
относительно заданных базисов.
		\end{theorem}
		\begin{proof}
Доказательство утверждения следует из подстановки
\eqref{eq: product of drc linear maps, tstar vector bundles, A}
в \eqref{eq: product of drc linear maps, tstar vector bundles, B}.
		\end{proof}

Записывая \drc линейное отображение в форме \RC произведения, мы можем переписать
\eqref{eq: drc linear map of vector bundles, product on scalar} в виде
	\begin{equation}
(ka)\RCstar \mathcal F=k(a\RCstar \mathcal F)
	\label{eq: drc linear map of vector bundles, product on scalar, image}
	\end{equation}
Утверждение теоремы
\ref{theorem: product of drc linear maps, vector bundles}
мы можем записать в виде
	\begin{equation}
(a\RCstar \mathcal F)\RCstar \mathcal G=a\RCstar (\mathcal F\RCstar \mathcal G)
	\label{eq: product of drc linear maps, vector bundles, image}
	\end{equation}
Равенства
\eqref{eq: drc linear map of vector bundles, product on scalar, image} и
\eqref{eq: product of drc linear maps, vector bundles, image}
представляют собой
\AddIndex{закон ассоциативности для \Drc линейных отображений векторных расслоений}
{associative law for drc linear maps of vector bundles}.
Это позволяет нам писать подобные выражения не пользуясь скобками.

Равенство \eqref{eq: drc linear map of vector bundles, presentation}
является координатной записью расслоенного \Drc линейного отображения.
На основе теоремы \ref{theorem: drc linear map of drc vector bundle}
бескоординатная запись также может быть представлена с помощью \RC произведения
	\begin{equation}
\Vector{b}=\Vector{a}\RCstar\Vector {\mathcal F}=a\RCstar \Vector{f}\RCstar\Vector {\mathcal F}
=a\RCstar \mathcal F\RCstar \Vector{e}
	\label{eq: drc linear map of vector bundles, presentation, 5}
	\end{equation}
Если подставить равенство \eqref{eq: drc linear map of vector bundles, presentation, 5} в теорему
\ref{theorem: product of drc linear maps, vector spaces},
то мы получим цепочку равенств
	\begin{align*}
\Vector{c}&=\Vector{b}\RCstar\Vector {\mathcal G}=b\RCstar \Vector{e}\RCstar\Vector {\mathcal G}
=b\RCstar \mathcal G\RCstar \Vector{g}\\
\Vector{c}&=\Vector{a}\RCstar\Vector {\mathcal F}\RCstar\Vector {\mathcal G}
=a\RCstar \Vector{f}\RCstar\Vector {\mathcal F}\RCstar\Vector {\mathcal G}
=a\RCstar \mathcal F\RCstar \mathcal G\RCstar \Vector{g}
	\end{align*}


==> Vector.Field.English.tex <==
%auto-ignore
\def\texVectorField{}
\ifx\PrintBook\Defined
				\chapter{Vector Field over Skew-Field}
				\label{chapter: Vector Field Over Skew-Field}
\fi

			\section{Vector Field over Skew-Field}
			\label{section: Vector Field Over Skew-Field}

To define \Ts representation
	\[
\mathcal F:\mathcal R\rightarrow {}^\star \mathcal{V}
	\]
of fibered ring $\mathcal R$ on the bundle $\mathcal{V}$
we need to define the structure of the fibered ring on the bundle
${}^\star \mathcal{V}$.

		\begin{theorem}
		\label{theorem: Ts representation of the ring}
\Ts representation $\mathcal F$ of the fibered ring
$\mathcal R$ on the bundle $\mathcal{V}$ is defined iff
\Ts representations of fibered multiplicative and additive groups
of the fibered ring $\mathcal R$ are defined
and these fibered \Ts representations hold relationship
\[
\mathcal F(a(b+c))=\mathcal F(a)\mathcal F(b)+\mathcal F(a)\mathcal F(c)
\]
		\end{theorem}
		\begin{proof}
Theorem follows from definition
\ref{definition: Tstar representation of fibered F-algebra}.
		\end{proof}

		\begin{theorem}
		\label{theorem: effective Ts representation of the fibered skew field}
\Ts representation of the fibered skew field $\mathcal D$ is
\AddIndex{effective}{effective representation of fibered skew field}
iff \Ts representation of its fibered multiplicative group is effective.
		\end{theorem}
		\begin{proof}
According to definitions \ref{definition: effective representation of fibered F-algebra}
and \ref{definition: isomorphism of fibered F-algebras} утверждение теоремы
проверяется в слое. В слое утверждение теоремы является следствием of theorem
\xRef{0701.238}{theorem: effective Ts representation of the skew field}.
		\end{proof}

According to the remark
\ref{remark: notation for effective representation of fibered F-algebra},
since the representation of the fibered skew field is effective, we identify
a section of the fibered skew field and
\Ts transformation corresponding to this section.

		\begin{definition}
		\label{definition: Tstar vector field}
$\mathcal{V}$ is a \AddIndex{$\mathcal D\star$\Hyph vector bundle}{Dstar vector bundle}
over a fibered skew field $\mathcal D$
if $\mathcal{V}$ is a fibered Abelian group and
there exists effective \Ts representation of fibered skew field $\mathcal D$.
Section of $\mathcal D\star$\Hyph vector bundle
is called a \AddIndex{$\mathcal D\star$\Hyph vector field}{Dstar vector field}.
		\qed
		\end{definition} 

		\begin{theorem}
Following conditions hold for $\mathcal D\star$\Hyph vector fields:
\begin{itemize}
\item 
\AddIndex{associative law}{associative law, Dstar vector fields}
	\begin{equation}
	\label{eq: associative law, Dstar vector fields}
(ab)\Vector{m}=a(b\Vector{m})
	\end{equation}
\item 
\AddIndex{distributive law}{distributive law, Dstar vector fields}
	\begin{align}
	\label{eq: distributive law, Dstar vector fields, 1}
a(\Vector{m}+\Vector{n})&=a\Vector{m}+a\Vector{n}\\
	\label{eq: distributive law, Dstar vector fields, 2}
(a+b)\Vector{m}&=a\Vector{m}+b\Vector{m}
	\end{align}
\item 
\AddIndex{unitarity law}{unitarity law, Dstar vector fields}
	\begin{equation}
	\label{eq: unitarity law, Dstar vector fields}
1\Vector{m}=\Vector{m}
	\end{equation}
\end{itemize}
for any $a, b \in \Gamma(\mathcal D)$, $\Vector{m}, \Vector{n} \in \Gamma(\mathcal{V})$.
We call \Ts representation
\AddIndex{$\mathcal D\star$\Hyph product of vector field over scalar}
{Dstar product of vector field over scalar, vector space}.
		\end{theorem}
		\begin{proof}
Since \Ts transformation $a$ is automorphism of the Abelian group,
we obtain the equation \eqref{eq: distributive law, Dstar vector fields, 1}.
Since \Ts representation is homomorphism of the aditive group of skew field $D$,
we obtain the equation \eqref{eq: distributive law, Dstar vector fields, 2}.
Since \Ts representation is \Ts representation of the multiplicative group of skew field $D$,
we obtain the equations \eqref{eq: associative law, Dstar vector fields} and
\eqref{eq: unitarity law, Dstar vector fields}.
		\end{proof}

According to our notation $D\star$\hyph vector space is
\AddIndex{left vector space}{left vector space} and
\AddIndex{$\star D$\hyph vector space}{starD-vector space} is
\AddIndex{right vector space}{right vector space}.

		\begin{definition}
Let $\mathcal{V}$ be a $D\star$\hyph vector space over a skew field $D$.
Set of vectors $\mathcal{N}$ is a
\AddIndex{subspace of $D\star$\hyph vector space}{subspace of Dstar vector space} $\mathcal{V}$
if $\Vector{a}+\Vector{b}\in\mathcal{N}$
and $k\Vector{a}\in\mathcal{N}$ for any
$\Vector{a}, \Vector{b} \in\mathcal{N}$ and for any $k\in D$.
		\qed
		\end{definition}

		\begin{example}
		\label{example: matrices vector space}
Let \symb{D^{\gi m}_{\gi n}}1{matrices vector space}
be set of $\gi m\times \gi n$
matrices over skew field $D$.
We define addition
	\[
a+b=
\left(a_{\gi i}^{\gi j}\right)
+
\left(b_{\gi i}^{\gi j}\right)
=
\left(a_{\gi i}^{\gi j}+b_{\gi i}^{\gi j}\right)
	\]
and product over scalar
	\[
da=
d\left(a_{\gi i}^{\gi j}\right)
=
\left(da_{\gi i}^{\gi j}\right)
	\]
$a=0$ iff $a_{\gi i}^{\gi j}=0$ for any ${\gi i}$, ${\gi j}$.
We can verify directly that
$D^{\gi m}_{\gi n}$ is a $D\star$\hyph vector space.
when product is defined from left. Otherwise $D^{\gi m}_{\gi n}$
is $\star D$\hyph vector space.
Vector space $D^{\gi m}_{\gi n}$ is called
\AddIndex{$D\star$\hyph matrices vector space}{matrices vector space}.
		\qed
		\end{example}

			\section{Vector Space Type}
			\label{section: vector space type}

The product of vector over scalar is asymmetric because
the product is defined for objects of different sets.
However we see difference between $D\star$\hyph\ and $\star D$\hyph vector space only when
we work with coordinate representation.
When we speak vector space is $D\star$\hyph\ or $\star D$\hyph\ we point out
how we multiply coordinates of vector over elements
of skew field: from left or right.

		\begin{definition}
Suppose $u$, $v$ are vectors of left vector space $\mathcal{V}$. We call
vector $w$ \AddIndex{$D\star$\hyph linear composition of  vectors}{linear composition of  vectors} $u$ and $v$
when we can write $w=au+bv$ where $a$ and $b$ are scalars.
		\qed
		\end{definition}

We can extend definition of the linear composition on any finite set
of vectors. Using generalized indexes to enumerate vectors we
can represent set of vectors as one dimensional matrix.
We use the convention that we represent any set of vectors of the vector space
or as \subs row either as \sups row.
This representation defines type of notation of linear composition.
Getting this representation in $D\star$- or $\star D$\hyph vector space we
get four different models of vector space.

For an opportunity to show
without change of the notation what kind of vector space
($D\star$- or $\star D$-) we study we introduce new notation.
We call symbol \symb{D\star}1{vector space type}\ \AddIndex{vector space type}{vector space type}
and this symbol means that we study
$D\star$\hyph vector space over skew field $D$.
The symbol of product in the type of vector space points to matrix operation used in
the linear composition.

		\begin{example}
Let \subs row
\[
\Vector{a}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{a} \\
...  \\
{}_{\gi n}\Vector{a}
\end{array}\right)
\]
represent the set of vectors
${}_{\gi a}\Vector{a}$, $\gi{a}\in\gi{I}$
of \AddIndex{\drc vector space}{drc vector space} $\mathcal{V}$
and \sups row
\[
c
=\left(\begin{array}{ccc}
c^{\gi 1} &
...  &
c^{\gi n}
\end{array}\right)
\]
represent the set of scalars
$c^{\gi a}$, $\gi{a}\in\gi{I}$.
Then we can write the linear composition of vectors ${}_{\gi a}\Vector{a}$ as
\[c^{\gi a}\ {}_{\gi a}\Vector{a}=c\RCstar\Vector{a}\]
We use notation \symb{{}_{D\RCstar}\mathcal{V}}1{left RC vector space}
when we want to tell that $\mathcal{V}$ is \drc vector space.
		\qed
		\end{example}

		\begin{example}
Let \sups row
\[
\Vector{a}
=\left(\begin{array}{ccc}
{}^{\gi 1}\Vector{a}&
... &
{}^{\gi n}\Vector{a}
\end{array}\right)
\]
represent the set of vectors
${}^{\gi a}\Vector{a}$, $\gi{a}\in\gi{I}$
of \AddIndex{\dcr vector space}{dcr vector space} $\mathcal{V}$
and \subs row
\[
c
=\left(\begin{array}{ccc}
c_{\gi 1} \\
...  \\
c_{\gi n}
\end{array}\right)
\]
represent the set of scalars
$c_{\gi a}$, $\gi{a}\in\gi{I}$.
Then we can write the linear composition of vectors ${}^{\gi a}\Vector{a}$ as
\[c_{\gi a}\ {}^{\gi a}\Vector{a}=c\CRstar\Vector{a}\]
We use notation \symb{{}_{D\CRstar}\mathcal{V}}1{left CR vector space}
when we want to tell that $\mathcal{V}$ is \dcr vector space.
		\qed
		\end{example}

		\begin{example}
Let \subs row
\[
\Vector{a}
=\left(\begin{array}{ccc}
\Vector{a}_{\gi 1} \\
...  \\
\Vector{a}_{\gi n}
\end{array}\right)
\]
represent the set of vectors
$\Vector{a}_{\gi a}$, $\gi{a}\in\gi{I}$
of \AddIndex{\crd vector space}{crd vector space} $\mathcal{V}$
and \sups row
\[
c
=\left(\begin{array}{ccc}
{}^{\gi 1}c &
...  &
{}^{\gi n}c
\end{array}\right)
\]
represent the set of scalars
${}^{\gi a}c$, $\gi{a}\in\gi{I}$.
Then we can write the linear composition of vectors $\Vector{a}_{\gi a}$ as
\[\Vector{a}_{\gi a}\ {}^{\gi a}c=\Vector{a}\CRstar c\]
We use notation \symb{\mathcal{V}_{\CRstar D}}1{right RC vector space}
when we want to tell that $\mathcal{V}$ is \crd vector space.
		\qed
		\end{example}

		\begin{example}
Let \sups row
\[
\Vector{a}
=\left(\begin{array}{ccc}
\Vector{a}^{\gi 1}&
... &
\Vector{a}^{\gi n}
\end{array}\right)
\]
represent the set of vectors
$\Vector{a}^{\gi a}$, $\gi{a}\in\gi{I}$
of \AddIndex{\rcd vector space}{rcd vector space} $\mathcal{V}$
and \subs row
\[
c
=\left(\begin{array}{ccc}
{}_{\gi 1}c \\
...  \\
{}_{\gi n}c
\end{array}\right)
\]
represent the set of scalars
${}_{\gi a}c$, $\gi{a}\in\gi{I}$.
Then we can write the linear composition of vectors $\Vector{a}^{\gi a}$ as
\[\Vector{a}^{\gi a}\ {}_{\gi a}c=\Vector{a}\RCstar c\]
We use notation \symb{\mathcal{V}_{\RCstar D}}1{right CR vector space}
when we want to tell that $\mathcal{V}$ is \rcd vector space.
		\qed
		\end{example}

		\begin{remark}
		\label{remark: left and right vector space notation}
We extend to vector space and its type convention
described in remark
\xRef{0612.111}{remark: left and right matrix notation}.
For instance, we execute operations in expression
\[A\RCstar B\RCstar v\lambda\]
from left to right. This corresponds to
the \rcd vector space. However we can execute product
from right to left. In custom notation this expression is
\[\lambda v\CRstar B\CRstar A\]
and corresponds to \dcr vector space. Similarly, reading this expression from
down up we get expression
\[A\CRstar B\CRstar v\lambda\]
corresponding to \crd vector space.
		\qed
		\end{remark}

			\section{\texorpdfstring{$D\RCstar$}{Drc}-Basis of Vector Space}
			\label{section: Basis of Vector Space}

		\begin{definition}
Vectors ${}_{\gi a}\Vector{a}$, $\gi{a}\in\gi{I}$ of \drc vector space
$\mathcal{V}$ are \AddIndex{\drc linearly independent}
{linearly independent, vector space}
if $c=0$ follows from the equation
\[c\RCstar\Vector{a}=0\]
Otherwise vectors ${}_{\gi a}\Vector{a}$
are \AddIndex{\drc linearly dependent}{linearly dependent, vector space}.
		\qed
		\end{definition}

		\begin{definition}
We call set of vectors
\symb{\Basis{e}=({}_{\gi a}\Vector{e},\gi{a}\in \gi{I})}1
{basis, vector space}
a \AddIndex{\drc basis for vector space}{drc basis, vector space}
if vectors ${}_{\gi a}\Vector{e}$ are
\drc linearly independent and adding to this system any other vector
we get a new system which is \drc linearly dependent.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: expansion relative basis, vector space}
If $\Basis{e}$ is a \drc basis of vector space $\mathcal{V}$
then any vector $\Vector{v}\in \mathcal{V}$
has one and only one expansion 
	\begin{equation}
\Vector{v}=v\RCstar\Vector{e}
	\label{eq: expansion relative basis, vector space}
	\end{equation}
relative to this \drc basis.
		\end{theorem}
		\begin{proof}
Because system of vectors ${}_{\gi a}\Vector{e}$
is a maximal set of \drc linearly independent vectors
the system of vectors $\Vector{v},{}_{\gi a}\Vector{e}$
is \drc linearly dependent and in equation
	\begin{equation}
b\Vector{v}+c\RCstar\Vector{e}=0
	\label{eq: expansion relative basis, vector space, 1}
	\end{equation}
at least $b$ is different from $0$. Then equation
	\begin{equation}
\Vector{v}=(-b^{-1}c)\RCstar\Vector{e}
	\label{eq: expansion relative basis, vector space, 2}
	\end{equation}
follows from \eqref{eq: expansion relative basis, vector space, 1}.
\eqref{eq: expansion relative basis, vector space} follows
from \eqref{eq: expansion relative basis, vector space, 2}.

Assume we get another expansion
	\begin{equation}
\Vector{v}=v'\RCstar\Vector{e}
	\label{eq: expansion relative basis, vector space, 3}
	\end{equation}
We subtract \eqref{eq: expansion relative basis, vector space}
from \eqref{eq: expansion relative basis, vector space, 3}
and get
	\[
0=(v'-v)\RCstar\Vector{e}
	\]
Because vectors ${}_{\gi a}\Vector{e}$ are \drc linearly independent we get
\[v'-v=0\]
		\end{proof}

		\begin{definition}
We call the matrix
$v$ in expansion \eqref{eq: expansion relative basis, vector space}
\AddIndex{coordinate matrix of vector $\Vector{v}$ in \drc basis $\Basis{e}$}
{coordinate matrix of vector in drc basis}
and we call its elements
\AddIndex{coordinates of vector $\Vector{v}$ in \drc basis $\Basis{e}$}
{coordinates of vector in drc basis}.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: coordinate vector space}
Set of coordinates $a$ of vector $\Vector{a}$ relative \drc basis $\Basis{e}$
forms \drc vector space \symb{D^{\gi n}}1{drc coordinate vector space}
isomorphic \drc vector space $\mathcal{V}$.
This \drc vector space is called
\AddIndex{\drc coordinate vector space}
{drc coordinate vector space}.
This isomorphism
is called \AddIndex{coordinate isomorphism}{coordinate isomorphism}.
		\end{theorem}
		\begin{proof}
Suppose vectors $\Vector{a}$ and $\Vector{b}\in\mathcal{V}$ have expansion
\[
\Vector{a}=a\RCstar \Vector{e}
\]
\[
\Vector{b}=b\RCstar \Vector{e}
\]
relative basis $\Basis{e}$. Then
\[
\Vector{a}+\Vector{b}=
a\RCstar \Vector{e}+b\RCstar \Vector{e}
=(a+b)\RCstar\Vector{e}
\]
\[
m\Vector{a}=m(a\RCstar \Vector{e})=(ma)\RCstar\Vector{e}
\]
for any $m\in S$.
Thus, operations in a vector space are defined by coordinates
\[
(a+b)^{\gi a}=a^{\gi a}+b^{\gi a}
\]
\[
(ma)^{\gi a}=ma^{\gi a}
\]
This completes the proof.
		\end{proof}

		\begin{example}
		\label{example: drc vector space}
Let $\Basis{e}=({}_{\gi i}\Vector{e},\gi i\in \gi I,|\gi I|=\gi n)$
be a \drc basis of vector space $D^{\gi n}$.
The coordinate matrix
\symb{a= \left(\begin{array}{ccc}
a^{\gi 1} &
... &
a^{\gi n}
\end{array}\right)}0{drc vector}
\[
\ShowSymbol{drc vector}
=(a^{\gi i},\gi i\in\gi I)
	\]
of vector $\Vector{a}$ in \drc basis $\Basis{e}$
is called \AddIndex{\drc vector}{drc vector}.\footnote{\drc vector
is an analogue of row vector. We can also call it \sups row $D\star$\Hyph vector.}
We call vector space
\symb{D^{\gi n}}1{r rows drc vector space}
\AddIndex{\sups rows \drc vector space}{sups rows drc vector space}.

Let \subs row
	\begin{equation}
	\label{eq: subs row, vectors}
\Vector{a}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{a} \\
...  \\
{}_{\gi m}\Vector{a}
\end{array}\right)
=({}_{\gi i}\Vector{a},\gi i\in\gi M)
	\end{equation}
be set of vectors.
Vectors ${}_{\gi a}\Vector{a}$ have expansion
	\[
{}_{\gi a}\Vector{a}={}_{\gi a}a\RCstar\Vector{f}
	\]
Substituting coordinate matrices of vector ${}_{\gi i}\Vector{a}$ to
matrix \eqref{eq: subs row, vectors} we get matrix
\[
a
=\left(\begin{array}{ccc}
\left(\begin{array}{ccc}
{}_{\gi 1}a^{\gi 1} &
... &
{}_{\gi 1}a^{\gi n}
\end{array}\right) \\
...  \\
\left(\begin{array}{ccc}
{}_{\gi m}a^{\gi 1} &
... &
{}_{\gi m}a^{\gi n}
\end{array}\right)
\end{array}\right)
=\left(\begin{array}{ccc}
{}_{\gi 1}a^{\gi 1} &
... &
{}_{\gi 1}a^{\gi n} \\
...&...&...  \\
{}_{\gi m}a^{\gi 1} &
... &
{}_{\gi m}a^{\gi n}
\end{array}\right)
=({}_{\gi i}a^{\gi j})
\]
We call the matrix $a$
\AddIndex{coordinate matrix of set of vectors}{coordinate matrix of set of vectors, drc vector space}
$({}_{\gi i}\Vector{a},\gi i\in\gi M)$ in basis $\Basis{e}$
and we call its elements
\AddIndex{coordinates of set of vectors}{coordinates of set of vectors, drc vector space}
$({}_{\gi i}\Vector{a},\gi i\in\gi M)$ in basis $\Basis{e}$.

\subs Row
\symb{\Vector{f}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{f} \\
...  \\
{}_{\gi n}\Vector{f}
\end{array}\right)}0{basis, r rows drc vector space}
\[
\ShowSymbol{basis, r rows drc vector space}
=({}_{\gi i}\Vector{f},\gi i\in\gi I)
\]
represents the
\AddIndex{\drc basis $\Basis{f}$ of \sups rows vector space}
{drc basis, r rows vector space}
$D^{\gi n}$.
We tell that coordinate matrix $f$ of set of vectors
$({}_{\gi i}\Vector{f},\gi i\in\gi I)$ defines coordinates
\symb{{}_{\gi i}f^{\gi j}}1{basis coordinates, r rows drc vector space}
of basis $\Basis{f}$ relative basis $\Basis{e}$.
		\qed
		\end{example}

		\begin{example}
		\label{example: dcr vector space}
Let $\Basis{e}=({}^{\gi i}\Vector{e},\gi i\in\gi I,|\gi I|=\gi n)$
be a \dcr basis of vector space $D_{\gi n}$.
The coordinate matrix
\symb{a= \left(\begin{array}{ccc}
a_{\gi 1} \\
...  \\
a_{\gi n}
\end{array}\right)}0{dcr vector}
\[
\ShowSymbol{dcr vector}
=(a_{\gi i},\gi i\in\gi I)
	\]
of vector $\Vector{a}$ in \dcr basis $\Basis{e}$
is called \AddIndex{\dcr vector}{dcr vector}.\footnote{\dcr vector
is an analogue of column vector. We can also call it \subs row $D\star$\Hyph vector}
We call vector space
\symb{D_{\gi n}}1{c rows dcr vector space}
\AddIndex{\subs rows \dcr vector space}{subs rows dcr vector space}.

Let \sups row
	\begin{equation}
	\label{eq: sups row, vectors}
\Vector{a}
=\left(\begin{array}{ccc}
{}^{\gi 1}\Vector{a} &
...  &
{}^{\gi m}\Vector{a}
\end{array}\right)
=({}^{\gi i}\Vector{a},\gi i\in\gi M)
	\end{equation}
be set of vectors.
Vectors ${}^{\gi a}\Vector{a}$ have expansion
	\[
{}^{\gi a}\Vector{a}={}^{\gi a}a\CRstar\Vector{f}
	\]
Substituting coordinate matrices of vector ${}^{\gi i}\Vector{a}$ to
matrix \eqref{eq: sups row, vectors} we get matrix
\[
a
= \left(\begin{array}{ccc}
\left(\begin{array}{ccc}
{}^{\gi 1}a_{\gi 1} \\
...  \\
{}^{\gi 1}a_{\gi n}
\end{array}\right) &
... &
\left(\begin{array}{ccc}
{}^{\gi m}a_{\gi 1} \\
...  \\
{}^{\gi m}a_{\gi n}
\end{array}\right)
\end{array}\right)
= \left(\begin{array}{ccc}
{}^{\gi 1}a_{\gi 1}&...&{}^{\gi m}a_{\gi 1} \\
... &...&... \\
{}^{\gi 1}a_{\gi n}&...&{}^{\gi m}a_{\gi n}
\end{array}\right)
=({}^{\gi i}a_{\gi j})
\]
We call the matrix $a$
\AddIndex{coordinate matrix of set of vectors}{coordinate matrix of set of vectors, dcr vector space}
$({}^{\gi i}\Vector{a},\gi i\in\gi M)$ in basis $\Basis{e}$
and we call its elements
\AddIndex{coordinates of set of vectors}{coordinates of set of vectors, dcr vector space}
$({}^{\gi i}\Vector{a},\gi i\in\gi M)$ in basis $\Basis{e}$.

\sups Row
\symb{\Vector{f}
= \left(\begin{array}{ccc}
{}^{\gi 1}\Vector{f} &
... &
{}^{\gi n}\Vector{f}
\end{array}\right)}0{basis, c rows dcr vector space}
\[
\ShowSymbol{basis, c rows dcr vector space}
=({}^{\gi i}\Vector{f},\gi i\in \gi I)
\]
represents the
\AddIndex{\dcr basis $\Basis{f}$ of \subs rows  vector space}
{dcr basis, c rows vector space}
$D_{\gi n}$.
We tell that coordinate matrix $f$ of set of vectors
$({}^{\gi i}\Vector{f},\gi i\in \gi I)$ defines coordinates
\symb{{}^{\gi i}f_{\gi j}}1{basis coordinates, c rows dcr vector space}
of basis $\Basis{f}$ relative basis $\Basis{e}$.
		\qed
		\end{example}

Since we express linear composition using matrices we can
extend the duality principle to the vector space theory.
We can write duality principle in one of the following forms

		\begin{theorem}[duality principle]
		\label{theorem: duality principle}
Let $\mathfrak{A}$ be true statement about vector spaces.
If we exchange the same time
\begin{itemize}
\item \drc vector and \dcr vector
\item \rcd vector and \crd vector
\item \RC product and \CR product
\end{itemize}
then we soon get true statement.
		\end{theorem}

		\begin{theorem}[duality principle]
%		\label{theorem: duality principle, quasideterminants}
Let $\mathfrak{A}$ be true statement about vector spaces.
If we exchange the same time
\begin{itemize}
\item \drc vector and \rcd vector or \dcr vector and \crd vector
\item \RC quasideterminant and \CR quasideterminant
\end{itemize}
then we soon get true statement.
		\end{theorem}

\input{Drc.Morphism.English}

			\section{System of \texorpdfstring{$D\RCstar$}{Drc}\hyph Linear Equations}
			\label{section: System of Linear Equations}

		\begin{definition}
		\label{definition: linear span, vector space}
Let $\mathcal{V}$ be a \drc vector space and
$\{{}_{\gi a}\Vector{a}\in\mathcal{V}, \gi{a}\in\gi{I}\}$ be set of vectors.
\AddIndex{\drc linear span in vector space}{linear span, vector space}
is set
\symb{\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})}1{linear span, vector space}
of vectors \drc linearly dependent on vectors ${}_{\gi a}\Vector{a}$.
		\qed
		\end{definition}

		\begin{theorem}
Let $\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})$ be \drc linear span in
vector space $\mathcal{V}$.
Then $\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})$ is subspace of $\mathcal{V}$.
		\end{theorem}
		\begin{proof}
Suppose
	\begin{align*}
\Vector{b}&\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})\\
\Vector{c}&\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})
	\end{align*}
According to definition \ref{definition: linear span, vector space}
	\begin{align*}
\Vector{b}&=b\RCstar \Vector{a}\\
\Vector{c}&=c\RCstar \Vector{a}
	\end{align*}
Then
	\begin{align*}
\Vector{b}+\Vector{c}
=b\RCstar\Vector{a}+c\RCstar\Vector{a}
=(b+c)\RCstar\Vector{a}
&\in\text{span}(\Vector{a}_{\gi a},\gi{a}\in\gi{I})\\
k\Vector{b}=k(b\RCstar\Vector{a})=(kb)\RCstar\Vector{a}
&\in\text{span}(\Vector{a}_{\gi a},\gi{a}\in\gi{I})
	\end{align*}
This proves the statement.
		\end{proof}

Let $\mathcal{V}$ be a \drc vector space and
\subs row
	\begin{equation}
	\label{eq: linear span, vectors}
\Vector{a}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{a} \\
...  \\
{}_{\gi n}\Vector{a}
\end{array}\right)
=({}_{\gi i}\Vector{a},\gi i\in\gi M)
	\end{equation}
be set of vectors.
To answer the question of whether vector
$\Vector{b}\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{M})$
we write linear equation
	\begin{equation}
\Vector{b}=x\RCstar\Vector{a}
	\label{eq: linear span, vector space, 1}
	\end{equation}
where
\[
x=\left(
 \begin{array}{ccc}
x^{\gi 1}&...&x^{\gi m}
\end{array}
\right)
\]
is \sups row of unknown coefficients of expansion.
$\Vector{b}\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{M})$
if equation \eqref{eq: linear span, vector space, 1}
has a solution.
Suppose $\Vector{f}=({}_{\gi b}\Vector{f},\gi{b}\in\gi{N})$ is a \drc basis.
Then vectors $\Vector{b}$, ${}_{\gi a}\Vector{a}$ have expansion
	\begin{align}
	\label{eq: linear span, vector space, b}
\Vector{b}&=b\RCstar\Vector{f}\\
	\label{eq: linear span, vector space, ai}
{}_{\gi a}\Vector{a}&={}_{\gi a}a\RCstar\Vector{f}
	\end{align}
If we substitute \eqref{eq: linear span, vector space, b}
and \eqref{eq: linear span, vector space, ai}
into \eqref{eq: linear span, vector space, 1} we get
	\begin{equation}
b\RCstar\Vector{f}=x\RCstar a\RCstar\Vector{f}
	\label{eq: linear span, vector space, 2}
	\end{equation}
Applying theorem \ref{theorem: expansion relative basis, vector space}
to \eqref{eq: linear span, vector space, 2} we get
\AddIndex{system of \drc linear equations}
{system of linear equations}
	\begin{equation}
	\label{eq: system of linear equations}
x\RCstar a=b
	\end{equation}

We can write system of \drc linear equations
\eqref{eq: system of linear equations} in one of the next forms
\[
\left(
 \begin{array}{ccc}
x^{\gi 1}&...&x^{\gi m}
\end{array}\right)
\RCstar \left(
 \begin{array}{ccc}
{}_{\gi 1}a^{\gi 1} & ... & {}_{\gi 1}a^{\gi n}\\
... & ... & ... \\
{}_{\gi m}a^{\gi 1} &...& {}_{\gi m}a^{\gi n}
\end{array}
\right)=\left(
 \begin{array}{ccc}
b^{\gi 1}&...&b^{\gi m}
\end{array}
\right)
\]
	\begin{equation}
	\label{eq: star columns system of linear equations}
x^{\gi a}\ {}_{\gi a}a^{\gi b}=b^{\gi b}
	\end{equation}
	\[
\begin{array}{ccc}
x^{\gi 1}\ {}_{\gi 1}a^{\gi 1} & ... & x^{\gi 1}\ {}_{\gi 1}a^{\gi n}\\
+& ... & +\\
... & ... & ... \\
+& ... & +\\
x^{\gi m}\ {}_{\gi m}a^{\gi 1} &...& x^{\gi m}\ {}_{\gi m}a^{\gi n} \\
=& ... & =\\
b^{\gi 1} &...& b^{\gi n} 
\end{array}
	\]

Let $\mathcal{V}$ be a \dcr vector space.
Reading system \eqref{eq: system of linear equations} of \drc linear equations from bottom up
we get system of \dcr linear equations
\[
x^\CRstar a=b
\]
which we can write in one of the following forms
\[
x\CRstar a=b
\]
\[
\left(
 \begin{array}{ccc}
x_{\gi 1}\\...\\x_{\gi n}
\end{array}\right)
\CRstar \left(
 \begin{array}{ccc}
{}^{\gi 1}a_{\gi 1} &...& {}^{\gi n}a_{\gi 1}\\
... & ... & ... \\
{}^{\gi 1}a_{\gi m} &...& {}^{\gi n}a_{\gi m}
\end{array}
\right)=\left(
 \begin{array}{ccc}
b_{\gi 1}\\...\\ b_{\gi m}
\end{array}
\right)
\]
	\begin{equation}
	\label{eq: star rows system of linear equations}
x_{\gi a}\ {}^{\gi a}a_{\gi b}=b_{\gi b}
	\end{equation}
	\[
\begin{array}{cccc}
x_{\gi 1}\ {}^{\gi 1}a_{\gi 1} &+...&+ x_{\gi n}\ {}^{\gi n}a_{\gi 1}&=b_{\gi 1}\\
... & ... & ...& ... \\
x_{\gi 1}\ {}^{\gi 1}a_{\gi m} &+...&+ x_{\gi n}\ {}^{\gi n}a_{\gi m}&=b_{\gi m}
\end{array}
	\]

		\begin{definition}
Suppose $a$
is \RC nonsingular matrix. We call appropriate systems
	\begin{equation}
	\label{eq: nonsingular system of linear equations}
x\RCstar a=b
	\end{equation}
\AddIndex{nonsingular system of \drc linear equations}
{nonsingular system of linear equations}.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: nonsingular system of linear equations}
Solution of nonsingular system of \drc linear equations
\eqref{eq: nonsingular system of linear equations}
is determined uniquely and can be presented
in either form\footnote{We can see a solution of system
\eqref{eq: nonsingular system of linear equations}
in theorem
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
I repeat this statement because I slightly changed the notation.
\label{footnote: nonsingular system of linear equations}}
	\begin{align}
	\label{eq: nonsingular system of linear equations, solution, matrix}
x&=b\RCstar a^{\RCInverse} \\
	\label{eq: nonsingular system of linear equations, solution, quasideterminant}
x&=b\RCstar \mathcal{H}\RCDet{a}
	\end{align}
		\end{theorem}
		\begin{proof}
Multiplying both sides of equation \eqref{eq: nonsingular system of linear equations}
from right by $a^{\RCInverse}$ we get
\eqref{eq: nonsingular system of linear equations, solution, matrix}.
Using definition
\xEqRef{0612.111}{eq: RC-quasideterminant definition}
we get \eqref{eq: nonsingular system of linear equations, solution, quasideterminant}.
Since theorem
\xEqRef{0612.111}{theorem: two products equal}
the solution is unique.
		\end{proof}

			\section{Rank of Matrix}
			\label{section: Rank of Matrix}

		\begin{definition}
Matrix\footnote{In
this section, we will make the following assumption.
\begin{itemize}
\item $\gi{a}\in\gi{M}$, $|\gi{M}|=\gi m$, $\gi{b}\in\gi{N}$, $|\gi{N}|=\gi n$.
\item $A=({}_{\gi a}A^{\gi b})$ is an arbitrary matrix.
\item $\gi k$, $\gi{s}\in \gi{S}\supseteq \gi{M}$,
$\gi l$, $\gi{t}\in \gi{T}\supseteq \gi{N}$, $\gi k=|\gi{S}|=|\gi{T}|$.
\item $\gi{p}\in\gi{M}\setminus\gi S$, $\gi{r}\in\gi{N}\setminus\gi{T}$.
\end{itemize}
\label{footnote: index assumption}}
${}_{\gi S}A^{\gi T}$ is a minor of an order $\gi k$.
		\qed
		\end{definition}

		\begin{definition}
If $\gi n\times \gi n$ matrix $a$ has \RC inverse matrix
we call such matrix
\AddIndex{\RC nonsingular matrix}{RC nonsingular matrix}.
Otherwise, we call such matrix
\AddIndex{\RC singular matrix}{RC singular matrix}.
		\qed
		\end{definition}

		\begin{definition}
If minor ${}_{\gi S}A^{\gi T}$ is \RC nonsingular matrix
then we say that
\RC rank of matrix $A$ is not less then $\gi k$.
\AddIndex{\RC rank of matrix $A$}{rc-rank of matrix}
\symb{\RCRank A}2{rc-rank of matrix}%
is the maximal value of $\gi k$.
We call an appropriate minor the \AddIndex{\RC major minor}{RC-major minor}.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: singular matrix and quasideterminant}
Let matrix $A$ be \RC singular matrix and minor ${}_{\gi S}A^{\gi T}$
be major minor. Then
	\begin{equation}
	\label{eq: singular matrix and quasideterminant}
{}_{\gi p}\RCDet{{}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}}^{\gi r}=0
	\end{equation}
		\end{theorem}
		\begin{proof}
To understand why minor ${}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}$
does not have \RC inverse matrix,\footnote{It is natural to expect relationship
between \RC singularity of the matrix
and its \RC quasideterminant similar to relationship which is known in commutative case.
However \RC quasideterminant is defined not always. For instance, it is not
defined when \RC inverse matrix
has too much elements equal $0$. As it follows from this theorem, the \RC quasideterminant
is undefined also in case when \RC rank of the matrix is less then $\gi{n-1}$.}
we assume that it has the \RC inverse matrix and write down the respective system
\xEqRef{0612.111}{eq: inverse minor,1},
\xEqRef{0612.111}{eq: inverse minor,2}.
We assume $\gi I=\gi r$, $\gi J=\gi p$ and will try to solve this system.
Assume
	\begin{equation}
	\label{eq: singular matrix and quasideterminant, 0}
B={}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}
	\end{equation}
Then we get system
	\begin{align}
	\label{eq: singular matrix and quasideterminant, 1}
{}_{\gi S}B^{\gi T}\RCstar
{}_{\gi T}B^{\RCInverse}{}^{\gi p}
+ {}_{\gi S}B^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=0\\
	\label{eq: singular matrix and quasideterminant, 2}
{}_{\gi p}B^{\gi T}\RCstar
{}_{\gi T}B^{\RCInverse}{}^{\gi p}
+{}_{\gi p}B^{\gi r}\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
We multiply \eqref{eq: singular matrix and quasideterminant, 1} by
$({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}$
	\begin{equation}
	\label{eq: singular matrix and quasideterminant, 3}
{}_{\gi T}B^{\RCInverse}{}^{\gi p}
+({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}\RCstar
{}_{\gi S}B^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}=0
	\end{equation}
Now we can substitute \eqref{eq: singular matrix and quasideterminant, 3} into
\eqref{eq: singular matrix and quasideterminant, 2}
	\begin{align}
	\label{eq: singular matrix and quasideterminant, 4}
-{}_{\gi p}B^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}\RCstar
{}_{\gi S}B^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}
+{}_{\gi p}B^{\gi r} \ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
From \eqref{eq: singular matrix and quasideterminant, 4} it follows that
	\begin{align}
	\label{eq: singular matrix and quasideterminant, 5}
({}_{\gi p}B^{\gi r}-{}_{\gi p}B^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}\RCstar
{}_{\gi S}B^{\gi r})
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
Expression in brackets is quasideterminant
${}_{\gi p}\RCDet{B}^{\gi r}$.
Substituting this expression into \eqref{eq: singular matrix and quasideterminant, 5},
we get

	\begin{align}
	\label{eq: singular matrix and quasideterminant, 6}
{}_{\gi p}\RCDet{B}^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
Thus we proved that quasideterminant ${}_{\gi p}\RCDet{B}^{\gi r}$
is defined and its equation to $0$ is necessary and sufficient condition
that the matrix $B$ is singular. Since \eqref{eq: singular matrix and quasideterminant, 0}
the statement of theorem is proved.
		\end{proof}

		\begin{theorem}
		\label{theorem: rc rank of matrix, sups-rows}
Suppose $A$ is a matrix,
$$\RCRank  A=\gi k<\gi m$$
and ${}_{\gi S}A^{\gi T}$ is \RC major minor.
Then \sups row ${}_{\gi p}A$ is
a \drc linear composition of \sups rows ${}_{\gi s}A$.
	\begin{align}
	\label{eq: rc rank of matrix, sups-rows}
{}_{\gi{M}\setminus\gi S}A&=r\RCstar {}_{\gi S}A\\
	\label{eq: rc rank of matrix, sups-rows, 1}
{}_{\gi p}A&={}_{\gi p}r\RCstar {}_{\gi S}A\\
	\label{eq: rc rank of matrix, sups-rows, 2}
{}_{\gi p}A^{\gi b}&={}_{\gi p}r^{\gi s}\ {}_{\gi s}A^{\gi b}
	\end{align}
		\end{theorem}
		\begin{proof}
If a number of \subs rows is $\gi k$ then assuming that \sups row ${}_{\gi p}A$
is a \drc linear combination \eqref{eq: rc rank of matrix, sups-rows, 1}
of \sups rows ${}_{\gi s}A$ with coefficients ${}_{\gi p}r^{\gi s}$
we get system \eqref{eq: rc rank of matrix, sups-rows, 2}.
According to theorem \ref{theorem: nonsingular system of linear equations}
this system has a unique solution\footnote{We assume
that unknown variables are $x^{\gi s}={}_{\gi p}r^{\gi s}$
\label{footnote: xs=rps}}
and it is nontrivial because all \RC quasideterminants are
different from $0$.

It remains to prove this statement in case when a number of \subs rows is more then $k$.
I get \sups row ${}_{\gi p}A$ and \subs row $A^{\gi r}$.
According to assumption minor
${}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}$ is a \RC singular matrix
and its \RC quasideterminant
	\begin{equation}
{}_{\gi p}\RCDet{{}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}}^{\gi r}=0
	\label{eq: rc rank of matrix, sups-rows, 3}
	\end{equation}
According to
\xEqRef{0612.111}{eq: quasideterminant, 1}
\eqref{eq: rc rank of matrix, sups-rows, 3} has form
	\[
{}_{\gi p}A^{\gi r}
-{}_{\gi p}A^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi r}=0
	\]
Matrix
	\begin{equation}
{}_{\gi p}r
={}_{\gi p}A^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})
	\label{eq: rc rank of matrix, sups-rows, 4}
	\end{equation}
do not depend on $\gi{r}$, Therefore, for any $\gi{r}\in\gi{N}\setminus\gi{T}$
	\begin{equation}
{}_{\gi p}A^{\gi r}
={}_{\gi p}r\RCstar {}_{\gi S}A^{\gi r}
	\label{eq: rc rank of matrix, sups-rows, 5}
	\end{equation}

From equation
	\[
(({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi l}
={}_{\gi T}\delta^{\gi l}
	\]
it follows that
	\begin{equation}
{}_{\gi p}A^{\gi l}=
{}_{\gi p}A^{\gi T}\RCstar {}_{\gi T}\delta^{\gi l}=
{}_{\gi p}A^{\gi T}\RCstar
(({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi l}
	\label{eq: rc rank of matrix, sups-rows, 7}
	\end{equation}
Substituting \eqref{eq: rc rank of matrix, sups-rows, 4}
into \eqref{eq: rc rank of matrix, sups-rows, 7} we get
	\begin{equation}
	\label{eq: rc rank of matrix, sups-rows, 8}
{}_{\gi p}A^{\gi l}=
{}_{\gi p}r\RCstar {}_{\gi S}A^{\gi l}
	\end{equation}
\eqref{eq: rc rank of matrix, sups-rows, 5} and \eqref{eq: rc rank of matrix, sups-rows, 8}
finish the proof.
		\end{proof}

		\begin{corollary}
		\label{corollary:rc rank of matrix, sups-rows}
Suppose $A$ is a matrix,
$\RCRank A=\gi k<\gi m$.
Then \sups rows of the matrix are \drc linearly dependent.
	\begin{equation}
	\label{eq: rc rank of matrix, sups-rows drc linearly dependent}
\lambda\RCstar A=0
	\end{equation}
		\end{corollary}
		\begin{proof}
Suppose \sups row ${}_{\gi p}A$ is a \drc linear composition
\eqref{eq: rc rank of matrix, sups-rows, 1}. We assume
$\lambda^{\gi p}=-1$, $\lambda^{\gi s}={}_{\gi p}r^{\gi s}$
and the rest $\lambda^{\gi c}=0$.
		\end{proof}

		\begin{theorem}
		\label{theorem: rank of coordinate matrix}
Let $({}_{\gi i}\Vector{a},\gi i\in\gi M,|\gi M|=\gi m)$ be set of
\drc linear independent vectors. Then \RC rank of their
coordinate matrix equal $\gi m$.
		\end{theorem}
		\begin{proof}
According to model built in example \ref{example: drc vector space},
the coordinate matrix of set of vectors $({}_{\gi i}\Vector{a})$ relative basis $\Basis{e}$
consists from \sups rows which are coordinate matrices of vectors
${}_{\gi i}\Vector{a}$ relative the basis $\Basis{e}$. Therefore \RC rank of
this matrix cannot be more then $\gi m$.

Let \RC rank of
the coordinate matrix be less then $\gi m$.
According to corollary \ref{corollary:rc rank of matrix, sups-rows}
\sups rows of matrix are \drc linear dependent. Let us multiply both parts of equation
\ref{eq: rc rank of matrix, sups-rows drc linearly dependent} over
\subs row $\Vector{e}$.
Suppose $c=\lambda\RCstar A$. Then we get that \drc linear composition
\[
c\RCstar \Vector{e}=0
\]
of vectors of basis equal $0$. This contradicts to statement that vectors $\Vector{e}$
form basis. We proved statement of theorem.
		\end{proof}

		\begin{theorem}
		\label{theorem: rc rank of matrix, subs-rows}
Suppose $A$ is a matrix,
$$\RCRank A=\gi k<\gi n$$
and ${}_{\gi S}A^{\gi T}$ is \RC major minor.
Then \subs row $A^{\gi r}$ is
a \rcd linear composition of \subs rows $A^{\gi t}$
	\begin{align}
	\label{eq: rc rank of matrix, star-columns}
A^{\gi{N}\setminus\gi{T}}&=A^{\gi T}\RCstar r\\
	\label{eq: rc rank of matrix, star-columns, 1}
A^{\gi r}&=A^{\gi T}\RCstar r^{\gi r}\\
	\label{eq: rc rank of matrix, star-columns, 2}
{}_{\gi a}A^{\gi r}&={}_{\gi a}A^{\gi t}\ {}_{\gi t}r^{\gi r}
	\end{align}
		\end{theorem}
		\begin{proof}
If a number of \sups rows is $\gi k$ then assuming that \subs row $A^{\gi r}$
is a \rcd linear combination \eqref{eq: rc rank of matrix, star-columns, 1}
of \subs rows $A^{\gi t}$ with coefficients ${}_{\gi t}r^{\gi r}$
we get system \eqref{eq: rc rank of matrix, star-columns, 2}.
According to theorem \ref{theorem: nonsingular system of linear equations}
this system has a unique solution\footnote{We assume
that unknown variables are ${}_{\gi t}x={}_{\gi t}r^{\gi r}$
\label{footnote: xt=rtq}}
and it is nontrivial because all \RC quasideterminants are
different from $0$.

It remains to prove this statement in case when a number of \sups rows is more then $\gi k$.
I get \subs row $A^{\gi r}$ and \sups row ${}_{\gi p}A$.
According to assumption minor
${}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}$ is a \RC singular matrix
and its $\mathcal{RC}$-quasideterminant
	\begin{equation}
{}_{\gi p}\RCDet{{}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}}^{\gi r}=0
	\label{eq: rc rank of matrix, star-columns, 3}
	\end{equation}
According to
\xEqRef{0612.111}{eq: quasideterminant, 1}
\eqref{eq: rc rank of matrix, star-columns, 3} has form
	\[
{}_{\gi p}A^{\gi r}
-{}_{\gi p}A^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi r}=0
	\]
Matrix
	\begin{equation}
r^{\gi r}
=({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi r}
	\label{eq: rc rank of matrix, star-columns, 4}
	\end{equation}
do not depend on $\gi{p}$, Therefore, for any $\gi{p}\in\gi{M}\setminus \gi{S}$
	\begin{equation}
{}_{\gi p}A^{\gi r}
={}_{\gi p}A^{\gi T}\RCstar r^{\gi r}
	\label{eq: rc rank of matrix, star-columns, 5}
	\end{equation}

From equation
	\[
{}_{\gi k}A^{\gi T}\RCstar (({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})^{\gi s}
={}_{\gi k}\delta^{\gi s}
	\]
it follows that
	\begin{equation}
{}_{\gi k}A^{\gi r}=
{}_{\gi k}\delta^{\gi S}\RCstar {}_{\gi S}A^{\gi r}=
{}_{\gi k}A^{\gi T}\RCstar (({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})^{\gi s}
\RCstar {}_{\gi s}A^{\gi r}
	\label{eq: rc rank of matrix, star-columns, 7}
	\end{equation}
Substituting \eqref{eq: rc rank of matrix, star-columns, 4}
into \eqref{eq: rc rank of matrix, star-columns, 7} we get
	\begin{equation}
	\label{eq: rc rank of matrix, star-columns, 8}
{}_{\gi k}A^{\gi r}=
{}_{\gi k}A^{\gi t}\RCstar r^{\gi r}
	\end{equation}
\eqref{eq: rc rank of matrix, star-columns, 5} and \eqref{eq: rc rank of matrix, star-columns, 8}
finish the proof.
		\end{proof}

		\begin{corollary}
		\label{corollary:rc rank of matrix, star-columns}
Suppose $A$ is a matrix,
$\RCRank A=\gi k<\gi m$.
Then \subs rows of the matrix are \rcd linearly dependent.
	\[
A\RCstar \lambda=0
	\]
		\end{corollary}
		\begin{proof}
Suppose \subs row $A^{\gi r}$ is a right linear composition
\eqref{eq: rc rank of matrix, star-columns, 1}. We assume
$\lambda_{\gi r}=-1$, $\lambda_{\gi t}=r_{\gi t}^{\gi r}$
and the rest $\lambda^{\gi c}=0$.
		\end{proof}

Base on theorem \xEqRef{0612.111}{theorem: duality principle, quasideterminants}
we can write similar statements for \CR rank of matrix.

		\begin{theorem}
		\label{theorem: cr rank of matrix, star-rows}
Suppose $A$ is a matrix,
\symb{\CRRank  A}0{cr-rank of matrix}
$$\ShowSymbol{cr-rank of matrix}=\gi k<\gi m$$
and ${}^{\gi T}A_{\gi S}$ is \CR major minor.
Then \sups row $A_{\gi p}$ is
a \crd linear composition of \sups rows $A_{\gi s}$.
	\begin{align}
	\label{eq: cr rank of matrix, star-rows}
A_{\gi{M}\setminus\gi S}&=A_{\gi S}\CRstar r\\
	\label{eq: cr rank of matrix, star-rows, 1}
A_{\gi p}&=A_{\gi S}\CRstar r_{\gi p}\\
	\label{eq: cr rank of matrix, star-rows, 2}
{}^{\gi b}A_{\gi p}&={}^{\gi b}A_{\gi s}\ {}^{\gi s}r_{\gi p}
	\end{align}
		\end{theorem}

		\begin{corollary}
		\label{corollary:cr rank of matrix, star-rows}
Suppose $A$ is a matrix,
$\CRRank A=\gi k<\gi m$.
Then \sups rows of matrix are \crd linearly dependent.
	\[
A\CRstar\lambda=0\\
	\]
		\end{corollary}

		\begin{theorem}
		\label{theorem: cr rank of matrix, star-columns}
Suppose $A$ is a matrix,
$$\CRRank A=\gi k<\gi n$$
and ${}^{\gi T}A_{\gi S}$ is \CR major minor.
Then \subs row ${}^{\gi r}A$ is
a \rcd linear composition of \subs rows $A^{\gi t}$
	\begin{align}
	\label{eq: cr rank of matrix, star-columns}
{}^{\gi{N}\setminus\gi{T}}A&=r\RCstar {}^{\gi T}A\\
	\label{eq: cr rank of matrix, star-columns, 1}
{}^{\gi r}A&={}^{\gi r}r\RCstar {}^{\gi T}A\\
	\label{eq: cr rank of matrix, star-columns, 2}
{}^{\gi r}A_{\gi a}&={}^{\gi r}r_{\gi t}\ {}^{\gi t}A_{\gi a}
	\end{align}
		\end{theorem}

		\begin{corollary}
		\label{corollary:cr rank of matrix, star-columns}
Suppose $A$ is a matrix,
$\CRRank a=\gi k<\gi m$.
Then \subs rows of matrix are \drc linearly dependent.
	\[
\lambda\RCstar A=0
	\]
		\end{corollary}

			\section{System of \texorpdfstring{$D\RCstar$}{Drc}\hyph Linear Equations}
			\label{section: Columns System of Linear Equations}

		\begin{definition}
Suppose\footref{footnote: index assumption}
$A$ is a matrix of system of \drc linear equations
\eqref{eq: star columns system of linear equations}.
We call matrix
	\begin{equation}
\left(
 \begin{array}{ccc}
{}_{\gi a}A^{\gi b}\\ b^{\gi b}
\end{array}\right)=
\left(
 \begin{array}{cccc}
{}_{\gi 1}A^1 & ... & {}_{\gi 1}A^n\\
... & ... & ... \\
{}_{\gi m}A^1&...& {}_{\gi m}A^n\\
b^1&...& b^n
\end{array}\right)
	\label{eq: extended matrix, system of drc linear equations}
	\end{equation}
an \AddIndex{extended matrix}{extended matrix, system of drc linear equations} of this system.
		\qed
		\end{definition}

		\begin{definition}
Suppose\footref{footnote: index assumption}
$a$ is a matrix of system of \rcd linear equations
\eqref{eq: star rows system of linear equations}.
We call matrix
	\begin{equation}
\left(
\begin{array}{ccc}
{}_{\gi a}A^{\gi b}& {}_{\gi a}b 
\end{array}\right)=
\left(
 \begin{array}{cccc}
{}_{\gi 1}A^1 & ... & {}_{\gi 1}A^n &{}_1b\\
... & ... & ... &...\\
{}_{\gi m}A^1 &...& {}_{\gi m}A^n&{}_mb
\end{array}\right)
	\label{eq: extended matrix, system of rcd linear equations}
	\end{equation}
an \AddIndex{extended matrix}{extended matrix, system of rcd linear equations} of this system.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: star columns system of linear equations}
System of \drc linear equations \eqref{eq: star columns system of linear equations}
has a solution iff
	\begin{equation}
\RCRank({}_{\gi a}A^{\gi b})=\RCRank\left(
 \begin{array}{ccc}
{}_{\gi a}A^{\gi b}\\ b^{\gi b}
\end{array}\right)
	\label{eq: star columns system of linear equations, rank}
	\end{equation}
		\end{theorem}
		\begin{proof}
Let ${}_{\gi S}A^{\gi T}$ be \RC major minor of matrix $A$.

Let a system of \drc linear equations \eqref{eq: star columns system of linear equations}
have solution $x^{\gi a}=d^{\gi a}$. Then
	\begin{equation}
d\RCstar A=b
	\label{eq: star columns system of linear equations, 1}
	\end{equation}
Equation \eqref{eq: star columns system of linear equations, 1} can be rewritten in form
	\begin{equation}
d^{\gi S}\RCstar {}_{\gi S}A+d^{\gi{M}\setminus\gi S}\RCstar {}_{\gi{M}\setminus\gi S}A=b
	\label{eq: star columns system of linear equations, 2}
	\end{equation}
Substituting \eqref{eq: rc rank of matrix, sups-rows} into
\eqref{eq: star columns system of linear equations, 2} we get
	\begin{equation}
d^{\gi S}\RCstar {}_{\gi S}A+d^{\gi{M}\setminus\gi S}\RCstar r\RCstar {}_{\gi S}A=b
	\label{eq: star columns system of linear equations, 3}
	\end{equation}
From \eqref{eq: star columns system of linear equations, 3} it follows that \sups row
$b$ is a \drc linear combination of \sups rows ${}_{\gi S}A$
	\[
(d^{\gi S}+d^{\gi{M}\setminus\gi S}\RCstar r)\RCstar {}_{\gi S}A=b
	\]
This holds equation \eqref{eq: star columns system of linear equations, rank}.

It remains to  prove that an existence of solution of system of \drc linear equations
\eqref{eq: star columns system of linear equations} follows from \eqref{eq: star columns system of linear equations, rank}.
Holding \eqref{eq: star columns system of linear equations, rank} means that
${}_{\gi S}A^{\gi T}$ is \RC major minor of extended matrix as well.
From theorem \ref{theorem: rc rank of matrix, sups-rows} it follows that \sups row $b$ is
a \drc linear composition of \sups rows $a_{\gi s}$
	\[
b=r^{\gi S}\RCstar {}_{\gi S}A
	\]
Assigning $r^{\gi p}=0$ we get
	\[
b=r\RCstar a
	\]
Therefore, we found at least one solution of system \eqref{eq: star columns system of linear equations}.
		\end{proof}

		\begin{theorem}
		\label{theorem: left system of linear equations, solution}
Suppose \eqref{eq: star columns system of linear equations} is
a system of \drc linear equations
satisfying \eqref{eq: star columns system of linear equations, rank}.
If $\RCRank  a=\gi k\le \gi m$
then solution of the system depends
on arbitrary values of $\gi m-\gi k$ variables not included into \RC major minor.
		\end{theorem}
		\begin{proof}
Let ${}_{\gi S}A^{\gi T}$ be \RC major minor of matrix $a$.
Suppose
	\begin{equation}
	\label{eq: star columns system of linear equations, reduce, 1}
x\RCstar a^{\gi r}=b^{\gi r}
	\end{equation}
is an equation with number $\gi{r}$.
Applying theorem \ref{theorem: rc rank of matrix, subs-rows}
to extended matrix \eqref{eq: extended matrix, system of drc linear equations} we get
	\begin{align}
	\label{eq: star columns system of linear equations, reduce, 2}
a^{\gi r}&=a^{\gi T}\RCstar r^{\gi r}\\
	\label{eq: star columns system of linear equations, reduce, 3}
b^{\gi r}&=b^{\gi T}\RCstar r^{\gi r}
	\end{align}
Substituting \eqref{eq: star columns system of linear equations, reduce, 2}
and \eqref{eq: star columns system of linear equations, reduce, 3}
into \eqref{eq: star columns system of linear equations, reduce, 1} we get
	\begin{equation}
	\label{eq: star columns system of linear equations, reduce, 4}
x\RCstar a^{\gi T}\RCstar r^{\gi r}=b^{\gi T}\RCstar r^{\gi r}
	\end{equation}
\eqref{eq: star columns system of linear equations, reduce, 4} means that
we can exclute equation \eqref{eq: star columns system of linear equations, reduce, 1}
from system \eqref{eq: star columns system of linear equations}
and the new system is equivalent to the old one.
Therefore, a number of equations can be reduced to $\gi k$.

At this point,
we have two choices. If the number of variables is also $\gi k$ then according to
theorem \ref{theorem: nonsingular system of linear equations} the system has unique solution
\eqref{eq: nonsingular system of linear equations, solution, quasideterminant}.
If the number of variables $\gi m>\gi k$ then we can move $\gi m-\gi k$ variables that are not
included into \RC major minor into right side.
Giving arbitrary values to these variables, we determine value of
the right side and for this value we get a unique solution according to
theorem \ref{theorem: nonsingular system of linear equations}.
		\end{proof}

		\begin{corollary}
		\label{corollary: nonsingular rows system of linear equations}
System of \drc linear equations \eqref{eq: star columns system of linear equations}
has a unique solution iff
its matrix is nonsingular.
		\qed
		\end{corollary}

		\begin{theorem}
		\label{theorem: Solutions homogenous system of linear equations}
Solutions of a homogenous system of \drc linear equations
	\begin{equation}
x\RCstar a=0
	\label{eq: homogenous system of linear equations}
	\end{equation}
form a \drc vector space.
		\end{theorem}
		\begin{proof}
Let $\mathcal{X}$ be set of solutions of
\eqref{eq: homogenous system of linear equations}.
Suppose $x=(x^{\gi a})\in\mathcal{X}$ and $y=(y^{\gi a})\in\mathcal{X}$. 
Then \[x^{\gi a}\ _{\gi a}a^{\gi b}=0\] \[y^{\gi a}\ _{\gi a}a^{\gi b}=0\]
Therefore
\[
(x^{\gi a}+y^{\gi a})\ _{\gi a}a^{\gi b}=
x^{\gi a}\ _{\gi a}a^{\gi b}+y^{\gi a}\ _{\gi a}a^{\gi b}=0
\]
\[x+y=(x^{\gi a}+y^{\gi a})\in\mathcal{X}\]
The same way we see
\[
(bx^{\gi a})\ _{\gi a}a^{\gi b}=b(x^{\gi a}\ _{\gi a}a^{\gi b})=0
\]
\[bx=(bx^{\gi a})\in\mathcal{X}\]
According to definition \ref{definition: Tstar vector space}
$\mathcal{X}$ is a \drc vector space.
		\end{proof}

			\section{Nonsingular Matrix}
%\begin{form}
%\CheckBox{label}
%\end{form}

Suppose $A$ is $\gi n\times \gi n$ matrix.
Corollaries \ref{corollary:rc rank of matrix, sups-rows}
and \ref{corollary:rc rank of matrix, star-columns}
tell us that if $\RCRank a<\gi n$
then \sups rows are \drc linearly dependent
and \subs rows are \rcd linearly dependent.\footnote{This
statement is similar to proposition
\citeBib{q-alg-9705026}-\href{http://arxiv.org/PS_cache/q-alg/pdf/9705/9705026.pdf\#Page=6}{1.2.5}.}

		\begin{theorem}
		\label{theorem: rc rank, rows}
Let $A$ be $\gi n\times\gi n$ matrix
and \sups row ${}_{\gi a}A$ be a \drc linear combination of other \sups rows.
Then $\RCRank  A<\gi n$.
		\end{theorem}
		\begin{proof}
The statement that \sups row ${}_{\gi a}A$ is a \drc linear combination of other \sups rows
means that system of \drc linear equations
	\begin{equation}
	\label{eq: rc rank, rows}
{}_{\gi a}A=\lambda\RCstar {}_{[\gi a]}A
	\end{equation}
has at least one solution.
According theorem \ref{theorem: star columns system of linear equations}
\[
\RCRank A=\RCRank {}_{[\gi a]}A
\]
Since a number of \sups rows is less then $\gi n$
we get $\RCRank {}_{[\gi a]}A<\gi n$.
		\end{proof}

		\begin{theorem}
		\label{theorem: rc rank, columns}
Let $A$ be $\gi n\times\gi n$ matrix
and \subs row $A^{\gi b}$ be a \rcd linear combination of other \subs rows.
Then $\RCRank A<\gi n$.
		\end{theorem}
		\begin{proof}
Proof of statement is similar to proof of theorem \ref{theorem: rc rank, rows}
		\end{proof}

		\begin{theorem}
Suppose $A$ and $B$ are $\gi n\times\gi n$ matrices and
	\begin{equation}
	\label{eq: RC product singular, 1}
C=A\RCstar B
	\end{equation}
$C$ is \RC singular matrix iff
either matrix $A$ or matrix $B$ is \RC singular matrix.
		\end{theorem}
		\begin{proof}
Suppose matrix $A$ is \RC singular.
According theorem \ref{theorem: rc rank of matrix, sups-rows}
\sups rows of matrix $A$ are
\drc linearly dependent. Therefore
	\begin{equation}
	\label{eq: RC product singular, 2}
0=\lambda\RCstar A
	\end{equation}
where $\lambda\ne 0$. From
\eqref{eq: RC product singular, 1} and \eqref{eq: RC product singular, 2}
it follows that
\[
\lambda\RCstar C=\lambda\RCstar A\RCstar B=0
\]
According theorem \ref{theorem: rc rank, rows} matrix $C$ is \RC singular.

Suppose matrix $A$ is not \RC singular, but matrix $B$ is \RC singular
According to theorem \ref{theorem: rc rank of matrix, sups-rows}
\sups rows of matrix $B$ are
\drc linearly dependent. Therefore
	\begin{equation}
	\label{eq: RC product singular, 3}
0=\mu\RCstar B
	\end{equation}
where $\mu\ne 0$. According to
theorem \ref{theorem: nonsingular system of linear equations}
the system
	\[
\lambda\RCstar A=\mu
	\]
has only solution where $\lambda\ne=0$.
Therefore
\[
\lambda\RCstar C=\lambda\RCstar A\RCstar B
=\mu\RCstar B=0
\]
According to theorem \ref{theorem: rc rank, rows} matrix $C$ is \RC singular.

Suppose matrix $C$ is \RC singular matrix.
According to the theorem \ref{theorem: rc rank of matrix, sups-rows}
\sups rows of matrix $C$ are
\drc linearly dependent. Therefore
	\begin{equation}
	\label{eq: RC product singular, 4}
0=\lambda\RCstar C
	\end{equation}
where $\lambda\ne 0$.
From \eqref{eq: RC product singular, 1}
and \eqref{eq: RC product singular, 4} it follows that
	\[
0=\lambda\RCstar A\RCstar B
	\]
If 
	\[
0=\lambda\RCstar A
	\]
satisfied then matrix $A$ is \RC singular. Suppose that
matrix $A$ is not \RC singular. Let us introduce
	\[
\mu=\lambda\RCstar A
	\]
where $\mu\ne 0$. Then
	\begin{equation}
	\label{eq: RC product singular, 5}
0=\mu\RCstar B
	\end{equation}
From \eqref{eq: RC product singular, 5} it follows that
matrix $B$ is \RC singular.
		\end{proof}

Basing theorem \xEqRef{0612.111}{theorem: duality principle, quasideterminants}
we can write similar statements for \crd linear combination of \sups rows
or \dcr linear combination of \subs rows and \CR quasideterminant.

		\begin{theorem}
		\label{theorem: cr rank, rows}
Let $A$ be $\gi n\times\gi n$ matrix
and \sups row ${}_{\gi a}A$ be a \crd linear combination of other \sups rows.
Then $\CRRank  A<\gi n$.
		\end{theorem}

		\begin{theorem}
		\label{theorem: cr rank, columns}
Let $A$ be $\gi n\times\gi n$ matrix
and \subs row $A^{\gi b}$ be a \drc linear combination of other \subs rows.
Then $\CRRank  A<\gi n$.
		\end{theorem}

		\begin{theorem}
Suppose $A$ and $B$ are $\gi n\times\gi n$ matrices and
$C=A\CRstar B$. $C$ is \CR singular matrix iff
either matrix $A$ or matrix $B$ is \CR singular matrix.
		\end{theorem}

		\begin{definition}
\AddIndex{\RC matrix group}{rc-matrix group}
\symb{\RCGL nD}1{rc-matrix group} is a group
of \RC nonsingular matrices where we define
\RC product of matrices
\xEqRef{0612.111}{eq: rc-product of matrices}
and \RC inverse matrix
$A^{\RCInverse}$.
		\qed
		\end{definition}

		\begin{definition}
\AddIndex{\CR matrix group}{cr-matrix group}
\symb{\CRGL nD}1{cr-matrix group} is a group
of \CR nonsingular matrices
where we define
\CR product of matrices
\xEqRef{0612.111}{eq: cr-product of matrices}
and \CR inverse matrix
$A^{\CRInverse}$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: CR RC singular matrix}
	\[
\RCGL nD\ne \CRGL nD
	\]
		\end{theorem}
		\begin{remark}
From theorem
\xEqRef{0612.111}{theorem: RC-inverse matrix, delta}
it follows that
there are matrices which are \CR nonsingular and \RC nonsingular.
Theorem \ref{theorem: CR RC singular matrix} implies that sets of
\CR nonsingular matrices and \RC nonsingular matrices are
not identical. For instance,
there exists such \RC nonsingular matrix which is
\CR singular matrix.
		\qed
		\end{remark}
		\begin{proof}
It is enough to prove this statement for $n={\gi 2}$.
Assume every \CR singular matrix
	\begin{equation}
a=
\left(
 \begin{array}{ccc}
a_{\gi 1}^{\gi 1} 
&
a_{\gi 1}^{\gi 2}
\\
a_{\gi 2}^{\gi 1} 
&
a_{\gi 2}^{\gi 2}
\end{array}
\right)
	\label{eq: CR-singular matrix, 1}
	\end{equation}
is \RC singular matrix.
It follows from theorem \ref{theorem: rc rank of matrix, sups-rows}
and theorem \ref{theorem: rc rank of matrix, subs-rows} that
\RC singular matrix satisfies to condition
	\begin{align}
	\label{eq: CR, row, 2 1, 1 1}
a_{\gi 2}^{\gi 1}&=b a_{\gi 1}^{\gi 1}\\
	\label{eq: CR, row, 2 2, 1 2}
a_{\gi 2}^{\gi 2}&=b a_{\gi 1}^{\gi 2}\\
	\label{eq: CR, column, 1 2, 1 1}
a_{\gi 1}^{\gi 2}&=a_{\gi 1}^{\gi 1} c\\
	\label{eq: CR, column, 2 2, 2 1}
a_{\gi 2}^{\gi 2}&=a_{\gi 2}^{\gi 1} c
	\end{align}
If we substitute \eqref{eq: CR, column, 1 2, 1 1}
into \eqref{eq: CR, row, 2 2, 1 2} we get
	\begin{equation}
	\label{eq: CR, a22, 2}
a_{\gi 2}^{\gi 2}=b a_{\gi 1}^{\gi 1} c
	\end{equation}
$b$ and $c$ are arbitrary elements of skew field $D$ and \RC singular matrix matrix
\eqref{eq: CR-singular matrix, 1} has form ($d=a_{\gi 1}^{\gi 1}$)
	\begin{equation}
a=
\left(
 \begin{array}{ccc}
d 
&
d c
\\
b d 
&
b d c
\end{array}
\right)
	\label{eq: RC-singular matrix, 2}
	\end{equation}
The similar way we can show that \CR singular matrix
has form
	\begin{equation}
a=
\left(
 \begin{array}{ccc}
d 
&
c' d
\\
d  b'
&
c' d b'
\end{array}
\right)
	\label{eq: CR-singular matrix, 2}
	\end{equation} 
From assumption it follows that \eqref{eq: CR-singular matrix, 2}
and \eqref{eq: RC-singular matrix, 2} represent the same matrix.
Comparing \eqref{eq: CR-singular matrix, 2}
and \eqref{eq: RC-singular matrix, 2} we get that
for every $d,c\in D$ exists such $c'\in D$ which does not depend on $d$ and
satisfies equation
\[d c=c'd\]
This contradicts the fact that $D$ is skew field.
		\end{proof}

		\begin{example}
Since we get skew field of quaternions  we assume $b=1+k$, $c=j$, $d=k$.
Then we get\footnote{I put calculation in file Vector.Space.English.tex.}
\[
a=\left(
 \begin{array}{ccc}
k
&
k j 
\\
(1+k) k 
&
(1+k) k j
\end{array}
\right)
=\left(
 \begin{array}{ccc}
k
&
-i
\\
k-1 
&
-i-j
\end{array}
\right)
\]
	\begin{align*}
\RCDet{a}^{\gi 2}_{\gi 2}
&=a_{\gi 2}^{\gi 2}
-a_{\gi 2}^{\gi 1}
(a_{\gi 1}^{\gi 1})^{-1} a_{\gi 1}^{\gi 2}
	\\
&=-i-j- (k-1)(k)^{-1} (-i)
	\\
%=-i-j-(k-1) k i
%=-i-j- k ki+ ki
%=-i-j+i +j
&=0
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 1}^{\gi 1}
&=a{}^{\gi 1}_{\gi 1}
-a^{\gi 1}_{\gi 2}(a^{\gi 2}_{\gi 2})^{-1}a^{\gi 2}_{\gi 1}
	\\
&=k
-(k-1) (-i-j)^{-1}(-i) 
	\\
%=k-(k-1)\frac 12 (i+j) (-i)
%=k+\frac 12 ((k-1)i+(k-1)j)i
%=k+\frac 12 (ki-i+kj-j)i
%=k+\frac 12 (j-i-i-j)i
%=k- ii
&=k+ 1
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 1}^{\gi 2}
&=a^{\gi 2}_{\gi 1}
-a^{\gi 2}_{\gi 1}(a^{\gi 1}_{\gi 2})^{-1}a^{\gi 2}_{\gi 1}
	\\
&=(-i)
-(-i) (k-1)^{-1} (-i)
	\\
%=-i+i\frac 12 (k+1) i
%=-i-\frac 12 (k+1) ii
%=-i+\frac 12(k+1)
&=-i+\frac 12k+\frac 12
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 2}^{\gi 1}
&=a^{\gi 1}_{\gi 2}
-a^{\gi 1}_{\gi 2}(a^{\gi 2}_{\gi 1})^{-1}a^{\gi 1}_{\gi 2}
	\\
&=(-i)
-(k-1) (-i)^{-1} (k-1)
	\\
%=(-i)-(k-1) i (k-1)
%=-i+i(k-1) (k-1) 
%=-i+i(k^2-2k+1)
%=-i-2ik
&=-i+2j
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 2}^{\gi 2}
&=a^{\gi 2}_{\gi 2}
-a^{\gi 2}_{\gi 1}
(a^{\gi 1}_{\gi 1})^{-1}a^{\gi 1}_{\gi 2}
	\\
&=-i-j
-(-i) (k)^{-1}(k-1)
	\\
%=-i-j-(k-1) k i
%=-i-j-k k i+ k i
%=-i-j+ i+ j
&=-2i
	\end{align*}
		\qed
		\end{example}

			\section{Dimension of \texorpdfstring{$D\RCstar$}{Drc}\hyph Vector Space}
			\label{section: Dimension of Vector Space}

		\begin{theorem}
		\label{theorem: basis of vector space}
Let $\mathcal{V}$ be a \drc vector space. Suppose $\mathcal{V}$ has
\drc bases $\Basis{e}=({}_{\gi a}\Vector{e},\gi{a}\in\gi{I})$
and $\Basis{g}=({}_{\gi b}\Vector{g}, \gi{b}\in\gi{J})$.
If $|\gi{I}|$ and $|\gi{J}|$ are finite numbers then $|\gi{I}|=|\gi{J}|$.
%If $|S|$ is finite number then $|\gi{J}|$ is finite number and $|\gi{I}|=|\gi{J}|$.
		\end{theorem}
		\begin{proof}
Suppose $|\gi{I}|=\gi m$ and $|\gi{J}|=\gi n$. Suppose
	\begin{equation}
\gi m<\gi n
	\label{eq: basis of vector space, 0}
	\end{equation}
Because $\Basis{e}$ is a \drc basis any
vector ${}_{\gi b}\Vector{g}$, $\gi{b}\in\gi{J}$
has expansion
	\[
{}_{\gi b}\Vector{g}={}_{\gi b}a\RCstar \Vector{e}
	\]
Because $\Basis{g}$ is a \drc basis
	\begin{equation}
\lambda=0
	\label{eq: basis of vector space, 1}
	\end{equation}
should follow from
	\[
\lambda\RCstar \Vector{g}
=\lambda\RCstar a\RCstar \Vector{e}=0
	\]
Because $\Basis{e}$ is a \drc basis we get
	\begin{equation}
\lambda\RCstar a=0
	\label{eq: 2 bases, vector space}
	\end{equation}
According to \eqref{eq: basis of vector space, 0}
$\RCRank a\le\gi2 m$ and system \eqref{eq: 2 bases, vector space}
has more variables then equations. According to
theorem \ref{theorem: left system of linear equations, solution}
$\lambda\ne 0$. This contradicts
statement \eqref{eq: basis of vector space, 1}. 
Therefore, statement $\gi m<\gi n$ is not valid.

In the same manner we can prove that the statement $\gi n<\gi m$ is not valid.
This completes the proof of the theorem.
		\end{proof}

		\begin{definition}
We call \AddIndex{dimension of \drc vector space}{dimension of vector space}
the number of vectors in a basis
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: coordinate matrix of basis}
The coordinate matrix of \drc basis $\Basis{g}$ relative \drc basis $\Basis{e}$ of
vector space $\mathcal{V}$ is \RC nonsingular matrix.
		\end{theorem}
		\begin{proof}
According to theorem \ref{theorem: rank of coordinate matrix}
\drc rank of the coordinate matrix of basis $\Basis{g}$ relative basis $\Basis{e}$
equal to the dimension of vector space. This proves the statement of the theorem.
		\end{proof}

		\begin{definition}
We call one-to-one map $\Vector A:\mathcal{A}\rightarrow \mathcal{B}$ 
\AddIndex{\drc isomorphism of vector spaces}{isomorphism of vector spaces}
if  this map is a \drc linear map of
vector spaces.
		\qed
		\end{definition}

		\begin{definition}
\AddIndex{\drc automorphism of vector space }{automorphism of vector space}
$\mathcal{V}$ is \drc isomorphism $\Vector A:\mathcal{V}\rightarrow \mathcal{V}$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: automorphism of vector space}
Suppose that $\Basis{f}$ is a \drc basis of vector space $\mathcal{V}$.
Then any \drc automorphism $\Vector A$ of vector space
$\mathcal{V}$ has form
	\begin{equation}
v'=v\RCstar  A
	\label{eq: automorphism, vector space}
	\end{equation}
where $A$ is a \RC nonsingular matrix.
		\end{theorem}
		\begin{proof}
\eqref{eq: automorphism, vector space} follows from
theorem \ref{theorem: drc linear map of drc vector space}.
Because $\Vector A$ is an isomorphism for each vector $\Vector v'$ exist one and only one vector $\Vector v$ such
that $\Vector v'=\Vector v\RCstar \Vector A$.
Therefore, system of \drc linear equations \eqref{eq: automorphism, vector space}
has a unique solution. According to corollary \ref{corollary: nonsingular rows system of linear equations}
matrix $A$
is a nonsingular matrix.
		\end{proof}

		\begin{theorem}
		\label{theorem: Automorphisms of vector space form a group}
Automorphisms of \drc vector space form a group $\RCGL nD$.
		\end{theorem}
		\begin{proof}
If we have two automorphisms $\Vector A$ and $\Vector B$ then we can write
	\begin{align*}
v'&=v\RCstar A\\
v''=v'\RCstar B&=v\RCstar A\RCstar B
	\end{align*}
Therefore, the resulting automorphism has matrix $A\RCstar B$.
		\end{proof}


==> Vector.Field.Russian.tex <==
%auto-ignore
\def\texVectorField{}
\ifx\PrintBook\Defined
				\chapter{Векторное поле над телом}
				\label{chapter: Vector Field Over Skew-Field}
\fi

			\section{Векторное поле над телом}
			\label{section: Vector Field Over Skew-Field}

Чтобы определить \Ts представление
	\[
\mathcal F:\mathcal R\rightarrow {}^\star \mathcal{V}
	\]
расслоенного кольца $\mathcal R$ на расслоении $\mathcal{V}$
мы должны определить структуру расслоенного кольца на расслоении
${}^\star \mathcal{V}$.

		\begin{theorem}
		\label{theorem: Ts representation of the ring}
\Ts представление $\mathcal F$
расслоенного кольца $\mathcal R$ на расслоении $\mathcal{V}$ определенно тогда и только
тогда, когда определены \Ts представления расслоенных мультипликативной и аддитивной групп
расслоенного кольца $\mathcal R$
и эти расслоенные \Ts представления удовлетворяют соотношению
\[
\mathcal F(a(b+c))=\mathcal F(a)\mathcal F(b)+\mathcal F(a)\mathcal F(c)
\]
		\end{theorem}
		\begin{proof}
Теорема следует из определения
\ref{definition: Tstar representation of fibered F-algebra}.
		\end{proof}

		\begin{theorem}
		\label{theorem: effective Ts representation of the fibered skew field}
\Ts представление расслоенного тела $\mathcal D$
\AddIndex{эффективно}{effective representation of fibered skew field},
если эффективно \Ts представление расслоенной мультипликативной группы тела $D$.
		\end{theorem}
		\begin{proof}
Согласно определениям \ref{definition: effective representation of fibered F-algebra}
и \ref{definition: isomorphism of fibered F-algebras} утверждение теоремы
проверяется в слое. В слое утверждение теоремы является следствием теоремы
\xRef{0701.238}{theorem: effective Ts representation of the skew field}.
		\end{proof}

Согласно замечанию
\ref{remark: notation for effective representation of fibered F-algebra},
если представление расслоенного тела эффективно, мы отождествляем сечение
расслоенного тела и соответствующее
ему \Ts преобразование.

		\begin{definition}
		\label{definition: Tstar vector field}
$\mathcal{V}$ - \AddIndex{$\mathcal D\star$\Hyph векторное расслоение}{Dstar vector bundle}
нaд расслоенным телом $\mathcal D$,
если $\mathcal{V}$ - расслоенная абелева группa и
определено эффективное \Ts представление расслоенного тела $\mathcal D$.
Сечение $\mathcal D\star$\Hyph векторного расслоения
называется \AddIndex{$\mathcal D\star$\Hyph векторным полем}{Dstar vector field}.
		\qed
		\end{definition} 

		\begin{theorem}
$\mathcal D\star$\Hyph векторного поля $\mathcal{V}$ удовлетворяют
соотношениям
\begin{itemize}
\item 
\AddIndex{закону ассоциативности}{associative law, Dstar vector field}
	\begin{equation}
	\label{eq: associative law, Dstar vector fields}
(ab)\Vector{m}=a(b\Vector{m})
	\end{equation}
\item 
\AddIndex{закону дистрибутивности}{distributive law, Dstar vector fields}
	\begin{align}
	\label{eq: distributive law, Dstar vector fields, 1}
a(\Vector{m}+\Vector{n})&=a\Vector{m}+a\Vector{n}\\
	\label{eq: distributive law, Dstar vector fields, 2}
(a+b)\Vector{m}&=a\Vector{m}+b\Vector{m}
	\end{align}
\item 
\AddIndex{закону унитарности}{unitarity law, Dstar vector fields}
	\begin{equation}
	\label{eq: unitarity law, Dstar vector fields}
1\Vector{m}=\Vector{m}
	\end{equation}
\end{itemize}
для любых $a, b \in \Gamma(\mathcal D)$, $\Vector{m}, \Vector{n} \in \Gamma(\mathcal{V})$.
Мы будем называть \Ts представление
\AddIndex{$\mathcal D\star$\Hyph произведением векторного поля на скаляр}
{Dstar product of vector field over scalar, vector space}.
		\end{theorem}
		\begin{proof}
Равенство \eqref{eq: distributive law, Dstar vector fields, 1} следует
из утверждения, что \Ts преобразование $a$ является автоморфизмом абелевой группы.
Равенство \eqref{eq: distributive law, Dstar vector fields, 2} следует
из утверждения, что \Ts представление является гомоморфизмом аддитивной группы
тела $D$.
Равенства \eqref{eq: associative law, Dstar vector fields} и
\eqref{eq: unitarity law, Dstar vector fields} следуют
из утверждения, что \Ts представление является ковариантным
\Ts представлением мультипликативной группы
тела $D$.
		\end{proof}

Согласно нашим обозначениям $D\star$\hyph векторное пространство -
это \AddIndex{левое векторное пространство}{left vector space} и
\AddIndex{$\star D$\hyph векторное пространство}{starD-vector space} -
это \AddIndex{правое векторное пространство}{right vector space}.

		\begin{definition}
Пусть $\mathcal{V}$ - $D\star$\hyph векторное пространство нaд кольцом $D$.
Множество векторов $\mathcal{N}$ -
\AddIndex{подпространство $D\star$\hyph векторного пространства}{subspace of Tstar vector space} $\mathcal{V}$,
если $\Vector{a}+\Vector{b}\in\mathcal{N}$
и $k\Vector{a}\in\mathcal{N}$ для любых
$\Vector{a}, \Vector{b} \in\mathcal{N}$ и для любого $k\in D$.
		\qed
		\end{definition}

		\begin{example}
		\label{example: matrices vector space}
Определим на множестве
\symb{D^{\gi m}_{\gi n}}1{matrices vector space}
$\gi m\times \gi n$
матриц над телом $D$
операцию сложения
	\[
a+b=
\left(a_{\gi i}^{\gi j}\right)
+
\left(b_{\gi i}^{\gi j}\right)
=
\left(a_{\gi i}^{\gi j}+b_{\gi i}^{\gi j}\right)
	\]
и умножения на скаляр
	\[
da=
d\left(a_{\gi i}^{\gi j}\right)
=
\left(da_{\gi i}^{\gi j}\right)
	\]
$a=0$ тогда и только тогда, когда $a_{\gi i}^{\gi j}=0$ для любых ${\gi i}$, ${\gi j}$.
Непосредственная проверка показывает, что
$D^{\gi m}_{\gi n}$ является $D\star$\hyph векторным пространством,
если произведение действует слева.
В противном случае $D^{\gi m}_{\gi n}$
- $\star D$\hyph векторное пространство.
Мы будем называть векторное пространство $D^{\gi m}_{\gi n}$
\AddIndex{$D\star$\hyph векторным пространством матриц}{matrices vector space}.
		\qed
		\end{example}

			\section{Тип векторного пространства}
			\label{section: vector space type}

Произведение вектора на скаляр асимметрично,
так как произведение определено для объектов разных множеств.
Однако различие между $D\star$\hyph\ и $\star D$\hyph векторным пространством появляется только тогда,
когда мы переходим к координатному представлению.
Говоря, векторное пространство является $D\star$\hyph\ или $\star D$\hyph, мы указываем,
с какой стороны, слева или справа, мы умножаем координаты
вектора на элементы тела.

		\begin{definition}
Допустим $u$, $v$ - векторы левого векторного пространства $\mathcal{V}$. Мы будем
говорить, что вектор $w$ является
\AddIndex{$D\star$\hyph линейной комбинацией векторов}{linear composition of  vectors} $u$ и $v$,
если мы можем записать $w=au+bv$, где $a$ и $b$ - скаляры.
		\qed
		\end{definition}

Мы можем распространить понятие линейной комбинации на любое конечное семейство
векторов. Пользуясь обобщённым индексом для нумерации векторов, мы
можем представить семейство векторов в виде одномерной матрицы.
Мы пользуемся соглашением, что в заданном векторном пространстве мы представляем любое семейство
векторов либо в виде \subs строки, либо \sups строки.
Это представление
определяет характер записи линейной комбинации.
Рассматривая это представление в $D\star$- или $\star D$\hyph векторном пространстве, мы
получаем четыре разных модели векторного пространства.

Чтобы иметь возможность,
не меняя записи указать, является векторное пространство
$D\star$- или $\star D$\hyph векторным пространством, мы вводим новое обозначение.
Символ \symb{D\star}1{vector space type}\ называется \AddIndex{типом векторного пространства}{vector space type} и
означает, что мы изучаем $D\star$\hyph векторное пространство над телом $D$.
Операция умножения в типе векторного пространства указывает на матричную операцию, используемую в
линейной комбинации.

		\begin{example}
Представим множество векторов
${}_{\gi a}\Vector{a}$, $\gi{a}\in\gi{I}$
\AddIndex{\drc векторного пространства}{drc vector space} $\mathcal{V}$
в виде \subs строки
\[
\Vector{a}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{a} \\
...  \\
{}_{\gi n}\Vector{a}
\end{array}\right)
\]
и множество скаляров
$c^{\gi a}$, $\gi{a}\in\gi{I}$
в виде \sups строки
\[
c
=\left(\begin{array}{ccc}
c^{\gi 1} &
...  &
c^{\gi n}
\end{array}\right)
\]
Тогда мы можем записать линейную комбинацию векторов ${}_{\gi a}\Vector{a}$ в виде
\[c^{\gi a}\ {}_{\gi a}\Vector{a}=c\RCstar\Vector{a}\]
Мы пользуемся записью \symb{{}_{D\RCstar}\mathcal{V}}1{left RC vector space},
когда мы хотим сказать, что $\mathcal{V}$ - \drc векторное пространство.
		\qed
		\end{example}

		\begin{example}
Представим множество векторов
${}^{\gi a}\Vector{a}$, $\gi{a}\in\gi{I}$
\AddIndex{\dcr векторного пространства}{dcr vector space} $\mathcal{V}$
в виде \sups строки
\[
\Vector{a}
=\left(\begin{array}{ccc}
{}^{\gi 1}\Vector{a}&
... &
{}^{\gi n}\Vector{a}
\end{array}\right)
\]
и множество скаляров
$c_{\gi a}$, $\gi{a}\in\gi{I}$
в виде \subs строки
\[
c
=\left(\begin{array}{ccc}
c_{\gi 1} \\
...  \\
c_{\gi n}
\end{array}\right)
\]
Тогда мы можем записать линейную комбинацию векторов ${}^{\gi a}\Vector{a}$ в виде
\[c_{\gi a}\ {}^{\gi a}\Vector{a}=c\CRstar\Vector{a}\]
Мы пользуемся записью \symb{{}_{D\CRstar}\mathcal{V}}1{left CR vector space},
когда мы хотим сказать, что $\mathcal{V}$ - \dcr векторное пространство.
		\qed
		\end{example}

		\begin{example}
Представим множество векторов
$\Vector{a}_{\gi a}$, $\gi{a}\in\gi{I}$
\AddIndex{\crd векторного пространства}{crd vector space} $\mathcal{V}$
в виде \subs строки
\[
\Vector{a}
=\left(\begin{array}{ccc}
\Vector{a}_{\gi 1} \\
...  \\
\Vector{a}_{\gi n}
\end{array}\right)
\]
и множество скаляров
${}^{\gi a}c$, $\gi{a}\in\gi{I}$
в виде \sups строки
\[
c
=\left(\begin{array}{ccc}
{}^{\gi 1}c &
...  &
{}^{\gi n}c
\end{array}\right)
\]
Тогда мы можем записать линейную комбинацию векторов $\Vector{a}_{\gi a}$ в виде
\[\Vector{a}_{\gi a}\ {}^{\gi a}c=\Vector{a}\CRstar c\]
Мы пользуемся записью \symb{\mathcal{V}_{\CRstar D}}1{right CR vector space},
когда мы хотим сказать, что $\mathcal{V}$ - \crd векторное пространство.
		\qed
		\end{example}

		\begin{example}
Представим множество векторов
$\Vector{a}^{\gi a}$, $\gi{a}\in\gi{I}$
\AddIndex{\rcd векторного пространства}{rcd vector space} $\mathcal{V}$
в виде \sups строки
\[
\Vector{a}
=\left(\begin{array}{ccc}
\Vector{a}^{\gi 1}&
... &
\Vector{a}^{\gi n}
\end{array}\right)
\]
и множество скаляров
${}_{\gi a}c$, $\gi{a}\in\gi{I}$
в виде \subs строки
\[
c
=\left(\begin{array}{ccc}
{}_{\gi 1}c \\
...  \\
{}_{\gi n}c
\end{array}\right)
\]
Тогда мы можем записать линейную комбинацию векторов $\Vector{a}^{\gi a}$ в виде
\[\Vector{a}^{\gi a}\ {}_{\gi a}c=\Vector{a}\RCstar c\]
Мы пользуемся записью \symb{\mathcal{V}_{\RCstar D}}1{right RC vector space},
когда мы хотим сказать, что $\mathcal{V}$ - \rcd векторное пространство.
		\qed
		\end{example}

		\begin{remark}
		\label{remark: left and right vector space notation}
Мы распространим на векторное пространство и его тип соглашение,
описанное в замечании
\xRef{0612.111}{remark: left and right matrix notation}.
Например, в выражении
\[A\RCstar B\RCstar v\lambda\]
мы выполняем операцию умножения слева направо. Это соответствует
\rcd векторному пространству. Однако мы можем выполнять операцию умножения
справа налево. В традиционной записи это выражение примет вид
\[\lambda v\CRstar B\CRstar A\]
и будет соответствовать \dcr векторному пространству. Аналогично, читая выражение
снизу вверх мы получим выражение
\[A\CRstar B\CRstar v\lambda\]
соответствующего \crd векторному пространству.
		\qed
		\end{remark}

			\section{\texorpdfstring{$D\RCstar$}{Drc}-базис векторного пространства}
			\label{section: Basis of Vector Space}

		\begin{definition}
Векторы ${}_{\gi a}\Vector{a}$, $\gi{a}\in\gi{I}$ \drc векторного пространства
$\mathcal{V}$ \AddIndex{\drc линейно независимы}
{linearly independent, vector space},
если $c=0$ следует из уравнения
\[c\RCstar\Vector{a}=0\]
В противном случае, векторы ${}_{\gi a}\Vector{a}$
\AddIndex{\drc линейно зависимы}{linearly dependent, vector space}.
		\qed
		\end{definition}

		\begin{definition}
Множество векторов
\symb{\Basis{e}=({}_{\gi a}\Vector{e},\gi{a}\in \gi{I})}1
{basis, vector space}
- \AddIndex{\drc базис векторного пространства}{drc basis, vector space},
если векторы ${}_{\gi a}\Vector{e}$ \drc линейно независимы и добавление
любого вектора к этой системе
делает эту систему \drc линейно зависимой.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: expansion relative basis, vector space}
Если $\Basis{e}$ - \drc базис векторного пространства $\mathcal{V}$,
то любой вектор $\Vector{v}\in \mathcal{V}$
имеет одно и только одно разложение
	\begin{equation}
\Vector{v}=v\RCstar\Vector{e}
	\label{eq: expansion relative basis, vector space}
	\end{equation}
относительно этого \drc базиса.
		\end{theorem}
		\begin{proof}
Так как система векторов ${}_{\gi a}\Vector{e}$ является
максимальным множеством \drc линейно независимых векторов,
система векторов $\Vector{v},{}_{\gi a}\Vector{e}$
- \drc линейно зависима и в уравнении
	\begin{equation}
b\Vector{v}+c\RCstar\Vector{e}=0
	\label{eq: expansion relative basis, vector space, 1}
	\end{equation}
по крайней мере $b$ отлично от $0$. Тогда равенство
	\begin{equation}
\Vector{v}=(-b^{-1}c)\RCstar\Vector{e}
	\label{eq: expansion relative basis, vector space, 2}
	\end{equation}
следует из \eqref{eq: expansion relative basis, vector space, 1}.
\eqref{eq: expansion relative basis, vector space} следует
из \eqref{eq: expansion relative basis, vector space, 2}.

Допустим мы имеем другое разложение
	\begin{equation}
\Vector{v}=v'\RCstar\Vector{e}
	\label{eq: expansion relative basis, vector space, 3}
	\end{equation}
Вычтя \eqref{eq: expansion relative basis, vector space}
из \eqref{eq: expansion relative basis, vector space, 3},
мы получим
	\[
0=(v'-v)\RCstar\Vector{e}
	\]
Так как векторы ${}_{\gi a}\Vector{e}$ \drc линейно независимы, мы имеем
\[v'-v=0\]
		\end{proof}

		\begin{definition}
Мы будем называть матрицу
$v$ разложения \eqref{eq: expansion relative basis, vector space}
\AddIndex{координатной матрицей вектора $\Vector{v}$ в \drc базисе $\Basis{e}$}
{coordinate matrix of vector in drc basis}
и её элементы
\AddIndex{координатами вектора $\Vector{v}$ в \drc базисе $\Basis{e}$}
{coordinates of vector in drc basis}.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: coordinate vector space}
Множество координат $a$ вектора $\Vector{a}$ в \drc базисе $\Basis{e}$
порождают \drc векторное пространство \symb{D^{\gi n}}1{drc coordinate vector space},
изоморфное \drc векторному пространству $\mathcal{V}$.
Это \drc векторное пространство называется
\AddIndex{\drc координатным векторным пространством}
{drc coordinate vector space},
а изоморфизм
\AddIndex{координатным изоморфизмом}{coordinate isomorphism}.
		\end{theorem}
		\begin{proof}
Допустим векторы $\Vector{a}$ и $\Vector{b}\in\mathcal{V}$ имеют разложение
\[
\Vector{a}=a\RCstar \Vector{e}
\]
\[
\Vector{b}=b\RCstar \Vector{e}
\]
в базисе $\Basis{e}$. Тогда
\[
\Vector{a}+\Vector{b}=
a\RCstar \Vector{e}+b\RCstar \Vector{e}
=(a+b)\RCstar\Vector{e}
\]
\[
m\Vector{a}=m(a\RCstar \Vector{e})=(ma)\RCstar\Vector{e}
\]
для любого $m\in S$.
Таким образом, операции в векторном пространстве определены по координатно
\[
(a+b)^{\gi a}=a^{\gi a}+b^{\gi a}
\]
\[
(ma)^{\gi a}=ma^{\gi a}
\]
Это доказывает теорему.
		\end{proof}

		\begin{example}
		\label{example: drc vector space}
Пусть $\Basis{e}=({}_{\gi i}\Vector{e},\gi i\in \gi I,|\gi I|=\gi n)$
- \drc базис векторного пространства $D^{\gi n}$.
координатная матрица
\symb{a= \left(\begin{array}{ccc}
a^{\gi 1} &
... &
a^{\gi n}
\end{array}\right)}0{drc vector}
\[
\ShowSymbol{drc vector}
=(a^{\gi i},\gi i\in\gi I)
	\]
вектора $\Vector{a}$ в \drc базисе $\Basis{e}$
называется \AddIndex{\drc вектором}{drc vector}.\footnote{\drc вектор
является аналогом вектор\hyph строки. Мы можем называть его также $D\star$\Hyph вектор \sups строкой}
Мы будем называть векторное пространство
\symb{D^{\gi n}}1{r rows drc vector space}
\AddIndex{\drc векторным пространством \sups строк}{sups rows drc vector space}.

Пусть \subs строка
	\begin{equation}
	\label{eq: subs row, vectors}
\Vector{a}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{a} \\
...  \\
{}_{\gi m}\Vector{a}
\end{array}\right)
=({}_{\gi i}\Vector{a},\gi i\in\gi M)
	\end{equation}
задаёт множество векторов.
Векторы ${}_{\gi a}\Vector{a}$ имеют разложение
	\[
{}_{\gi a}\Vector{a}={}_{\gi a}a\RCstar\Vector{f}
	\]
Если мы подставим координатные матрицы вектора ${}_{\gi i}\Vector{a}$ в
матрицу \eqref{eq: subs row, vectors}, мы получим матрицу
\[
a
=\left(\begin{array}{ccc}
\left(\begin{array}{ccc}
{}_{\gi 1}a^{\gi 1} &
... &
{}_{\gi 1}a^{\gi n}
\end{array}\right) \\
...  \\
\left(\begin{array}{ccc}
{}_{\gi m}a^{\gi 1} &
... &
{}_{\gi m}a^{\gi n}
\end{array}\right)
\end{array}\right)
=\left(\begin{array}{ccc}
{}_{\gi 1}a^{\gi 1} &
... &
{}_{\gi 1}a^{\gi n} \\
...&...&...  \\
{}_{\gi m}a^{\gi 1} &
... &
{}_{\gi m}a^{\gi n}
\end{array}\right)
=({}_{\gi i}a^{\gi j})
\]
Мы будем называть матрицу $a$
\AddIndex{координатной матрицей множества векторов}{coordinate matrix of set of vectors, drc vector space}
$({}_{\gi i}\Vector{a},\gi i\in\gi M)$ в базисе $\Basis{e}$
и её элементы
\AddIndex{координатами множества векторов}{coordinates of set of vectors, drc vector space}
$({}_{\gi i}\Vector{a},\gi i\in\gi M)$ в базисе $\Basis{e}$.

Мы будем представлять
\AddIndex{\drc базис $\Basis{f}$ векторного пространства \sups строк}
{drc basis, r rows vector space}
$D^{\gi n}$
в форме \subs строки
\symb{\Vector{f}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{f} \\
...  \\
{}_{\gi n}\Vector{f}
\end{array}\right)}0{basis, r rows drc vector space}
\[
\ShowSymbol{basis, r rows drc vector space}
=({}_{\gi i}\Vector{f},\gi i\in\gi I)
\]
Мы будем говорить, что координатная матрица $f$ множества векторов
$({}_{\gi i}\Vector{f},\gi i\in\gi I)$ определяет координаты
\symb{{}_{\gi i}f^{\gi j}}1{basis coordinates, r rows drc vector space}
базиса $\Basis{f}$ относительно базиса $\Basis{e}$.
		\qed
		\end{example}

		\begin{example}
		\label{example: dcr vector space}
Пусть $\Basis{e}=({}^{\gi i}\Vector{e},\gi i\in\gi I,|\gi I|=\gi n)$
- \dcr базис векторного пространства $D_{\gi n}$.
координатная матрица
\symb{a= \left(\begin{array}{ccc}
a_{\gi 1} \\
...  \\
a_{\gi n}
\end{array}\right)}0{dcr vector}
\[
\ShowSymbol{dcr vector}
=(a_{\gi i},\gi i\in\gi I)
	\]
вектора $\Vector{a}$ в \dcr базисе $\Basis{e}$
называется \AddIndex{\dcr вектором}{dcr vector}.\footnote{\dcr вектор
является аналогом вектор\hyph столбца. Мы можем называть его также $D\star$\Hyph вектор \subs строкой}
Мы будем называть векторное пространство
\symb{D_{\gi n}}1{c rows dcr vector space}
\AddIndex{\dcr векторным пространством \subs строк}{subs rows dcr vector space}.

Пусть \sups строка
	\begin{equation}
	\label{eq: sups row, vectors}
\Vector{a}
=\left(\begin{array}{ccc}
{}^{\gi 1}\Vector{a} &
...  &
{}^{\gi m}\Vector{a}
\end{array}\right)
=({}^{\gi i}\Vector{a},\gi i\in\gi M)
	\end{equation}
задаёт множество векторов.
Векторы ${}^{\gi a}\Vector{a}$ имеют разложение
	\[
{}^{\gi a}\Vector{a}={}^{\gi a}a\CRstar\Vector{f}
	\]
Если мы подставим координатные матрицы вектора ${}^{\gi i}\Vector{a}$ в
матрицу \eqref{eq: sups row, vectors}, мы получим матрицу
\[
a
= \left(\begin{array}{ccc}
\left(\begin{array}{ccc}
{}^{\gi 1}a_{\gi 1} \\
...  \\
{}^{\gi 1}a_{\gi n}
\end{array}\right) &
... &
\left(\begin{array}{ccc}
{}^{\gi m}a_{\gi 1} \\
...  \\
{}^{\gi m}a_{\gi n}
\end{array}\right)
\end{array}\right)
= \left(\begin{array}{ccc}
{}^{\gi 1}a_{\gi 1}&...&{}^{\gi m}a_{\gi 1} \\
... &...&... \\
{}^{\gi 1}a_{\gi n}&...&{}^{\gi m}a_{\gi n}
\end{array}\right)
=({}^{\gi i}a_{\gi j})
\]
Мы будем называть матрицу $a$
\AddIndex{координатной матрицей множества векторов}{coordinate matrix of set of vectors, dcr vector space}
$({}^{\gi i}\Vector{a},\gi i\in\gi M)$ в базисе $\Basis{e}$
и её элементы
\AddIndex{координатами множества векторов}{coordinates of set of vectors, dcr vector space}
$({}^{\gi i}\Vector{a},\gi i\in\gi M)$ в базисе $\Basis{e}$.

Мы будем представлять
\AddIndex{\dcr базис $\Basis{f}$ векторного пространства \subs строк}
{dcr basis, c rows vector space}
$D_{\gi n}$
в форме \sups строки
\symb{\Vector{f}
= \left(\begin{array}{ccc}
{}^{\gi 1}\Vector{f} &
... &
{}^{\gi n}\Vector{f}
\end{array}\right)}0{basis, c rows dcr vector space}
\[
\ShowSymbol{basis, c rows dcr vector space}
=({}^{\gi i}\Vector{f},\gi i\in \gi I)
\]
Мы будем говорить, что координатная матрица $f$ множества векторов
$({}^{\gi i}\Vector{f},\gi i\in \gi I)$ определяет координаты
\symb{{}^{\gi i}f_{\gi j}}1{basis coordinates, c rows dcr vector space}
базиса $\Basis{f}$ относительно базиса $\Basis{e}$.
		\qed
		\end{example}

Так как мы линейную комбинацию выражаем с помощью матриц, мы можем
распространить принцип двойственности на теорию векторных пространств.
Мы можем записать принцип двойственности в одной из следующих форм

		\begin{theorem}[принцип двойственности]
		\label{theorem: duality principle}
Пусть $\mathfrak{A}$ - истинное утверждение о векторных пространствах.
Если мы заменим одновременно
\begin{itemize}
\item \drc вектор и \dcr вектор
\item \rcd вектор и \crd вектор
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
		\end{theorem}

		\begin{theorem}[принцип двойственности]
%		\label{theorem: duality principle, quasideterminants}
Пусть $\mathfrak{A}$ - истинное утверждение о векторных пространствах.
Если мы одновременно заменим
\begin{itemize}
\item \drc вектор и \rcd вектор или \dcr вектор и \crd вектор
\item \RC квазидетерминант и \CR квазидетерминант
\end{itemize}
то мы снова получим истинное утверждение.
		\end{theorem}

\input{Drc.Morphism.Russian}

			\section{Система \texorpdfstring{$D\RCstar$}{Drc}\hyph линейных уравнений}
			\label{section: System of Linear Equations}

		\begin{definition}
		\label{definition: linear span, vector space}
Пусть $\mathcal{V}$ - \drc векторное пространство и
$\{{}_{\gi a}\Vector{a}\in\mathcal{V}, \gi{a}\in\gi{I}\}$ - множество векторов.
\AddIndex{\drc линейная оболочка в векторном пространстве}{linear span, vector space}
- это множество
\symb{\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})}1{linear span, vector space}
векторов, \drc линейно зависимых от векторов ${}_{\gi a}\Vector{a}$.
		\qed
		\end{definition}

		\begin{theorem}
Пусть $\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})$ - \drc линейная оболочка в
векторном пространстве $\mathcal{V}$.
Тогда $\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})$
- подпространство векторного пространства $\mathcal{V}$.
		\end{theorem}
		\begin{proof}
Предположим, что
	\begin{align*}
\Vector{b}&\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})\\
\Vector{c}&\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{I})
	\end{align*}
Согласно определению \ref{definition: linear span, vector space}
	\begin{align*}
\Vector{b}&=b\RCstar \Vector{a}\\
\Vector{c}&=c\RCstar \Vector{a}
	\end{align*}
Тогда
	\begin{align*}
\Vector{b}+\Vector{c}
=b\RCstar\Vector{a}+c\RCstar\Vector{a}
=(b+c)\RCstar\Vector{a}
&\in\text{span}(\Vector{a}_{\gi a},\gi{a}\in\gi{I})\\
k\Vector{b}=k(b\RCstar\Vector{a})=(kb)\RCstar\Vector{a}
&\in\text{span}(\Vector{a}_{\gi a},\gi{a}\in\gi{I})
	\end{align*}
Это доказывает утверждение.
		\end{proof}

Пусть $\mathcal{V}$ - \drc векторное пространство и
\subs строка
	\begin{equation}
	\label{eq: linear span, vectors}
\Vector{a}
=\left(\begin{array}{ccc}
{}_{\gi 1}\Vector{a} \\
...  \\
{}_{\gi n}\Vector{a}
\end{array}\right)
=({}_{\gi i}\Vector{a},\gi i\in\gi M)
	\end{equation}
задаёт множество векторов.
Чтобы ответить на вопрос, или вектор
$\Vector{b}\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{M})$,
мы запишем линейное уравнение
	\begin{equation}
\Vector{b}=x\RCstar\Vector{a}
	\label{eq: linear span, vector space, 1}
	\end{equation}
где
\[
x=\left(
 \begin{array}{ccc}
x^{\gi 1}&...&x^{\gi m}
\end{array}
\right)
\]
\sups строка неизвестных коэффициентов разложения.
$\Vector{b}\in\text{span}({}_{\gi a}\Vector{a},\gi{a}\in\gi{M})$,
если уравнение \eqref{eq: linear span, vector space, 1}
имеет решение.
Предположим, что $\Basis{f}=({}_{\gi b}\Vector{f},\gi{b}\in\gi{N})$ - \drc базис.
Тогда векторы $\Vector{b}$, ${}_{\gi a}\Vector{a}$ имеют разложение
	\begin{align}
	\label{eq: linear span, vector space, b}
\Vector{b}&=b\RCstar\Vector{f}\\
	\label{eq: linear span, vector space, ai}
{}_{\gi a}\Vector{a}&={}_{\gi a}a\RCstar\Vector{f}
	\end{align}
Если мы подставим \eqref{eq: linear span, vector space, b}
и \eqref{eq: linear span, vector space, ai}
в \eqref{eq: linear span, vector space, 1}, мы получим
	\begin{equation}
b\RCstar\Vector{f}=x\RCstar a\RCstar\Vector{f}
	\label{eq: linear span, vector space, 2}
	\end{equation}
Применяя теорему \ref{theorem: expansion relative basis, vector space}
к \eqref{eq: linear span, vector space, 2}, мы получим
\AddIndex{систему \drc линейных уравнений}
{system of linear equations}
	\begin{equation}
	\label{eq: system of linear equations}
x\RCstar a=b
	\end{equation}

Мы можем записать систему \drc линейных уравнений
\eqref{eq: system of linear equations} в одной из следующих форм
\[
\left(
 \begin{array}{ccc}
x^{\gi 1}&...&x^{\gi m}
\end{array}\right)
\RCstar \left(
 \begin{array}{ccc}
{}_{\gi 1}a^{\gi 1} & ... & {}_{\gi 1}a^{\gi n}\\
... & ... & ... \\
{}_{\gi m}a^{\gi 1} &...& {}_{\gi m}a^{\gi n}
\end{array}
\right)=\left(
 \begin{array}{ccc}
b^{\gi 1}&...&b^{\gi m}
\end{array}
\right)
\]
	\begin{equation}
	\label{eq: star columns system of linear equations}
x^{\gi a}\ {}_{\gi a}a^{\gi b}=b^{\gi b}
	\end{equation}
	\[
\begin{array}{ccc}
x^{\gi 1}\ {}_{\gi 1}a^{\gi 1} & ... & x^{\gi 1}\ {}_{\gi 1}a^{\gi n}\\
+& ... & +\\
... & ... & ... \\
+& ... & +\\
x^{\gi m}\ {}_{\gi m}a^{\gi 1} &...& x^{\gi m}\ {}_{\gi m}a^{\gi n} \\
=& ... & =\\
b^{\gi 1} &...& b^{\gi n} 
\end{array}
	\]

Пусть $\mathcal{V}$ - \dcr векторное пространство.
Читая систему \eqref{eq: system of linear equations} \drc линейных уравнений снизу вверх,
мы получим систему \dcr линейных уравнений
\[
x^\CRstar a=b
\]
которую можем записать в одной из следующих форм
\[
x\CRstar a=b
\]
\[
\left(
 \begin{array}{ccc}
x_{\gi 1}\\...\\x_{\gi n}
\end{array}\right)
\CRstar \left(
 \begin{array}{ccc}
{}^{\gi 1}a_{\gi 1} &...& {}^{\gi n}a_{\gi 1}\\
... & ... & ... \\
{}^{\gi 1}a_{\gi m} &...& {}^{\gi n}a_{\gi m}
\end{array}
\right)=\left(
 \begin{array}{ccc}
b_{\gi 1}\\...\\ b_{\gi m}
\end{array}
\right)
\]
	\begin{equation}
	\label{eq: star rows system of linear equations}
x_{\gi a}\ {}^{\gi a}a_{\gi b}=b_{\gi b}
	\end{equation}
	\[
\begin{array}{cccc}
x_{\gi 1}\ {}^{\gi 1}a_{\gi 1} &+...&+ x_{\gi n}\ {}^{\gi n}a_{\gi 1}&=b_{\gi 1}\\
... & ... & ...& ... \\
x_{\gi 1}\ {}^{\gi 1}a_{\gi m} &+...&+ x_{\gi n}\ {}^{\gi n}a_{\gi m}&=b_{\gi m}
\end{array}
	\]

		\begin{definition}
Предположим, что $a$
- \RC невырожденная матрица. Мы будем называть соответствующую систему
	\begin{equation}
	\label{eq: nonsingular system of linear equations}
x\RCstar a=b
	\end{equation}
\AddIndex{невырожденной системой \drc линейных уравнений}
{nonsingular system of linear equations}.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: nonsingular system of linear equations}
Решение невырожденной системы \drc линейных уравнений
\eqref{eq: nonsingular system of linear equations} определено однозначно
и может быть записано в любой из следующих форм\footnote{Мы можем найти решение системы
\eqref{eq: nonsingular system of linear equations}
в теореме
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
Я повторяю это утверждение, так как я слегка изменил обозначения.
\label{footnote: nonsingular system of linear equations}}
	\begin{align}
	\label{eq: nonsingular system of linear equations, solution, matrix}
x&=b\RCstar a^{\RCInverse}\\
	\label{eq: nonsingular system of linear equations, solution, quasideterminant}
x&=b\RCstar \mathcal{H}\RCDet{a}
	\end{align}
		\end{theorem}
		\begin{proof}
Умножая обе части равенства \eqref{eq: nonsingular system of linear equations}
справа на $a^{\RCInverse}$, мы получим
\eqref{eq: nonsingular system of linear equations, solution, matrix}.
Пользуясь определением
\xEqRef{0612.111}{eq: RC-quasideterminant definition},
мы получим \eqref{eq: nonsingular system of linear equations, solution, quasideterminant}.
Решение системы единственно в силу теоремы
\xEqRef{0612.111}{theorem: two products equal}.
		\end{proof}

			\section{Ранг матрицы}
			\label{section: Rank of Matrix}

		\begin{definition}
Мы будем называть матрицу\footnote{Мы
делаем следующие предположения в этом разделе
\begin{itemize}
\item $\gi{a}\in\gi{M}$, $|\gi{M}|=\gi m$, $\gi{b}\in\gi{N}$, $|\gi{N}|=\gi n$.
\item $A=({}_{\gi a}A^{\gi b})$ - произвольная матрица.
\item $\gi k$, $\gi{s}\in \gi{S}\supseteq \gi{M}$,
$\gi l$, $\gi{t}\in \gi{T}\supseteq \gi{N}$, $\gi k=|\gi{S}|=|\gi{T}|$.
\item $\gi{p}\in\gi{M}\setminus\gi S$, $\gi{r}\in\gi{N}\setminus\gi{T}$.
\end{itemize}
\label{footnote: index assumption}}
${}_{\gi S}A^{\gi T}$ минором порядка $\gi k$.
		\qed
		\end{definition}

		\begin{definition}
Если $\gi n\times \gi n$ матрица $A$ имеет \RC обратную матрицу,
мы будем называть такую матрицу
\AddIndex{\RC невырожденной матрицей}{RC nonsingular matrix}.
В противном случае, мы будем называть такую матрицу
\AddIndex{\RC вырожденной матрицей}{RC singular matrix}.
		\qed
		\end{definition}

		\begin{definition}
Если минор ${}_{\gi S}A^{\gi T}$ - \RC невырожденная матрица,
то мы будем говорить, что
\RC ранг матрицы $A$ не меньше, чем $\gi k$.
\AddIndex{\RC ранг матрицы $A$}{rc-rank of matrix}
\symb{\RCRank A}2{rc-rank of matrix}%
- это максимальное значение $\gi k$.
Мы будем называть соответствующий минор \AddIndex{\RC главным минором}{RC-major minor}.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: singular matrix and quasideterminant}
Пусть матрица $A$ - \RC вырожденная матрица и минор ${}_{\gi S}A^{\gi T}$
- главный минор, тогда
	\begin{equation}
	\label{eq: singular matrix and quasideterminant}
{}_{\gi p}\RCDet{{}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}}^{\gi r}=0
	\end{equation}
		\end{theorem}
		\begin{proof}
Чтобы понять, почему минор ${}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}$
не имеет \RC обратной матрицы,\footnote{Естественно ожидать связь между \RC вырожденностью матрицы
и её \RC квазидетерминантом, подобную связи, известной в коммутативном случае.
Однако \RC квазидетерминант определён не всегда. Например, если \RC обратная матрица
имеет слишком много элементов, равных $0$. Как следует из этой теоремы, не определён \RC квазидетерминант
также в случае, когда \RC ранг матрицы меньше $\gi{n-1}$.}
мы предположим, что он имеет \RC обратную матрицу
и запишем соответствующую систему
\xEqRef{0612.111}{eq: inverse minor,1},
\xEqRef{0612.111}{eq: inverse minor,2},
полагая $\gi I=\gi r$, $\gi J=\gi p$ и попробуем решить эту систему.
Положив
	\begin{equation}
	\label{eq: singular matrix and quasideterminant, 0}
B={}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}
	\end{equation}
мы получим систему
	\begin{align}
	\label{eq: singular matrix and quasideterminant, 1}
{}_{\gi S}B^{\gi T}\RCstar
{}_{\gi T}B^{\RCInverse}{}^{\gi p}
+ {}_{\gi S}B^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=0\\
	\label{eq: singular matrix and quasideterminant, 2}
{}_{\gi p}B^{\gi T}\RCstar
{}_{\gi T}B^{\RCInverse}{}^{\gi p}
+{}_{\gi p}B^{\gi r}\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
Мы умножим \eqref{eq: singular matrix and quasideterminant, 1} на
$({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}$
	\begin{equation}
	\label{eq: singular matrix and quasideterminant, 3}
{}_{\gi T}B^{\RCInverse}{}^{\gi p}
+({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}\RCstar
{}_{\gi S}B^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}=0
	\end{equation}
Теперь мы можем подставить \eqref{eq: singular matrix and quasideterminant, 3} в
\eqref{eq: singular matrix and quasideterminant, 2}
	\begin{align}
	\label{eq: singular matrix and quasideterminant, 4}
-{}_{\gi p}B^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}\RCstar
{}_{\gi S}B^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}
+{}_{\gi p}B^{\gi r} \ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
Из \eqref{eq: singular matrix and quasideterminant, 4} следует
	\begin{align}
	\label{eq: singular matrix and quasideterminant, 5}
({}_{\gi p}B^{\gi r}-{}_{\gi p}B^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}B_\bullet{}^{\gi S}_-)^{\RCInverse}\RCstar
{}_{\gi S}B^{\gi r})
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
Выражение в скобках является квазидетерминантом
${}_{\gi p}\RCDet{B}^{\gi r}$.
Подставляя это выражение в \eqref{eq: singular matrix and quasideterminant, 5},
мы получим
	\begin{align}
	\label{eq: singular matrix and quasideterminant, 6}
{}_{\gi p}\RCDet{B}^{\gi r}
\ {}_{\gi r}B^{\RCInverse}{}^{\gi p}&=\delta
	\end{align}
Тем самым мы доказали, что квазидетерминант ${}_{\gi p}\RCDet{B}^{\gi r}$
определён и условие его обращения в $0$ необходимое и достаточное условие
вырожденности матрицы $B$. Теорема доказана в силу соглашения
\eqref{eq: singular matrix and quasideterminant, 0}.
		\end{proof}

		\begin{theorem}
		\label{theorem: rc rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$$\RCRank  A=\gi k<\gi m$$
и ${}_{\gi S}A^{\gi T}$ - \RC главный минор.
Тогда \sups строка ${}_{\gi p}A$ является
\drc линейной комбинацией \sups строк ${}_{\gi s}A$.
	\begin{align}
	\label{eq: rc rank of matrix, sups-rows}
{}_{\gi{M}\setminus\gi S}A&=r\RCstar {}_{\gi S}A\\
	\label{eq: rc rank of matrix, sups-rows, 1}
{}_{\gi p}A&={}_{\gi p}r\RCstar {}_{\gi S}A\\
	\label{eq: rc rank of matrix, sups-rows, 2}
{}_{\gi p}A^{\gi b}&={}_{\gi p}r^{\gi s}\ {}_{\gi s}A^{\gi b}
	\end{align}
		\end{theorem}
		\begin{proof}
Если число \subs строк - $\gi k$, то, полагая, что \sups строка ${}_{\gi p}A$
- \drc линейная комбинация \eqref{eq: rc rank of matrix, sups-rows, 1}
\sups строк ${}_{\gi s}A$ с коэффициентами ${}_{\gi p}r^{\gi s}$,
мы получим систему \eqref{eq: rc rank of matrix, sups-rows, 2}.
Согласно теореме \ref{theorem: nonsingular system of linear equations}
эта система имеет единственное решение\footnote{Мы положим,
что неизвестные переменные здесь - это $x^{\gi s}={}_{\gi p}r^{\gi s}$
\label{footnote: xs=rps}}
и оно нетривиально потому, что все \RC квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \subs строк больше чем $k$.
Пусть нам даны \sups строка ${}_{\gi p}A$ и \subs строка $A^{\gi r}$.
Согласно предположению минор
${}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}$ - \RC вырожденная матрица
и его \RC квазидетерминант
	\begin{equation}
{}_{\gi p}\RCDet{{}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}}^{\gi r}=0
	\label{eq: rc rank of matrix, sups-rows, 3}
	\end{equation}
Согласно
\xEqRef{0612.111}{eq: quasideterminant, 1}
\eqref{eq: rc rank of matrix, sups-rows, 3} имеет вид
	\[
{}_{\gi p}A^{\gi r}
-{}_{\gi p}A^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi r}=0
	\]
Матрица
	\begin{equation}
{}_{\gi p}r
={}_{\gi p}A^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})
	\label{eq: rc rank of matrix, sups-rows, 4}
	\end{equation}
не зависят от $\gi{r}$. Следовательно, для любых $\gi{r}\in\gi{N}\setminus\gi{T}$
	\begin{equation}
{}_{\gi p}A^{\gi r}
={}_{\gi p}r\RCstar {}_{\gi S}A^{\gi r}
	\label{eq: rc rank of matrix, sups-rows, 5}
	\end{equation}

Из равенства
	\[
(({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi l}
={}_{\gi T}\delta^{\gi l}
	\]
следует, что
	\begin{equation}
{}_{\gi p}A^{\gi l}=
{}_{\gi p}A^{\gi T}\RCstar {}_{\gi T}\delta^{\gi l}=
{}_{\gi p}A^{\gi T}\RCstar
(({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi l}
	\label{eq: rc rank of matrix, sups-rows, 7}
	\end{equation}
Подставляя \eqref{eq: rc rank of matrix, sups-rows, 4}
в \eqref{eq: rc rank of matrix, sups-rows, 7}, мы получим
	\begin{equation}
	\label{eq: rc rank of matrix, sups-rows, 8}
{}_{\gi p}A^{\gi l}=
{}_{\gi p}r\RCstar {}_{\gi S}A^{\gi l}
	\end{equation}
\eqref{eq: rc rank of matrix, sups-rows, 5} и \eqref{eq: rc rank of matrix, sups-rows, 8}
завершают доказательство.
		\end{proof}

		\begin{corollary}
		\label{corollary:rc rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$\RCRank A=\gi k<\gi m$.
Тогда \sups строки матрицы \drc линейно зависимы.
	\begin{equation}
	\label{eq: rc rank of matrix, sups-rows drc linearly dependent}
\lambda\RCstar A=0
	\end{equation}
		\end{corollary}
		\begin{proof}
Предположим, что \sups строка ${}_{\gi p}A$ - \drc линейная комбинация
\eqref{eq: rc rank of matrix, sups-rows, 1}. Мы положим
$\lambda^{\gi p}=-1$, $\lambda^{\gi s}={}_{\gi p}r^{\gi s}$
и остальные $\lambda^{\gi c}=0$.
		\end{proof}

		\begin{theorem}
		\label{theorem: rank of coordinate matrix}
Пусть $({}_{\gi i}\Vector{a},\gi i\in\gi M,|\gi M|=\gi m)$ семейство
\drc линейно независимых векторов. Тогда \RC ранг их
координатной матрицы равен $\gi m$.
		\end{theorem}
		\begin{proof}
Согласно конструкции, изложенной в примере \ref{example: drc vector space},
координатная матрица семейства векторов $({}_{\gi i}\Vector{a})$ относительно базиса $\Basis{e}$
состоит из \sups строк, являющихся координатными матрицами векторов
${}_{\gi i}\Vector{a}$ относительно базиса $\Basis{e}$. Поэтому \RC ранг
этой матрицы не может превышать $\gi m$.

Допустим \RC ранг
координатной матрицы меньше $\gi m$.
Согласно следствию \ref{corollary:rc rank of matrix, sups-rows}
\sups строки матрицы \drc линейно зависимы. Если мы умножим обе части равенства
\ref{eq: rc rank of matrix, sups-rows drc linearly dependent} на
\subs строку $\Vector{e}$ 
и положим $c=\lambda\RCstar A$, то мы получим, что \drc линейная комбинация
\[
c\RCstar \Vector{e}=0
\]
векторов базиса равна $0$. Это противоречит утверждению, что векторы $\Vector{e}$ образуют
базис. Утверждение теоремы доказано.
		\end{proof}

		\begin{theorem}
		\label{theorem: rc rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
$$\RCRank A=\gi k<\gi n$$
и ${}_{\gi S}A^{\gi T}$ - \RC главный минор.
Тогда \subs строка $A^{\gi r}$ является
\rcd линейной композицией \subs строк $A^{\gi t}$
	\begin{align}
	\label{eq: rc rank of matrix, star-columns}
A^{\gi{N}\setminus\gi{T}}&=A^{\gi T}\RCstar r\\
	\label{eq: rc rank of matrix, star-columns, 1}
A^{\gi r}&=A^{\gi T}\RCstar r^{\gi r}\\
	\label{eq: rc rank of matrix, star-columns, 2}
{}_{\gi a}A^{\gi r}&={}_{\gi a}A^{\gi t}\ {}_{\gi t}r^{\gi r}
	\end{align}
		\end{theorem}
		\begin{proof}
Если число \sups строк - $\gi k$, то, полагая, что \subs строка $A^{\gi r}$
- \rcd линейная комбинацию \eqref{eq: rc rank of matrix, star-columns, 1}
\subs строк $A^{\gi t}$ с коэффициентами ${}_{\gi t}r^{\gi r}$,
мы получим систему \eqref{eq: rc rank of matrix, star-columns, 2}.
Согласно теореме \ref{theorem: nonsingular system of linear equations}
эта система имеет единственное решение\footnote{Мы положим,
что неизвестные переменные здесь - это ${}_{\gi t}x={}_{\gi t}r^{\gi r}$
\label{footnote: xt=rtq}}
и оно нетривиально потому, что все \RC квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \sups строк больше, чем $\gi k$.
Пусть нам даны \subs строка $A^{\gi r}$ и \sups строка ${}_{\gi p}A$.
Согласно предположению минор
${}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}$ - \RC вырожденная матрица
и его \RC квазидетерминант
	\begin{equation}
{}_{\gi p}\RCDet{{}_{\gi S\cup\{\gi p\}}A^{\gi T\cup\{\gi r\}}}^{\gi r}=0
	\label{eq: rc rank of matrix, star-columns, 3}
	\end{equation}
Согласно
\xEqRef{0612.111}{eq: quasideterminant, 1}
\eqref{eq: rc rank of matrix, star-columns, 3} имеет вид
	\[
{}_{\gi p}A^{\gi r}
-{}_{\gi p}A^{\gi T}\RCstar
({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi r}=0
	\]
Матрица
	\begin{equation}
r^{\gi r}
=({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})\RCstar {}_{\gi S}A^{\gi r}
	\label{eq: rc rank of matrix, star-columns, 4}
	\end{equation}
не зависит от $\gi{p}$, Следовательно, для любых $\gi{p}\in\gi{M}\setminus \gi{S}$
	\begin{equation}
{}_{\gi p}A^{\gi r}
={}_{\gi p}A^{\gi T}\RCstar r^{\gi r}
	\label{eq: rc rank of matrix, star-columns, 5}
	\end{equation}

Из равенства
	\[
{}_{\gi k}A^{\gi T}\RCstar (({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})^{\gi s}
={}_{\gi k}\delta^{\gi s}
	\]
следует, что
	\begin{equation}
{}_{\gi k}A^{\gi r}=
{}_{\gi k}\delta^{\gi S}\RCstar {}_{\gi S}A^{\gi r}=
{}_{\gi k}A^{\gi T}\RCstar (({}^\bullet{}^-_{\gi T}A_\bullet{}^{\gi S}_-)^{\RCInverse})^{\gi s}
\RCstar {}_{\gi s}A^{\gi r}
	\label{eq: rc rank of matrix, star-columns, 7}
	\end{equation}
Подставляя \eqref{eq: rc rank of matrix, star-columns, 4}
в \eqref{eq: rc rank of matrix, star-columns, 7}, мы получим
	\begin{equation}
	\label{eq: rc rank of matrix, star-columns, 8}
{}_{\gi k}A^{\gi r}=
{}_{\gi k}A^{\gi T}\RCstar r^{\gi r}
	\end{equation}
\eqref{eq: rc rank of matrix, star-columns, 5} и \eqref{eq: rc rank of matrix, star-columns, 8}
завершают доказательство.
		\end{proof}

		\begin{corollary}
		\label{corollary:rc rank of matrix, star-columns}
Предположим, что $A$ - матрица,
$\RCRank A=\gi k<\gi m$.
Тогда \subs строки матрицы \rcd линейно зависимы.
	\[
A\RCstar \lambda=0
	\]
		\end{corollary}
		\begin{proof}
Предположим, что \subs строка $A^{\gi r}$ - правая линейная комбинация
\eqref{eq: rc rank of matrix, star-columns, 1}. Мы положим
$\lambda_{\gi r}=-1$, $\lambda_{\gi t}=r_{\gi t}^{\gi r}$
и остальные $\lambda^{\gi c}=0$.
		\end{proof}

Опираясь на теорему \xEqRef{0612.111}{theorem: duality principle, quasideterminants},
мы можем записать подобные утверждения для \CR ранга матрицы.

		\begin{theorem}
		\label{theorem: cr rank of matrix, star-rows}
Предположим, что $A$ - матрица,
\symb{\CRRank  A}0{cr-rank of matrix}
$$\ShowSymbol{cr-rank of matrix}=\gi k<\gi m$$
и ${}^{\gi T}A_{\gi S}$ - \CR главный минор.
Тогда \sups строка $A_{\gi p}$ является
\crd линейной композицией \sups строк $A_{\gi s}$.
	\begin{align}
	\label{eq: cr rank of matrix, star-rows}
A_{\gi{M}\setminus\gi S}&=A_{\gi S}\CRstar r\\
	\label{eq: cr rank of matrix, star-rows, 1}
A_{\gi p}&=A_{\gi S}\CRstar r_{\gi p}\\
	\label{eq: cr rank of matrix, star-rows, 2}
{}^{\gi b}A_{\gi p}&={}^{\gi b}A_{\gi s}\ {}^{\gi s}r_{\gi p}
	\end{align}
		\end{theorem}

		\begin{corollary}
		\label{corollary:cr rank of matrix, star-rows}
Предположим, что $A$ - матрица,
$\CRRank A=\gi k<\gi m$.
Тогда \sups строки матрицы \crd линейно зависимы.
	\[
A\CRstar\lambda=0
	\]
		\end{corollary}

		\begin{theorem}
		\label{theorem: cr rank of matrix, star-columns}
Предположим, что $A$ - матрица,
$$\CRRank A=\gi k<\gi n$$
и ${}^{\gi T}A_{\gi S}$ - \CR главный минор.
Тогда \subs строка ${}^{\gi r}A$ является
\rcd линейной композицией \subs строк $A^{\gi t}$
	\begin{align}
	\label{eq: cr rank of matrix, star-columns}
{}^{\gi{N}\setminus\gi{T}}A&=r\RCstar {}^{\gi T}A\\
	\label{eq: cr rank of matrix, star-columns, 1}
{}^{\gi r}A&={}^{\gi r}r\RCstar {}^{\gi T}A\\
	\label{eq: cr rank of matrix, star-columns, 2}
{}^{\gi r}A_{\gi a}&={}^{\gi r}r_{\gi t}\ {}^{\gi t}A_{\gi a}
	\end{align}
		\end{theorem}

		\begin{corollary}
		\label{corollary:cr rank of matrix, star-columns}
Предположим, что $A$ - матрица,
$\CRRank a=\gi k<\gi m$.
Тогда \subs строки матрицы \drc линейно зависимы.
	\[
\lambda\RCstar A=0
	\]
		\end{corollary}

			\section{Система \texorpdfstring{$D\RCstar$}{Drc}\hyph линейных уравнений}
			\label{section: Columns System of Linear Equations}

		\begin{definition}
Предположим, что\footref{footnote: index assumption}
$A$ - матрица системы \drc линейных уравнений
\eqref{eq: star columns system of linear equations}.
Мы будем называть матрицу
	\begin{equation}
\left(
 \begin{array}{ccc}
{}_{\gi a}A^{\gi b}\\ b^{\gi b}
\end{array}\right)=
\left(
 \begin{array}{cccc}
{}_{\gi 1}A^1 & ... & {}_{\gi 1}A^n\\
... & ... & ... \\
{}_{\gi m}A^1&...& {}_{\gi m}A^n\\
b^1&...& b^n
\end{array}\right)
	\label{eq: extended matrix, system of drc linear equations}
	\end{equation}
\AddIndex{расширенной матрицей}{extended matrix, system of drc linear equations} этой системы.
		\qed
		\end{definition}

		\begin{definition}
Предположим, что\footref{footnote: index assumption}
$a$ - матрица системы \rcd линейных уравнений
\eqref{eq: star rows system of linear equations}.
Мы будем называть матрицу
	\begin{equation}
\left(
\begin{array}{ccc}
{}_{\gi a}A^{\gi b}& {}_{\gi a}b 
\end{array}\right)=
\left(
 \begin{array}{cccc}
{}_{\gi 1}A^1 & ... & {}_{\gi 1}A^n &{}_1b\\
... & ... & ... &...\\
{}_{\gi m}A^1 &...& {}_{\gi m}A^n&{}_mb
\end{array}\right)
	\label{eq: extended matrix, system of rcd linear equations}
	\end{equation}
\AddIndex{расширенной матрицей}{extended matrix, system of rcd linear equations} этой системы.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: star columns system of linear equations}
Система \drc линейных уравнений \eqref{eq: star columns system of linear equations}
имеет решение тогда и только тогда, когда
	\begin{equation}
\RCRank({}_{\gi a}A^{\gi b})=\RCRank\left(
 \begin{array}{ccc}
{}_{\gi a}A^{\gi b}\\ b^{\gi b}
\end{array}\right)
	\label{eq: star columns system of linear equations, rank}
	\end{equation}
		\end{theorem}
		\begin{proof}
Пусть ${}_{\gi S}A^{\gi T}$ - \RC главный минор матрицы $A$.

Пусть система \drc линейных уравнений \eqref{eq: star columns system of linear equations}
имеет решение $x^{\gi a}=d^{\gi a}$. Тогда
	\begin{equation}
d\RCstar A=b
	\label{eq: star columns system of linear equations, 1}
	\end{equation}
Уравнение \eqref{eq: star columns system of linear equations, 1} может быть записано в форме
	\begin{equation}
d^{\gi S}\RCstar {}_{\gi S}A+d^{\gi{M}\setminus\gi S}\RCstar {}_{\gi{M}\setminus\gi S}A=b
	\label{eq: star columns system of linear equations, 2}
	\end{equation}
Подставляя \eqref{eq: rc rank of matrix, sups-rows} в
\eqref{eq: star columns system of linear equations, 2}, мы получим
	\begin{equation}
d^{\gi S}\RCstar {}_{\gi S}A+d^{\gi{M}\setminus\gi S}\RCstar r\RCstar {}_{\gi S}A=b
	\label{eq: star columns system of linear equations, 3}
	\end{equation}
Из \eqref{eq: star columns system of linear equations, 3} следует, что \sups строка
$b$ является \drc линейной комбинацией \sups строк $a_{\gi s}$
	\[
(d^{\gi S}+d^{\gi{M}\setminus\gi S}\RCstar r)\RCstar {}_{\gi S}A=b
	\]
Это эквивалентно уравнению \eqref{eq: star columns system of linear equations, rank}.

Нам осталось доказать, что существование решения \drc системы линейных уравнений
\eqref{eq: star columns system of linear equations} следует из \eqref{eq: star columns system of linear equations, rank}.
Истинность \eqref{eq: star columns system of linear equations, rank} означает, что
${}_{\gi S}A^{\gi T}$ - так же \RC главный минор расширенной матрицы.
Из теоремы \ref{theorem: rc rank of matrix, sups-rows} следует, что \sups строка $b$
является \drc линейной композицией \sups строк $a_{\gi s}$
	\[
b=r^{\gi S}\RCstar {}_{\gi S}A
	\]
Полагая $r^{\gi p}=0$, мы получим
	\[
b=r\RCstar a
	\]
Следовательно, мы нашли, по крайней мере, одно решение системы \eqref{eq: star columns system of linear equations}.
		\end{proof}

		\begin{theorem}
		\label{theorem: left system of linear equations, solution}
Предположим, что \eqref{eq: star columns system of linear equations}
- система \drc линейных уравнений,
удовлетворяющих \eqref{eq: star columns system of linear equations, rank}.
Если $\RCRank  a=\gi k\le \gi m$,
то решение системы зависит
от произвольных значений $\gi m-\gi k$ переменных, не включённых в \RC главный минор.
		\end{theorem}
		\begin{proof}
Пусть ${}_{\gi S}A^{\gi T}$ - \RC главный минор матрицы $a$.
Предположим, что
	\begin{equation}
	\label{eq: star columns system of linear equations, reduce, 1}
x\RCstar a^{\gi r}=b^{\gi r}
	\end{equation}
уравнение с номером $\gi{r}$.
Применяя теорему \ref{theorem: rc rank of matrix, subs-rows}
к расширенной матрице \eqref{eq: extended matrix, system of drc linear equations}, мы получим
	\begin{align}
	\label{eq: star columns system of linear equations, reduce, 2}
a^{\gi r}&=a^{\gi T}\RCstar r^{\gi r}\\
	\label{eq: star columns system of linear equations, reduce, 3}
b^{\gi r}&=b^{\gi T}\RCstar r^{\gi r}
	\end{align}
Подставляя \eqref{eq: star columns system of linear equations, reduce, 2}
и \eqref{eq: star columns system of linear equations, reduce, 3}
в \eqref{eq: star columns system of linear equations, reduce, 1}, мы получим
	\begin{equation}
	\label{eq: star columns system of linear equations, reduce, 4}
x\RCstar a^{\gi T}\RCstar r^{\gi r}=b^{\gi T}\RCstar r^{\gi r}
	\end{equation}
\eqref{eq: star columns system of linear equations, reduce, 4} означает, что
мы можем исключить уравнение \eqref{eq: star columns system of linear equations, reduce, 1}
из системы \eqref{eq: star columns system of linear equations}
и новая система эквивалентна старой.
Следовательно, число уравнений может быть уменьшено до $\gi k$.

В этом случае
у нас есть два варианта. Если число переменных также равно $\gi k$, то
согласно теореме \ref{theorem: nonsingular system of linear equations} система имеет единственное решение
\eqref{eq: nonsingular system of linear equations, solution, quasideterminant}.
Если число переменных $\gi m>\gi k$, то мы можем передвинуть $\gi m-\gi k$ переменных, которые не
включены в \RC главный минор в правой части.
Присваивая произвольные значения этим переменным, мы определяем значение
правой части и для этого значения мы получим единственное решение
согласно теореме \ref{theorem: nonsingular system of linear equations}.
		\end{proof}

		\begin{corollary}
		\label{corollary:  nonsingular rows system of linear equations}
Система \drc линейных уравнений \eqref{eq: star columns system of linear equations}
имеет единственное решение тогда и только тогда, когда
её матрица невырожденная.
		\qed
		\end{corollary}

		\begin{theorem}
		\label{theorem: Solutions homogenous system of linear equations}
Решения однородной системы \drc линейных уравнений
	\begin{equation}
x\RCstar a=0
	\label{eq: homogenous system of linear equations}
	\end{equation}
порождают \drc векторное пространство.
		\end{theorem}
		\begin{proof}
Пусть $\mathcal{X}$ - множество решений системы
\eqref{eq: homogenous system of linear equations}.
Предположим, что $x=(x^{\gi a})\in\mathcal{X}$ and $y=(y^{\gi a})\in\mathcal{X}$.
Тогда \[x^{\gi a}\ _{\gi a}a^{\gi b}=0\] \[y^{\gi a}\ _{\gi a}a^{\gi b}=0\]
Следовательно,
\[
(x^{\gi a}+y^{\gi a})\ _{\gi a}a^{\gi b}=
x^{\gi a}\ _{\gi a}a^{\gi b}+y^{\gi a}\ _{\gi a}a^{\gi b}=0
\]
\[x+y=(x^{\gi a}+y^{\gi a})\in\mathcal{X}\]
Таким же образом мы видим
\[
(bx^{\gi a})\ _{\gi a}a^{\gi b}=b(x^{\gi a}\ _{\gi a}a^{\gi b})=0
\]
\[bx=(bx^{\gi a})\in\mathcal{X}\]
Согласно определению \ref{definition: Tstar vector space}
$\mathcal{X}$ является \drc векторным пространством.
		\end{proof}

			\section{Невырожденная матрица}

Предположим, что нам дана $\gi n\times \gi n$ матрица $A$.
Следствия \ref{corollary:rc rank of matrix, sups-rows}
и \ref{corollary:rc rank of matrix, star-columns}
говорят нам, что если $\RCRank a<\gi n$,
то \sups строки \drc линейно зависимы
и \subs строки \rcd линейно зависимы.\footnote{Это
утверждение похоже на утверждение
\citeBib{q-alg-9705026}-\href{http://arxiv.org/PS_cache/q-alg/pdf/9705/9705026.pdf\#Page=6}{1.2.5}.}

		\begin{theorem}
		\label{theorem: rc rank, rows}
Пусть $A$ - $\gi n\times\gi n$ матрица
и \sups строка ${}_{\gi a}A$ - \drc линейная комбинация других \sups строк.
Тогда $\RCRank  A<\gi n$.
		\end{theorem}
		\begin{proof}
Утверждение, что \sups строка ${}_{\gi a}A$ является \drc линейной комбинацией других \sups строк,
означает, что система \drc линейных уравнений
	\begin{equation}
	\label{eq: rc rank, rows}
{}_{\gi a}A=\lambda\RCstar {}_{[\gi a]}A
	\end{equation}
имеет, по крайней мере, одно решение.
Согласно теореме \ref{theorem: star columns system of linear equations}
\[
\RCRank A=\RCRank {}_{[\gi a]}A
\]
Так как число \sups строк меньше, чем $\gi n$, то
$\RCRank {}_{[\gi a]}A<\gi n$.
		\end{proof}

		\begin{theorem}
		\label{theorem: rc rank, columns}
Пусть $A$ - $\gi n\times \gi n$ матрица
и \subs строка $A^{\gi b}$ - \rcd линейная комбинация других \subs строк.
Тогда $\RCRank A<\gi n$.
		\end{theorem}
		\begin{proof}
Доказательство утверждения похоже на доказательство теоремы \ref{theorem: rc rank, rows}
		\end{proof}

		\begin{theorem}
Предположим, что $A$ и $B$ - $\gi n\times\gi n$ матрицы и
	\begin{equation}
	\label{eq: RC product singular, 1}
C=A\RCstar B
	\end{equation}
$C$ - \RC вырожденная матрица тогда и только тогда, когда
либо матрица $A$, либо матрица $B$ - \RC вырожденная матрица.
		\end{theorem}
		\begin{proof}
Предположим, что матрица $A$ - \RC вырожденная.
Согласно теореме \ref{theorem: rc rank of matrix, sups-rows}
\sups строки матрицы $A$
\drc линейно зависимы. Следовательно,
	\begin{equation}
	\label{eq: RC product singular, 2}
0=\lambda\RCstar A
	\end{equation}
где $\lambda\ne 0$. Из
\eqref{eq: RC product singular, 1}
и \eqref{eq: RC product singular, 2} следует, что
\[
\lambda\RCstar C=\lambda\RCstar A\RCstar B=0
\]
Согласно теореме \ref{theorem: rc rank, rows} матрица $C$
является \RC вырожденной.

Предположим, что матрица $A$ - не \RC вырожденная, но матрица $B$ - \RC вырожденная.
Согласно теореме \ref{theorem: rc rank of matrix, sups-rows}
\sups строки матрицы $B$
\drc линейно зависимы. Следовательно,
	\begin{equation}
	\label{eq: RC product singular, 3}
0=\mu\RCstar B
	\end{equation}
где $\mu\ne 0$. Согласно
теореме \ref{theorem: nonsingular system of linear equations} система
	\[
\lambda\RCstar A=\mu
	\]
имеет единственное решение, где $\lambda\ne 0$.
Следовательно,
\[
\lambda\RCstar C=\lambda\RCstar A\RCstar B
=\mu\RCstar B=0
\]
Согласно теореме \ref{theorem: rc rank, rows} матрица $C$ является \RC вырожденной.

Предположим, что матрица $C$ - \RC вырожденная матрица.
Согласно теореме \ref{theorem: rc rank of matrix, sups-rows}
\sups строки матрицы $C$
\drc линейно зависимы. Следовательно,
	\begin{equation}
	\label{eq: RC product singular, 4}
0=\lambda\RCstar C
	\end{equation}
где $\lambda\ne 0$.
Из \eqref{eq: RC product singular, 1}
и \eqref{eq: RC product singular, 4} следует, что
	\[
0=\lambda\RCstar A\RCstar B
	\]
Если 
	\[
0=\lambda\RCstar A
	\]
выполнено, то матрица $A$ - \RC вырожденная. Предположим, что
матрица $A$ не \RC вырожденная. Положим
	\[
\mu=\lambda\RCstar A
	\]
где $\mu\ne 0$. Тогда
	\begin{equation}
	\label{eq: RC product singular, 5}
0=\mu\RCstar B
	\end{equation}
Из \eqref{eq: RC product singular, 5} следует, что
матрица $B$ - \RC вырожденная.
		\end{proof}

Опираясь на теорему \xEqRef{0612.111}{theorem: duality principle, quasideterminants},
мы можем записать подобные утверждения для \crd линейной комбинации \sups строк
или \drc линейной комбинации \subs строк и \CR квазидетерминанта.

		\begin{theorem}
		\label{theorem: cr rank, rows}
Пусть $A$ - $\gi n\times\gi n$ матрица
и \sups строка $A_{\gi a}$ - \crd линейная комбинация других \sups строк.
Тогда $\CRRank  A<\gi n$.
		\end{theorem}

		\begin{theorem}
		\label{theorem: cr rank, columns}
Пусть $A$ - $\gi n\times \gi n$ матрица
и \subs строка $A^{\gi b}$ - \dcr линейная комбинация других \subs строк.
Тогда $\CRRank  A<\gi n$.
		\end{theorem}

		\begin{theorem}
Предположим, что $A$ и $B$ - $\gi n\times\gi n$ матрицы и
$C=A\CRstar B$. $C$ - \CR вырожденная матрица тогда и только тогда, когда
либо матрица $A$, либо матрица $B$ - \CR вырожденная матрица.
		\end{theorem}

		\begin{definition}
\AddIndex{\RC матричная группа}{rc-matrix group}
\symb{\RCGL nD}1{rc-matrix group} - это группа
\RC невырожденных матриц, гле мы определяем
\RC произведение матриц
\xEqRef{0612.111}{eq: rc-product of matrices}
и \RC обратную матрица
$A^{\CRInverse}$.
		\qed
		\end{definition}

		\begin{definition}
\AddIndex{\CR матричная группа}{cr-matrix group}
\symb{\CRGL nD}1{cr-matrix group} - это группа
\CR невырожденных матриц
где мы определяем
\CR произведение матриц
\xEqRef{0612.111}{eq: cr-product of matrices}
и \CR обратную матрицу
$A^{\CRInverse}$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: CR RC singular matrix}
	\[
\RCGL nD\ne \CRGL nD
	\]
		\end{theorem}
		\begin{remark}
Из теоремы
\xEqRef{0612.111}{theorem: RC-inverse matrix, delta}
следует, что
существуют матрицы, которые \CR невырожденны и \RC невырожденны.
Теорема \ref{theorem: CR RC singular matrix} означает, что множества
\CR невырожденных матриц и \RC невырожденных матриц
не совпадают. Например,
существует такая \RC невырожденная матрица, которая
\CR вырожденная матрица.
		\qed
		\end{remark}
		\begin{proof}
Это утверждение достаточно доказать для $n={\gi 2}$.
Предположим, что каждая \CR вырожденная матрица
	\begin{equation}
a=
\left(
 \begin{array}{ccc}
a_{\gi 1}^{\gi 1} 
&
a_{\gi 1}^{\gi 2}
\\
a_{\gi 2}^{\gi 1} 
&
a_{\gi 2}^{\gi 2}
\end{array}
\right)
	\label{eq: CR-singular matrix, 1}
	\end{equation}
является \RC вырожденной матрицей.
Из теоремы \ref{theorem: rc rank of matrix, subs-rows} и
теоремы \ref{theorem: rc rank of matrix, subs-rows} следует, что
\RC вырожденная матрица удовлетворяет условию
	\begin{align}
	\label{eq: CR, row, 2 1, 1 1}
a_{\gi 2}^{\gi 1}&=b a_{\gi 1}^{\gi 1}\\
	\label{eq: CR, row, 2 2, 1 2}
a_{\gi 2}^{\gi 2}&=b a_{\gi 1}^{\gi 2}\\
	\label{eq: CR, column, 1 2, 1 1}
a_{\gi 1}^{\gi 2}&=a_{\gi 1}^{\gi 1} c\\
	\label{eq: CR, column, 2 2, 2 1}
a_{\gi 2}^{\gi 2}&=a_{\gi 2}^{\gi 1} c
	\end{align}
Если мы подставим \eqref{eq: CR, column, 1 2, 1 1}
в \eqref{eq: CR, row, 2 2, 1 2}, мы получим
	\begin{equation}
	\label{eq: CR, a22, 2}
a_{\gi 2}^{\gi 2}=b a_{\gi 1}^{\gi 1} c
	\end{equation}
$b$ и $c$ - произвольные элементы тела $D$ и \RC вырожденная матрица
\eqref{eq: CR-singular matrix, 1} имеет вид ($d=a_{\gi 1}^{\gi 1}$)
	\begin{equation}
a=
\left(
 \begin{array}{ccc}
d 
&
d c
\\
b d 
&
b d c
\end{array}
\right)
	\label{eq: RC-singular matrix, 2}
	\end{equation}
Подобным образом мы можем показать, что \CR вырожденная матрица
имеет вид
	\begin{equation}
a=
\left(
 \begin{array}{ccc}
d 
&
c' d
\\
d  b'
&
c' d b'
\end{array}
\right)
	\label{eq: CR-singular matrix, 2}
	\end{equation} 
Из предположения следует, что \eqref{eq: CR-singular matrix, 2}
и \eqref{eq: RC-singular matrix, 2} представляют одну и ту же матрицу.
Сравнивая \eqref{eq: CR-singular matrix, 2}
и \eqref{eq: RC-singular matrix, 2}, мы получим, что
для любых $d,c\in D$ существует такое $c'\in D$, которое не зависит от $d$ и
удовлетворяет уравнению
\[d c=c'd\]
Это противоречит утверждению, что $D$ - тело.
		\end{proof}

		\begin{example}
В случае тела кватернионов мы положим $b=1+k$, $c=j$, $d=k$.
Тогда мы имеем\footnote{Я привожу расчёты в файле Vector.Space.Russian.tex.}
\[
a=\left(
 \begin{array}{ccc}
k
&
k j 
\\
(1+k) k 
&
(1+k) k j
\end{array}
\right)
=\left(
 \begin{array}{ccc}
k
&
-i
\\
k-1 
&
-i-j
\end{array}
\right)
\]
	\begin{align*}
\RCDet{a}^{\gi 2}_{\gi 2}
&=a_{\gi 2}^{\gi 2}
-a_{\gi 2}^{\gi 1}
(a_{\gi 1}^{\gi 1})^{-1}a_{\gi 1}^{\gi 2}
	\\
&=-i-j- (k-1)(k)^{-1} (-i)
	\\
%=-i-j-(k-1) k i
%=-i-j- k ki+ ki
%=-i-j+i +j
&=0
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 1}^{\gi 1}
&=a^{\gi 1}_{\gi 1}
-a^{\gi 1}_{\gi 2}(a^{\gi 2}_{\gi 2})^{-1}a^{\gi 2}_{\gi 1}
	\\
&=k
-(k-1) (-i-j)^{-1}(-i) 
	\\
%=k-(k-1)\frac 12 (i+j) (-i)
%=k+\frac 12 ((k-1)i+(k-1)j)i
%=k+\frac 12 (ki-i+kj-j)i
%=k+\frac 12 (j-i-i-j)i
%=k- ii
&=k+ 1
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 1}^{\gi 2}
&=a^{\gi 2}_{\gi 1}
-a^{\gi 2}_{\gi 1}(a^{\gi 1}_{\gi 2})^{-1}a^{\gi 2}_{\gi 1}
	\\
&=(-i)
-(-i) (k-1)^{-1} (-i)
	\\
%=-i+i\frac 12 (k+1) i
%=-i-\frac 12 (k+1) ii
%=-i+\frac 12(k+1)
&=-i+\frac 12k+\frac 12
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 2}^{\gi 1}
&=a^{\gi 1}_{\gi 2}
-a^{\gi 1}_{\gi 2}(a^{\gi 2}_{\gi 1})^{-1}a^{\gi 1}_{\gi 2}
	\\
&=(-i)
-(k-1) (-i)^{-1} (k-1)
	\\
%=(-i)-(k-1) i (k-1)
%=-i+i(k-1) (k-1) 
%=-i+i(k^2-2k+1)
%=-i-2ik
&=-i+2j
	\end{align*}
	\begin{align*}
\CRDet{a}_{\gi 2}^{\gi 2}
&=a^{\gi 2}_{\gi 2}
-a^{\gi 2}_{\gi 1}
(a^{\gi 1}_{\gi 1})^{-1}\ a^{\gi 1}_{\gi 2}
	\\
&=-i-j
-(-i) (k)^{-1}(k-1)
	\\
%=-i-j-(k-1) k i
%=-i-j-k k i+ k i
%=-i-j+ i+ j
&=-2i
	\end{align*}
		\qed
		\end{example}

			\section{Размерность \texorpdfstring{$D\RCstar$}{Drc}\hyph векторного пространства}
			\label{section: Dimension of Vector Space}

		\begin{theorem}
		\label{theorem: basis of vector space}
Пусть $\mathcal{V}$ - \drc векторное пространство. Предположим, что $\mathcal{V}$ имеет
\drc базисы $\Basis{e}=({}_{\gi a}\Vector{e},\gi{a}\in\gi{I})$
и $\Basis{g}=({}_{\gi b}\Vector{g}, \gi{b}\in\gi{J})$.
Если $|\gi{I}|$ и $|\gi{J}|$ - конечные числа, то $|\gi{I}|=|\gi{J}|$.
%Если $|S|$ is конечные число, то $|\gi{J}|$ is конечные число и $|\gi{I}|=|\gi{J}|$.
		\end{theorem}
		\begin{proof}
Предположим, что $|\gi{I}|=\gi m$ и $|\gi{J}|=\gi n$. Предположим, что
	\begin{equation}
\gi m<\gi n
	\label{eq: basis of vector space, 0}
	\end{equation}
Так как $\Basis{e}$ - \drc базис, любой
вектор ${}_{\gi b}\Vector{g}$, $\gi{b}\in\gi{J}$
имеет разложение
	\[
{}_{\gi b}\Vector{g}={}_{\gi b}a\RCstar \Vector{e}
	\]
Так как $\Basis{g}$ - \drc базис
	\begin{equation}
\lambda=0
	\label{eq: basis of vector space, 1}
	\end{equation}
следует из
	\[
\lambda\RCstar \Vector{g}
=\lambda\RCstar a\RCstar \Vector{e}=0
	\]
Так как $\Basis{e}$ - \drc базис, мы получим
	\begin{equation}
\lambda\RCstar a=0
	\label{eq: 2 bases, vector space}
	\end{equation}
Согласно \eqref{eq: basis of vector space, 0}
$\RCRank a\le \gi m$ и система \eqref{eq: 2 bases, vector space}
имеет больше переменных, чем уравнений. Согласно
теорема \ref{theorem: left system of linear equations, solution}
$\lambda\ne 0$. Это противоречит
утверждению \eqref{eq: basis of vector space, 1}. 
Следовательно, утверждение $\gi m<\gi n$ неверно.

Таким же образом мы можем доказать, что утверждение $\gi n<\gi m$ неверно.
Это завершает доказательство теоремы.
		\end{proof}

		\begin{definition}
Мы будем называть \AddIndex{размерностью \drc векторного пространства}{dimension of vector space}
число векторов в базисе
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: coordinate matrix of basis}
Координатная матрица \drc базиса $\Basis{g}$ относительно \drc базиса $\Basis{e}$
векторного пространства $\mathcal{V}$ является \RC невырожденной матрицей.
		\end{theorem}
		\begin{proof}
Согласно лемме \ref{theorem: rank of coordinate matrix}
\drc ранг координатной матрицы базиса $\Basis{g}$ относительно базиса $\Basis{e}$
равен размерности векторного пространства, откуда следует утверждение теоремы.
		\end{proof}

		\begin{definition}
Мы будем называть взаимно однозначное отображение $\Vector A:\mathcal{A}\rightarrow \mathcal{B}$ 
\AddIndex{\drc изоморфизмом векторных пространств}{isomorphism of vector spaces},
если это отображение - \drc линейное отображение
векторных пространств.
		\qed
		\end{definition}

		\begin{definition}
\AddIndex{\drc автоморфизм векторного пространства}{automorphism of vector space}
$\mathcal{V}$ - это \drc изоморфизм $\Vector A:\mathcal{V}\rightarrow \mathcal{V}$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: automorphism of vector space}
Предположим, что $\Basis{f}$ - \drc базис в векторном пространстве $\mathcal{V}$.
Тогда любой \drc автоморфизм $\Vector A$ векторного пространства
$\mathcal{V}$ имеет вид
	\begin{equation}
v'=v\RCstar  A
	\label{eq: automorphism, vector space}
	\end{equation}
где $A$ - \RC невырожденная матрица.
		\end{theorem}
		\begin{proof}
\eqref{eq: automorphism, vector space} следует из
теоремы \ref{theorem: drc linear map of drc vector space}.
Так как $\Vector A$ - изоморфизм, то для каждого вектора $\Vector v'$ существует единственный вектор $\Vector v$ такой,
что $\Vector v'=\Vector v\RCstar \Vector A$.
Следовательно, система \drc линейных уравнений \eqref{eq: automorphism, vector space}
имеет единственное решение. Согласно следствию \ref{corollary: nonsingular rows system of linear equations}
матрица $A$ невырожденна.
		\end{proof}

		\begin{theorem}
		\label{theorem: Automorphisms of vector space form a group}
Автоморфизмы \drc векторного пространства порождают группу $\RCGL nD$.
		\end{theorem}
		\begin{proof}
Если даны два автоморфизма $\Vector A$ и $\Vector B$, то мы можем записать
	\begin{align*}
v'&=v\RCstar A\\
v''=v'\RCstar B&=v\RCstar A\RCstar B
	\end{align*}
Следовательно, результирующий автоморфизм имеет матрицу $A\RCstar B$.
		\end{proof}

